Sharp, strong and unique minimizers for low complexity robust recovery

In this paper, we show the important roles of sharp minima and strong minima for robust recovery. We also obtain several characterizations of sharp minima for convex regularized optimization problems. Our characterizations are quantitative and verifiable especially for the case of decomposable norm regularized problems including sparsity, group-sparsity, and low-rank convex problems. For group-sparsity optimization problems, we show that a unique solution is a strong solution and obtain quantitative characterizations for solution uniqueness.

==> tex_220921/sec_conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper we show that sharp minima and strong minima play important roles for robust recovery with different rates. We also provide some quantitative  characterizations for sharp solutions to convex regularized problems. Unique solutions to $\ell_1$ problems are actually sharp solutions. For group sparsity problems, unique solutions are strong solutions. We also obtain several conditions guaranteeing solution uniqueness to group sparsity problems.   As solution uniqueness to $\ell_1$ problem plays a central role in the area of exact recovery with high probability, we plan to use our results to find a better bound for exact recovery for group-sparsity problems in comparison with the one obtained in \cite{CR13,RRN12}, at which they only use sufficient conditions for solution uniqueness. 

Example~\ref{Last3} and Example~\ref{Last} raise important questions about the solution uniqueness and strong minima for the nuclear norm minimization problems. Unique solutions to \eqref{BP0} with the nulear norm are neither sharp nor strong solutions. But a strong solution in this case is certainly a unique solution. It means that second-order analysis can provide a sufficient condition for solution uniqueness, and such a condition should be weaker than the one in Theorem~\ref{mtheo} for sharp solutions. However, unlike the analysis in Lemma~\ref{SOD}, the second subderivative of the nuclear norm is far more intricate to compute. Understanding  solution uniqueness and strong minima for the case of the nuclear norm, or more generally for spectral functions, is a project that we plan to pursue in the future. %We need geometric characterization for strong solution like (iii) in Theorem~\ref{BP12} to proceed further.  


==> tex_220921/sec_intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem statement}
Inverse problems and regularization theory is a central theme in various areas of engineering and science. A typical case is where one observes a vector $y_0 \in \R^m$ of linear measurements according to
\begin{equation}\label{y0}
    y_0=\Phi x_0 
\end{equation}
where $\Phi \in \R^{m\times n}$ is known, and is typically an idealization of the sensing mechanism in signal/imaging science applications, or the design matrix in a parametric statistical regression problem. The vector $x_0 \in \R^n$ is the unknown quantity of interest. 

Solving the inverse problem associated to the linear forward model \eqref{y0} amounts to recovering $x_0$, either exactly or to a good approximation, knowing $y_0$ and $\Phi$. This is however a quite challenging task especially when the linear system \eqref{y0} is underdetermined with $m \ll n$. In fact, even when $m=n$, $\Phi$ is in general ill-conditioned or even singular. This entails that the linear inverse problem is in general ill-posed.

In order to bring back the problem to the land of well-posedness, it is necessary to restrict the inversion process to a well-chosen subset of $\R^n$ containing the plausible solutions including $x_0$. This can be achieved by adopting a variational framework and solving the following optimization problem
\begin{equation}\label{BP0}
    \min_{x\in \R^n}\quad J(x) \qsubjq \Phi x=y_0,
\end{equation}
where $J$ is function which is bounded from below (wlog non-negative). The function $J$, known as a regularizer, is designed in such way that it is the smallest on the sought-after solutions. Popular example in signal/image processing and machine learning is the $\ell_1$ norm to promote sparsity, the $\ell_1/\ell_2$ to promote group sparsity, analysis sparsity seminorm (i.e., $J = J_0 \circ D^*$, $D^*: \R^n \to \R^p$ is linear and $J_0$ is the $\ell_1$ or $\ell_1/\ell_2$ norm); see \cite{BDE09,CT04,DH01, JKL15,RRN12, RF08, T96, VPDF13,YL06} to cite a few. Another popular example is the nuclear norm, i.e., the $\ell_1$ norm of the singular values of a matrix, to recover low-rank matrices \cite{CRPW12,CR09}. These prototypical cases are included in the class of decomposable norms \cite{NRWY09,CR13,FPVDS13} that covers a wide range of optimization-based recovery problems in different areas of data science. 


When the observation is subject to errors, the system \eqref{y0} is modified to   
\begin{equation}\label{yw}
    y=\Phi x_0 +\omega
\end{equation}
where $\omega$ that accounts either for noise and/or modeliing errors. The errors can be either deterministic (in this case, one typically assumes to know some bound on $\|\omega\|$) or random (in which case its distribution is assumed to be known). Throughout, $\omega$ will be assumed deterministic with $\|\omega\|\le \delta$, with $\delta > 0$ known.

To recover $x_0$ from \eqref{yw}, one solves the noise-aware form (aka as Mozorov regularization in the inverse problems literature)
\begin{equation}\label{BP1}
\min_{x \in \R^n} J(x)\quad \mbox{subject to}\quad \|y - \Phi x\| \le \delta
\end{equation}
or its penalized/Lagrangian form (aka Tikhonov regularization in the inverse problems literature)
\begin{equation}\label{Las3}
\min_{x \in \R^n} \frac{1}{2}\|\Phi x-y\|^2+ \mu J(x) .
\end{equation}
with regularization parameter $\mu>0$. It is well-known that \eqref{BP1} and \eqref{Las3} are formally equivalent in the sense that there exists a bijection between $\delta$ and $\mu$ such that the both problems share the same set of solutions.

We say that {\em robust recovery} occurs when solutions to \eqref{BP1} or \eqref{Las3} are close enough to the original signal $x_0$ as long as $\mu$ is appropriately chosen (as a function of the noise level $\delta$). For $\ell_1$-regularized optimization problem, a significant result was achieved in \cite[Theorem~4.7]{GHS11}, which shows that when $\mu$ is proportional to $\delta$, the error between any solution of problem \eqref{Las3} to $x_0$ is $\mathcal{O}(\delta)$\footnote{This justifies the conventional terminology "linear convergence rate".} if and only if $x_0$ is the unique solution to \eqref{BP0}. The structure of the $\ell_1$ norm plays a crucial role in their result. Sufficient (but not necessary in general) conditions for robust recovery with a linear convergence rate have been proposed for general class of regularizers by solving either \eqref{BP1} or \eqref{Las3}; see \cite{CRPW12, FPVDS13, V14, VPF15, Tropp15} and references therein. For instance \cite{CRPW12} and \cite{Tropp15} provide a sufficient condition via the geometric notion of {\em descent cone} for robust recovery with linear rate by solving \eqref{BP1} (but not \eqref{Las3}). Injectivity of $\Phi$ on the descent cone turns out to be a sufficient and necessary condition for solution uniqueness of \eqref{BP0}. However, solution uniqueness is not enough to guarantee robust recovery with linear rate for general regularizers. 

In fact, we observe that \cite{CRPW12} needs $x_0$ to be a {\em sharp} solution to problem \eqref{BP0}. A sharp minimum, introduced by Crome and Polyak \cite{C78,P79,P87}, is a point around which the objective value has a first-order growth (see Section~\ref{sec:prelim} for a rigorous definition and discussion). It is certainly sufficient for solution uniqueness and indeed is called {\em strong uniqueness} in \cite{C78}. In the case of polyhedral problems, e.g., problem \eqref{BP0} with $\ell_1$ or $\ell_\infty$ norms, solution uniqueness is equivalent to sharp minima. This is the key reason why \cite{GHS11} only needs solution uniqueness for robust recovery. In the optimization community, sharp minima is well-known for its essence to finite convergence of the proximal point algorithms; see, e.g., \cite{P87, R76}.    



%outside the case of polyhedral norm such as $\ell_1$ and $\ell_\infty$ norms, solution uniqueness i    



% and the loss function $f:\R^m\to\R\cup\{\infty\}$ being convex. The appearance of $f(\Phi x)$ in \eqref{Las0} usually represents for the distance between $\Phi x$ and $\oy$. The choice of $f$ normally depends on the type of noise $\omega$ and the information of data set. For example, if $\omega$ is a Gaussian noise, $f(\cdot)$ could be chosen  as $\frac{1}{2}\|\cdot-\bar y\|^2$; if $\omega$ is a Poisson noise, $f(\cdot)$  could be  chosen as the Kulback-Leibler divergence.  %There are many other different choices of cost functions such as logistic regression loss, 

Sharp minima is actually hidden in both {\em exact recovery} (by solving \eqref{BP0}) and robust recovery. As we will show later, sharpness is closely related to many other results on exact and robust recovery, for instance those involving conditions based on non-degenerate dual certificates (aka {\em Strong Source Condition}) and restricted injectivity of $\Phi$, or the {\em Null Space Property} and its variants; see \cite{DH01, CT04, T04, F05, T06, CR09, BDE09, GHS11, FR13, VPDF13, FPVDS13, CR13, VPDF13, V14, VPF15, ZYY16}. When $\Phi$ is drawn from an appropriate random ensemble, existing sample complexiy bounds (i.e., a lower-bound on $m$ depending on the "intrinsic" dimension of the model subspace containing $x_0$ and logarithmically on $n$) rely on verifying the afore-mentioned conditions with high probability on $\Phi$; see \cite{FR13,VPF15,Tropp15} for comprehensive reviews. For Gaussian measurements, sample complexity bounds for exact recovery are provided in terms of the Gaussian width in \cite{CRPW12} and the statistical dimension in \cite{ALMT14}, and the latter has been shown to precise predictions about the quantitative aspects of the phase transition for exact recovery from Gaussian measurements.

Another popular notion in optimization \cite{BS00,RW98} is that of {\em strong minima}, which is a sufficient condition for solution uniqueness. It is also used implicitly in many results on robust recovery. A strong minimum is a point around which the objective value has a quadratic (or second-order) growth. Strong minima are certainly weaker than sharp minima. In the $\ell_1$ case, we observe  that the cost function in \eqref{Las3} belongs to the bigger class of convex {\em piecewise linear-quadratic functions} \cite{RW98}. A unique solution to this function is also a strong solution. This simple observation was used recently in \cite{BLN19} to obtain some characterizations for solution uniqueness to \eqref{Las3} for the case of the Lasso problem. Necessary and sufficient conditions for solution uniqueness to \eqref{Las3} where $J$ is piecewise linear are also studied in \cite{G17,MS19,ZYY16}.
%For $\ell_1$ problems, Fuchs \cite{F05} and Tropp \cite{T04} introduced a synthesis criterion that guarantees solution uniqueness to \eqref{Las3} when $\mu$ is sufficiently small and $y=y_0$. Moreover,  this unique solution has the same sign and support with the original signal $x_0$. It means that one only needs to solve problem \eqref{Las3} with some small  $\mu$ to get enough information about the sign and support of $x_0$. This   criterion has been studied extensively in the literature; see, e.g., \cite{BDE09, FPVDS13, VPDF13, T06}. Solution uniqueness to problem \eqref{Las3} is significant in this direction.  \\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contributions and relation to prior work} 
The chief goal of this paper is to show the intricate and important roles of sharp minima and strong minima in robust recovery. Our main contributions are as follows.

\begin{enumerate}[label=$\bullet$]
\item As discussed above, solution uniqueness and sharp minima play a pivotal role for robust recovery with linear rate. However,except the case where the regularizer $J$ is merely polyhedral, a unique solution may not be sharp. For example, as we will show in our Section~\ref{sec:stronggroup}, a unique solution to the group-sparsity problem \eqref{BP0} is always a strong minimum but not a sharp one. The natural question is therefore wether strong minima could also lead to some meaningful results for robust recovery. Section~\ref{sec:unique} answers this question positively without even needing convexity of $J$, unlike the previous work of \cite{V14,VPF15} which showed that a sharp minimizer implicitly guarantees robust recovery with linear rate, but convexity was essential there. We show that if $x_0$ is a strong solution to \eqref{BP0}, then we have robust recovery by solving \eqref{BP1} or \eqref{Las3} with a convergence rate $\mathcal{O}(\sqrt{\delta})$ (Theorem~\ref{SRob}). This rate can be improved to the linear rate $\mathcal{O}(\delta)$ when $J = \|\cdot\|$. Whether this linear rate for robust recovery can be achieved for other regularizers under the sole strong minimality assumption is an open question. Besides that main result, we also revisit in Theorem~\ref{Rob} robust recovery results when $x_0$ is assumed to be a sharp minimizer by proving linear convergence and providing more explicit bounds in comparison to the results in \cite{CRPW12, FPVDS13, GHS11, ZYY16}.    


\item Our second main contribution, at the heart of Section~\ref{sec:sharp}, is to study necessary and sufficient conditions for the properties of sharp and strong minima. As mentioned above, solution uniqueness is characterized via the descent cone \cite{CRPW12}. But it is hard to compute the descent cone for general functions $J$. On the other hand, sharp and strong minima can be characterized explicitly via first and second-order analysis \cite{BS00,P87,RW98}. We leverage these tools (see Theorem~\ref{mtheo} and Proposition~\ref{Stheo}) to get equivalent charaterizations of unique/sharp/strong solutions, and to obtain a quantitative condition for convex regularized problems that allows us to check numerically that a solution is sharp. This condition bears similarities with the strong source condition of \cite{GHS11,V14,VPF15}. Our approach does not rely on any polyhedral structure. This distinguishes our results from several ones the literature as in \cite{G17,MS19,ZYY16}, and allows us to work on more general optimization problems. We also believe that non-smooth second-order analysis of the type we develop here, which is a powerful tool in variational analysis and nonsmooth optimization, is not well-known in the robust recovery literature, and are thus of particular importance in this context.


\item Finally, Section~\ref{sec:stronggroup} is devoted to a comprehensive treatment of unique/strong solutions for group-sparsity minimization problems \cite{RRN12,RF08,YL06}, an important class of \eqref{BP0} where $J$ is the $\ell_1/\ell_2$ norm. Sufficient conditions for solution uniqueness for group-sparsity minimization problems were achieved in \cite{CR13, G11, JKL15, RRN12, RF08, V14, VPF15}, but none of them are necessary. To find a characterization for solution uniqueness, we first obtain a closed form for the descent cone (Theorem~\ref{Uniq}). To the best of our knowledge, this was an open question in the literature, though the {\em statistical dimension} of this cone is more computable \cite{ALMT14}. By relying again on second-order analysis \cite{BS00, RW98}, we show that a unique solution to group-sparsity minimization problems \eqref{BP0} and \eqref{Las3} is indeed a strong solution (Theorem~\ref{BP12}). This result is interesting in two ways: first, the function in \eqref{BP0} is not piecewise linear-quadratic, which rules out the approach developed in \cite{BLN19} to unify solution uniqueness and strong minima; second, strong solutions are possibly more natural than sharp solutions for non-polyhedral minimization problems whenever solution uniqueness occurs. Moreover, we establish a quantitative condition for checking unique/strong solutions to group-sparsity problems that is equivalent to solving a smooth convex optimization  problem. This convex problem can be solved via available packages such as \texttt{cvxopt} as we will illustrate in the numerical results of Section~\ref{sec:numerics}. Consequently, we show that solution uniqueness to group-sparsity problem is equivalent to the robust recovery with rate $\mathcal{O}(\sqrt{\delta})$ for both problems \eqref{BP1} and \eqref{Las3}. 

\end{enumerate}

\begin{Remark}
Although we do not have a rigorous study for the case where $J$ is the nuclear norm in this paper, we provide several examples showing that a unique solution to \eqref{BP0} with the nuclear norm is neither sharp nor strong. This raises the challenge of understanding the interplay between unique, sharp, and strong solutions in this case. Some open questions will be discussed in Section~\ref{sec:conclusion} for further research in this direction.
\end{Remark}


%Solution uniqueness to problem \eqref{BP0} and \eqref{Las0} is highly desired for exact and reliable recovery in signal/image processing  \cite{BDE09,F05,FPVDS13,G11,GHS11,NDEG13,T04,T06,VPDF13}. For example, \cite{F05} Fuchs introduced a sufficient condition for solution uniqueness to Lasso \cite{T96}, a particular example of problem \eqref{Las0} such that this unique solution recovers exactly the sign of the signal $x_0$.  In the non-deterministic situation, when $\Phi$ is a Gaussian measurement map, one needs few measurements $m$ to recover the unique solution $x_0$ to problem \eqref{BP0} with high probability \cite{CRPW12,CR09, CR13}. Sufficient conditions for solution uniqueness  is the central tool in this direction. Under some mild assumptions on strict  convexity for the loss function $f$, if $\ox$ is an optimal solution to \eqref{Las0} then  it is unique if and only if it is the unique optimal solution to problem \eqref{BP0}. Uniqueness of optimal solution between  problems \eqref{BP0} and \eqref{Las0} are somewhat equivalent. 

%There are many works of finding necessary and sufficient condition for solution uniqueness to problems \eqref{BP0} and \eqref{Las0}.  Sufficient conditions for this property to Basis Pursuit, a particular case of \eqref{BP0} when $D^*=\Id$ and $\|\cdot\|_\AA=\|\cdot\|_1$ was studied in \cite{BDE09, DH01} by using the {\em spark} and the more computable {\em mutual coherence} of the matrix $\Phi$. In \cite[Theorem~4]{F05} Fuchs introduced another  sufficient condition for this property, which were proved later to be also necessary \cite{GHS11,ZYC13,ZYY16}. Fuchs's condition is precisely the  \cite[Condition~4.3]{GHS11}  including the so-called {\em Strong Source Condition} and {\em Restricted Injectivity}, which were introduced and developed by Grasmair, Haltmeier, and Scherzerto to characterize unique solution to \eqref{BP0}  even  in infinite dimensional space. These conditions are indeed characterizations for robust recovery by using solutions to Lasso \eqref{Las0} to recover the signal $x_0$. There are also many necessary and sufficient conditions for solution uniqueness to Lasso \cite{BLN19,MS19,T04,T06, T13,ZYC13}. 

%With the appearance of linear transformation $D^*$ as in \eqref{BP0}, but $\|\cdot\|_\AA$ being still $\|\cdot\|_1$, Vaiter {\em et al} \cite{VPDF13} introduced the {\em analysis Identifiability Criterion} generalizing the synthesis one from \cite{F05} to have a sufficient condition for solution uniqueness to problem \eqref{Las0}. Another independent sufficient condition was proposed by Nam {\em el al} \cite{NDEG13} by using a generalization of the {\em Null Space Property} \cite{DH01}. Recently, Fuchs's condition is generalized in \cite{ZYY16} by Zhang, Yan, and Yin to characterize this property.  Further results in this direction are also established recently in \cite{G17, MS19} by exploiting the polyhedrality in the  structure of related  regularized problems.  

%When the norm $\|\cdot\|_\AA$ is {\em decomposable} \cite{CR13,NRWY09}, problems \eqref{BP0} and \eqref{Las0} cover three important classes of sparsity,  group sparsity, and low-rank problems corresponding with the choices of the $\ell_1$ norm, the $\ell_1/\ell_2$ norm, and the nuclear norm. For the latter two classes, these norms are not polyhedral. Characterizing their solution uniqueness is more challenging. In \cite[Lemma~1]{CR13}, Cand\`es and Retch generalize Fuchs's condition \cite{F05} to obtain a sufficient condition when $D^*=\Id$. For $\ell_1$ problem, this condition is also necessary. It is natural to question whether Cand\`es and Retch's condition is necessary for solution uniqueness to \eqref{BP0} in the case of decomposable norms. Our Example~\ref{Ex12} and Example~\eqref{Last} provide negative answers for both cases of $\ell_1/\ell_2$ and nuclear norms. The lying reason is that polyhedrality is not present in these two norms. This motivates us to find the answer for the main question of this paper: ``what are characterizations for solution uniqueness to decomposable norm regularized problems?''

%Although Cand\`es and Retch's condition is not necessary for solution uniqueness to \eqref{BP0}, we show that it is indeed a characterization for {\em sharp minima} \cite{C78,P87}, a well-known property that is  stronger than solution uniqueness and plays significant role in complexity and finite convergence of many iterative algorithms. We introduce a quantitative and computable criteria inspired from \cite[Corollary~8]{NDEG13} and \cite[Section~5]{ZYY16} for this property. Our approach  from first-order convex analysis is typical for sharp minima and widely used in previous works about solution uniqueness to problem \eqref{BP0} \cite{CR13,F05,FPVDS13,G17,GHS11,ZYY16}. The proof for sufficiency is standard \cite{CR13}, but our proof for  necessity is more involved. It is worth noticing that  we do not need polyhedrality in the structure of decomposable norms. This distinguishes our results from several one in \cite{G17,MS19,ZYY16} and allows us to work on more general optimization problems. %Furthermore, as discussed above if $\ox$ is a solution to \eqref{Las0}, it is unique if and only if it is a unique solution  to \eqref{BP0}  with $x_0=\ox$. This observation allows \cite{MS19,ZYC13,ZYY16} use the generalized Fuchs's condition to characterize solution uniqueness for both \eqref{BP0} and \eqref{Las0} in the case of $\ell_1$ optimization. Cand\`es and Retch's condition is not characterization for either solution uniqueness or sharp minima for \eqref{Las0} in general. However, we show that if $\ox$ is a sharp solution to \eqref{BP0}, i.e., Cand\`es and Retch's condition holds,   it becomes a {\em strong solution} \cite{BS00, RW98} to \eqref{Las0}. Moreover, if $\ox$ is a strong solution to \eqref{Las0}, it is a strong solution to \eqref{BP0}. These observations  shed the light of using second-order analysis to investigate solution uniqueness for \eqref{Las0}. Correlations between unique/sharp/strong solution to problems \eqref{BP0} and \eqref{Las0} are also studied throughout our paper. 

%The still question is that if it is possible to characterize solution uniqueness to \eqref{BP0}. In the case of group sparsity, we observe that $\ox$ is a unique solution to \eqref{BP0} if and only if it is a strong solution. This observation  sheds the light of using second-order analysis to investigate solution uniqueness for \eqref{Las0}.% The idea of using second-order analysis to  characterize this property for Lasso was  promoted in \cite{BLN19}.     Lasso belongs to the bigger class of convex piecewise linear-quadratic functions whose subdifferentials are polyhedra. The approach in \cite{BLN19} with second order analysis \cite{BS00,RW98} could be extended to investigate solution uniqueness for the latter class, which is also studied recently in \cite{MS19} via different approach. 
% In Section 4,  we establish a quantitative and computable criteria for the unique/strong solution uniqueness to $\ell_1/\ell_2$ problem \eqref{BP0}. This condition is also the characterization of the same property for the corresponding problem \eqref{Las0}.   Our conditions are certainly weaker than several sufficient conditions in \cite{G11,JKL15,RF08}. For nuclear norm regularized problem, we provide several examples showing that a unique solution to \eqref{BP0} or \eqref{Las0} is neither sharp nor strong. It seems that the approach of second-order analysis can only help to find sufficient conditions for  uniqueness of optimal solution to nuclear norm regularized problem. Characterization of solution uniqueness  for this important class remains open.  

%The rest of our paper is follows. Section 2 provides some preliminaries and especially recall first and second subderivatives to characterize sharp and strong solutions. In Section 3, we obtain some characterizations for sharp minima for decomposable norm regularized problem  and discuss the connection of our result with other ones in this direction. Several questions are raised in this section. The first one, which is important in understanding solution uniqueness for decomposable norm regularized problem is:
%\begin{enumerate}[{\bf (Q1)}]
%\item Can a unique solution be sharp to a decomposable norm regularized problem?
%\end{enumerate}
%The answer is Yes for the $\ell_1$ problem, but No for both cases of  the $\ell_1/\ell_2$ norm and the nuclear norm. Moreover, we establish some connection between  unique solutions to \eqref{BP0} and \eqref{Las0}. Particularly, suppose that  $\ox$ is a solution to \eqref{Las0}, we show that if it is a sharp solution to \eqref{BP0} with $x_0=\ox$ then it is a strong solution to \eqref{Las0}; moreover, if it is a strong solution to \eqref{Las0}, it is also strong to \eqref{BP0}. This result raises two questions:

%We have positive answer for {\bf (Q2)} for $\ell_1$ problem, but it turns negative for  both cases of  the $\ell_1/\ell_2$ norm and the nuclear norm.  The answer detailed in Section~4 is Yes for {\bf (Q3)} for group sparsity problem, but No for the other two classes. 

%In Section 4, we notice that the unique solution to $\ell_1/\ell_2$ norm regularized problem is exactly the strong solution. This encourages the use of second-order analysis to characterize solution uniqueness for both \eqref{BP0} and\eqref{Las0}. Our conditions are  quantitative and checkable. The results we obtain here are stronger some from \cite{G11,JKL15,RF08}. The last question we raise in this section is somewhat similar to {\bf (Q1)}:
%\begin{enumerate}[{\bf (Q4)}]end{enumerate}
%The answer is positive for group sparsity problem as discussed above, but negative for the other two classes. All the questions {\bf (Q1)--(Q4)} are supported by theoretical results and many examples throughout the paper. 

%In Section 5, we provide some numerical results of testing solution uniqueness and classifying sharp solution and unique/strong solution to group sparsity problems \eqref{BP0} and \eqref{Las0}. Section 6 gives some conclusion about what we have achieved and some future research on finding better bounds for exact recovery in the non-deterministic situation. We raise the last question about how to characterize solution uniqueness for nuclear norm regularized problems.  It seems that first-order and second-order analysis are not enough to answer this question. 


==> tex_220921/sec_numerics.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Verifying solution uniqueness to group-sparsity problem via numerical methods}
\label{sec:numerics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
With an aim of demonstrating that our conditions for sharp, strong/unique solution are verifiable, we have implemented a simulation using synthetic data. In our simulation study, $\Phi$ was generated as an $(2000\times 240)$ Gaussian matrix whose entries are independently and identically drawn from the standard normal distribution, $N(0,1)$. We next randomly divided the set of indicators range from $1$ to $2000$ into $k=100$ groups of size $20$ with $5$ randomly selected active groups. Then, we constructed a measured signal of length $m=240$, $y_0 \eqdef \Phi x_0$, based on the original signal $x_0$ whose elements in each active group are independently and identically distributed $N(0,1)$. We then used our proposed conditions to verify whether $x_0$ is a solution to \eqref{BP0} using the conditions in Proposition~\ref{Sol} and summarize the number of cases where $x_0$ is classified as sharp or unique/strong solution by the criteria from Theorem~\ref{mtheo} and \ref{BP12}.
For checking strong and sharp minima, we only need to compute the Source Identiy $\rho(e)$ and the Strong Source Identity $\zeta(e)$ whenever $\tau(e)$ in \eqref{xi} or $\gamma(e)$ in \eqref{gamma} is greater than or equal to $1$, respectively, since calculating these numbers are much easier. Similar to the scheme for calculating $\zeta(e)$ in \eqref{zeta2}, $\rho^2(e)$ is the optimal value to  the following smooth convex optimization problem
\begin{equation}\label{rho2}
\Min\quad t\quad \mbox{subject to}\quad ND z=-NDe,\quad \|z_g\|^2\le t, g\in J,\quad \mbox{and}\quad z\in \bigoplus_{g\in J}V_g. 
\end{equation}
Note that \eqref{zeta2} and \eqref{rho2} are second-order cone programming problems and can be solved via function \texttt{solvers.socp} of \texttt{cvxopt} package. In our experiment, $\rho(e)$ or $\zeta(e)$ are calculated when $\tau(e)$ or $\gamma(e)$ is greater than or equal to $0.99$. 


The results are recorded in the following tree diagram: 
\begin{center}
\begin{tikzpicture}[sibling distance=5cm,
  every node/.style = {shape=rectangle, rounded corners,
    draw, align=center,
    top color=white, bottom color=white!20}]]
 \node {$x_0$ is a solution \\$100$ tests}
    child { node {$\Ker\Phi\cap\Ker D^*_{S} =\{0\}$\\ 100 tests} 
        child { node {$\tau(e)<0.99$\\ 11 cases}
           }
        child { node {$\tau(e)\geq 0.99$\\ 89 cases} 
            child { node {$\rho(e)<0.95$\\ 60 cases} }
            child { node {$0.95\leq\rho(e)<1.05$\\29 cases} 
                child { node {$\gamma(e)<0.99$\\ 26 cases} } 
                child { node {$\gamma(e)\geq 0.99$\\ 3 cases} 
                    child { node {$\zeta(e)<0.95$\\ 3 cases} }}}}
    };
\end{tikzpicture}
\end{center}
In all $100$ tested random cases, $x_0$ is verified as a solution to \eqref{BP0} and satisfying the Restricted Injectivity Condition. Among them, there are $11$ cases with $\tau(e)<0.99$ thus are classified as sharp solution, the rest are passed to next step for calculating $\rho(e)$. There are $60$ cases with $\rho<0.95$ and $29$ tests with $0.95<\rho(e)<1.05$. Hence, we had $71$ cases $x_0$ is the sharp solution. We continue the experiment by checking the strong solution condition on the rest $29$ cases. Note that since all cases satisfy the Restricted Injectivity Condition, they automatically satisfy the Strong Restricted Injectivity Condition and it is left to check the Analysis Strong Source Condition. All $29$ cases are indicated as satisfying the Analysis Strong Source Condition with $26$ cases having $\gamma(e)<0.99$ and $3$ cases where $\gamma(e)\geq 0.99$ and $\zeta(e)<0.95$. It means that we have 29 cases of strong solutions that are not sharp. 
\begin{table}[h!]
    \centering
    \begin{tabular}{l c}
    \hline
   & number of cases \\
     \hline

\medspace
Sharp solution & 71 \\

\medspace
Strong solution (non-sharp) & 29\\
\hline

    \end{tabular}
    \caption{Number of cases with strong and sharp solutions}
    \label{tab:strong}
\end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%      & scenario 1 & scenario 2 & scenario 3 \\
%      \hline
% unique solution & 87 & 100 & 100\\
% \hline
% $\Ker\Phi\cap\mathcal{E}\cap\Ker D_{T^{\perp}} =\{0\}$ & 87 & 100 & 100\\ 
% \hline
% $\gamma(e)<0.9$ & 81 & 99 & 100\\
% \hline
% $0.9\leq \gamma(e)<1$ & 6 & 1 & 0 \\
% \hline
% $\gamma(e)\geq 1$ & 0 & 0 & 0\\
% \hline
%     \end{tabular}
%     \caption{Number of cases that have unique solutions}
%     \label{tab:unique}
% \end{table}


==> tex_220921/sec_prelim.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}
\label{sec:prelim}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Throughout the paper, $\R^n$ is the Euclidean space with dimension $n$. In $\R^n$ we denote the inner product by $\dotp{\cdot}{\cdot}$, the Euclidean norm by $\norm{\cdot}$, and the closed ball of radius $r > 0$ centered at $x \in \R^n$ by $\B_r(x)$, and $\Id$ the identity operator.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some linear algebra} 
Given an $m\times n$ matrix $A$, $\Ker A$ (resp. $\Im A$) is the kernel/null (resp. image) space of $A$. The Moore-Penrose generalized inverse \cite[Page~423]{M00} of $A$ is denoted by $A^\dag$, which satisfies the property
\begin{equation}\label{MP1}
AA^\dag A=A.
\end{equation}
Moreover, we have 
\begin{equation}\label{cons}
    \mbox{ $Ax=b$ is consistent if and only if } AA^\dag b=b.  
\end{equation}
In this case, the set of all solutions to equation $Ax=b$ is $A^\dag b+\Ker A$.  If $A$ is injective then $A^\dag=(A^*A)^{-1}A^*$.

Suppose that  $\ox$ is a solution to the consistent system $Ax=b$. The projection of $x\in \R^n$ onto the affine set $C \eqdef A^{-1}b$ is
\begin{equation}\label{Pro}
P_{C}(x)=(\Id-A^\dag A)(x-\ox)+\ox=x- A^\dag A(x-\ox);
\end{equation}
see, e.g., \cite[page~435--437]{M00}. Let $\|\cdot\|_\AA$ and $\|\cdot\|_\BB$ be two arbitrary norms in $\R^m$ and $\R^n$, respectively. The matrix operator norm $\|\cdot\|_{\AA,\BB}: \R^{m \times n} \to \R_+ $  is defined by
\begin{equation*}
\|A\|_{\AA,\BB} \eqdef  \max_{x\in \R^n\setminus\{0\} }\dfrac{\|Ax\|_\AA}{\|x\|_{\BB}}.
\end{equation*}
We write $\|A\|_{2,2}$ for $\|A\|$.  The Frobenius norm of $A$ is known as
\[
\|A\|_F=\sqrt{\Tr(A^*A)}.
\]
Recall that the nuclear norm of $A$ is \[
\|A\|_*=\sum_{k=1}^{\min(m,n)} \sigma_k,
\]
where $\sigma_k$, $1\le k\le \min(m,n)$ are all the singular values of $A$. 
%By the definition, for any $1\leq p, q\leq\infty$, $A\in\R^{m\times n}$ and $x\in \R^n$, one has
%\begin{equation}\label{norm_ineq}
%    \|Ax\|_p\leq \|A\|_{p,q}\|x\|_q.
%\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some convex analysis}
Let $\ph:\R^n \to \oR  \eqdef  \R\cup\{+\infty\}$ be a proper lower semi-continuous (lsc) convex function with domain $\dom \ph \eqdef \enscond{x\in \R^n}{\ph(x)<\infty}$. The subdifferential of $\ph$ at $x\in\dom \ph$ is defined by
\[
\partial \ph(x) \eqdef \enscond{v\in \R^n}{\ph(u) \geq \ph(x) + \dotp{v}{u-x}, \quad \forall u\in \R^n}. 
\]
When $\ph(\cdot)=\iota_C(\cdot)$, the indicator function of a nonempty closed convex set $C$, i.e., $\iota_C(x)=0$ if $x\in C$ and $+\infty$ otherwise, the subdifferential of $\iota_C$ at $x\in C$ is the {\em normal cone} to $C$ at $x$:
\begin{equation}\label{Nor}
N_C(x) \eqdef \enscond{v\in \R^n}{\dotp{v}{u-x} \le 0, \quad \forall u\in C}.
\end{equation}
For a set $\Omega \subset \R^n$, $\cone \Omega$ is its {\em conical hull}. Given a convex cone $K \subset \R^n$, the {\em polar} of $K$ is defined to be the cone
\begin{equation}\label{Pola}
K^\circ \eqdef \enscond{v \in \R^n}{\dotp{v}{u} \le 0, \quad \forall u\in \Omega} .
\end{equation}
It is well known, see \cite[Corollary~6.21]{RW98} that $K^\circ$ is closed and convex, and that 
\begin{equation}\label{Dual}
K^\circ=\cl(K)^\circ \qandq K^{\circ\circ} = (K^\circ)^\circ= \cl (K),
\end{equation}
where$\cl$ denotes the topological {\em closure}. 
The {\em gauge function} of $\Omega$ is  defined by 
\begin{equation}\label{ga}
\gg_\Omega(u) \eqdef \inf\enscond{r>0}{u\in rC}, \qforq u\in \R^n.
\end{equation}
The {\em support function} to $\Omega$ is denoted by
\begin{equation}\label{Sup}
\sigma_\Omega(v) \eqdef \sup_{x\in \Omega}\dotp{v}{x}, \qforq v\in \R^n.
\end{equation}
The {\em polar set} of $\Omega$ is given by
\begin{equation}\label{Polar}
    \Omega^\circ \eqdef \sup\{v\in \R^n|\; \sigma_ C(v)\le 1\}.
\end{equation}
It is well-known that
\begin{equation}\label{PoGa}
\gg_\Omega=\sigma_{\Omega^\circ},
\end{equation}
when $\Omega$ is a nonempty closed convex set; see, e.g., 
\cite[Corollary~15.1.2]{R70}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sharp and strong minima} 
Let us first recall the definition of sharp and strong solutions in \cite{BS00,C78,P87,RW98} that are playing central roles throughout the paper.

\begin{Definition}[Sharp and strong minima] We say $\ox$ to be a sharp solution/minimizer to the (non necessarily convex) function $\ph$ with a constant $c>0$ if there exists $\ve>0$ such that 
\begin{equation}\label{Sha}
    \ph(x) \geq \ph(\ox) + c\norm{x-\ox},\quad \forall x \in  \B_\ve(\ox).
\end{equation}
Moreover, $\ox$ is said to be a strong solution/minimizer with a constant $\kk>0$ if  there exists $\delta>0$ such that 
\begin{equation}\label{Str}
    \ph(x) \geq \ph(\ox) + \frac{\kk}{2}\|x-\ox\|^2,\quad \forall x \in \B_\delta(\ox).
\end{equation}
\end{Definition}
Properties \eqref{Sha} and \eqref{Str} are also known as respectiverly, first order and second order (or quadratic) growth properties.

Strong minima is certainly weaker than sharp minima. Moreover, if $\ox$ is a sharp or strong solution to $\ph$, it is a unique local minimizer to $\ph$ (and the unique minimizer if $\ph$ is convex). When the function $\ph$ is a convex {\em piecewise linear convex}, i.e., its epigraph is a polyhedral,  $\ox$ is a unique solution to $\ph$ if and only if  it is a sharp solution. Furthermore, if $\ph$ is a convex {\em piecewise linear-quadratic} function in the sense that its domain is a union of finitely many polyhedral sets, relative to each of which $\ph$ is a quadratic function, $\ox$ is a strong solution if and only if  it is a unique solution, see, e.g., \cite{BLN19}.

To characterize sharp and strong solutions, it is typical to use directional derivative and second  subderivative; see, e.g., \cite{BS00,RW98}. \JF{In the following, I've insisted on the fact that $\ph$ is convex as otherwise, there are many subtelties to be taken care of for the properties hereafter to hold true.}
%Actually, without convexity, this rather requires $\ph$ to be subdifferentially regular and strictly continuous/locally Lipschitz continuous (see \cite[Theorem~19.6]{RW98}). Think of $|\cdot|^p, p \in ]0,1[$, at the origin}
\begin{Definition}[directional derivative and second subderivatives]\label{DD12}  
Let $\ph:\R^n \to \oR$ be a proper lsc convex function. The directional derivative of $\ph$ at $\ox \in \dom \ph$ is the function $d\ph(\ox):\R^n\to\oR$ defined by
\begin{equation}\label{sub1}
d\ph(\ox)(w) \eqdef \lim_{t\dn 0}\dfrac{\ph(\ox+tw)-\ph(\ox)}{t} \qforq w\in \R^n.
\end{equation}
The second subderivative of $\ph$ at $\ox \in \dom \ph$ for $\ov\in \partial \ph(\ox)$ is the function $d^2 \ph(\ox|\ov):\R^n\to \oR_+$  defined by   
\begin{equation}\label{Subd}
d^2\ph(\ox|\ov)(w) \eqdef \liminf_{t\dn 0, w^\prime \to w}\dfrac{\ph(\ox+tw^\prime)-\ph(\ox)-t\dotp{\ov}{ w^\prime}}{\frac{1}{2}t^2} \qforq w\in \R^n.
\end{equation}
\end{Definition}
It is well-known that $d\ph(\ox)(w)=\max\enscond{\dotp{v}{w}}{v\in \partial \ph(\ox)}$ if $\ph$ is continuous at $\ox$. The calculation of $d^2\ph(\ox|\ov)(w)$ is quite involved in general; see, e.g., \cite{BS00,RW98,MR11}. Note that from \cite[Proposition~13.5 and Proposition~13.20]{RW98}, the function $d^2\ph(\ox|\ov)$ is non-negative, lsc, positively homogeneous of degree 2, and 
\begin{equation}\label{dom2}
\dom d^2\ph(\ox|\ov) \subset \mathcal{K}(\ox|\ov) \eqdef \enscond{w\in \R^n}{d\ph(\ox)(w)=\dotp{\ov}{w}}.
\end{equation}
If, moreover, $\ph$ is twice-differentiable at $\ox$, we have (see \cite[Example~13.8]{RW98})
\begin{equation}\label{smooth}
d^2\ph(\ox|\nabla \ph(\ox))(w)=\dotp{w}{\nabla^2\ph(\ox)w}.
\end{equation}
The following sum rule for second subderivatives will be useful. 
\begin{Lemma}
Let $\ph, \phi:\R^n\to\oR$ be proper lsc convex functions with $\ox\in \dom \ph\cap\dom \phi$. Suppose that $\ph$ is twice differentiable at $\ox\in {\rm int}\,(\dom \ph)$ and $\ov\in \partial (\ph+\phi)(\ox)=\nabla \ph(\ox)+\partial \phi(\ox)$. Then we have
\begin{equation}\label{sum}
d^2(\ph+\phi)(\ox|\ov)(w)=\la w,\nabla^2\ph(\ox)w\ra+d^2\phi(\ox| \ov-\nabla \ph(\ox))(w)\quad \mbox{for all}\quad w\in \R^n.
\end{equation}
\end{Lemma}

\begin{proof}
Use convexity of $\ph,\phi$ and twice-differentiability of $\ph$ at $\ox$ into \cite[Proposition~13.19]{RW98}.
\end{proof}


The next result taken from \cite[Lemma~3, Chapter~5]{P87} and \cite[Theorem~13.24]{RW98} characterize sharp and strong minima.

\begin{Lemma}[Characterization of sharp and strong minima]\label{Fa} 
Let $\ph:\R^n \to \oR$ be a proper lsc convex function with $\ox\in \dom \ph$. We have: 
\begin{enumerate}[label={\rm (\roman*)}]
\item \label{lemFa:item1}
$\ox$ is a sharp minimizer to $\ph$ if and only if there exists $c>0$ such that $d\ph(\ox)(w)\ge c\|w\|$ for all $w\in \R^n$, i.e., $d\ph(\ox)(w)>0$ for all $w\in \R^n\setminus\{0\}$. 
   % \item[{\rm (b)}] There exist $c,\delta>0$ such that ${\rm dist}\,(0,\ph(x))\ge c$ for all $x\in \B_\ve(\ox)\setminus\{\ox\}$ .

\item \label{lemFa:item2}
$\ox$ is a strong minimizer to $\ph$ if and only if $0\in \partial \ph(\ox)$ and there exists $\kk>0$ such that $d^2\ph(\ox|0)(w)\ge \kk\|w\|^2$ for all $w\in \R^n$, which means
\[
\Ker d^2\ph(\ox|0) \eqdef \enscond{w\in\R^n}{d^2\ph(\ox|0)(w)=0}=\{0\}.
\]
\end{enumerate}
\end{Lemma}

It is important to observe that although the sharpness of a minimizer as defined in \eqref{Sha} is a local property, it is actually a global one for convex problems. 
\begin{Lemma}[Global sharp minima]\label{Glo} Suppose that $\ox$ is a sharp solution to the proper lsc convex function $\ph$. Then there exists $c>0$ such that 
\[
\ph(x)-\ph(\ox)\ge c\|x-\ox\|\quad \mbox{for all}\quad x\in \R^n.
\]
\end{Lemma}

\begin{proof} 
Since $\ox$ is a sharp solution to $\ph$, we have from Lemma~\ref{Fa}\ref{lemFa:item1} that $\exists c > 0$ such that $d\ph(\ox)(w)\ge c\|w\|$, $\forall  w\in \R^n$. Thus for any $x\in \R^n$, we have
\[
\ph(x)-\ph(\ox)=\ph(\ox+(x-\ox))-\ph(\ox)\ge \inf_{t>0}\dfrac{\ph(\ox+t(x-\ox))-\ph(\ox)}{t}=d\ph(\ox)(x-\ox)\ge c\|x-\ox\|. 
\]
The proof is complete.
\end{proof}




==> tex_220921/sec_sharp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Quantitative characterizations of sharp minima for convex  minimization problems}
\label{sec:sharp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As in Lemma~\ref{Fa} and Proposition~\ref{Pop},  sharp minima can be characterized via critical cone and descent cone. However, it is not easy to verify them numerically, especially when the dimension is large. In this section, we mainly derive quantitative characterizations for  sharp minima to problem \eqref{BP0}. 


Throughout this section, we suppose that $J_0$ is a non-negative, continuous, and convex function. The following definition taken from \cite[Definition~3.1]{V14} is significant in our study. 
\begin{Definition}[Model Tangent Subspace]\label{MTan} For $u_0=D^*x_0$, we denote the {\em model vector} $e$ by the projection from $0$ to the affine hull of $\partial J_0(u_0)$
\begin{equation}\label{e}
    e \eqdef P_{{\rm aff}\, (\partial J_0(u_0))}(0).
\end{equation}
The {\em model tangent subspace} $T$ of $u_0$ associated to $J_0$ is defined by
\begin{equation}\label{TS}
    T \eqdef S^\perp\quad \mbox{with}\quad S \eqdef  {\rm aff}\, (\partial J_0(u_0))-e.
\end{equation}
\end{Definition}

\begin{Lemma}[Decomposability, {\cite[Theorem~3.4]{V14}}]\label{Decom} Let $u_0\in \R^n\setminus\{0\}$ and $v_0$ be a vector in $\ri \partial J_0({u_0})$. Then 
\begin{equation}\label{Decop}
    \partial J_0(u_0)=\{v\in \R^n|\; P_Tv=e, \gg_{C}(P_S(v-v_0))\le 1\},
\end{equation}
where $C \eqdef  \partial J_0(u_0)-v_0$ and $\gg_C$ is the gauge function of $C$ defined in \eqref{ga}. Moreover $v\in \ri\partial J_0(u_0)$ if and only if $P_Tv=e$ and $\gg_C(P_S(v-v_0))<1$. 
\end{Lemma}


%For $x_0\in \R^n$, we have $\ri (\partial J(x_0))\neq \emptyset$. Pick a vector $v_0\in \ri (\partial J(x_0))$

%As discussed in Introduction part, solution uniqueness to \eqref{BP0} plays an essential role in robust and exact recovery. It could be characterized by using the so-called {\em descent tangent cone} \cite{CRPW12}. Although descent tangent cone is an important notion that is used widely in many papers, it does not have a closed form. More explicit characterizations are desired. In the case of $\ell_1$ problems, solution uniqueness to \eqref{BP0} is characterized via the Restricted Injectivity and Source Condition in \cite{GHS11}. But in $\ell_1$ problem a solution is unique if and only if it is a sharp solution  imply sharp minima. This is the lying reason that many results on robust and exact recovery only need solution uniqueness. For different frameworks, unique solution is distinct from sharp solution. Let us consider the following simple example, which tells that a unique solution to a problem is not a sharp solution, but a strong solution. Indeed, for the case of group sparsity minimization problem, solution uniqueness and strong minima are equivalent;  see further study in our Section~5.






Note from Lemma~\ref{Decom} that   $x_0$ is an optimal solution to problem \eqref{BP0} if and only if there exists $v\in \R^p$ such that $P_Tv=e$, $\gg_C(P_S(v-v_0))\le 1$, and that $Dv\in \Im\Phi^*$.  A quantitative condition is more desirable  for checking optimality. 

\begin{Proposition}[Quantitative characterization for optimality]\label{Sol}  $x_0$ is an optimal solution to problem \eqref{BP0} if and only if the following two conditions are satisfied
\begin{eqnarray}
    &&ND_{S}(ND_{S})^\dag NDe=NDe\quad \mbox{and}\quad  \label{yz}\\
    &&\rho(e) \eqdef \disp \min_{u\in {\rm Ker}\, ND_{S}}\gg_C(-(ND_{S})^\dag NDe-P_Sv_0+u)\le1,  \label{xyz}
\end{eqnarray}
where $N$ is a matrix satisfying $\Ker N=\Im \Phi^*$ and  $D_S \eqdef DP_S$.
\end{Proposition}
\begin{proof} 
To justify the necessity, suppose that $x_0$ is a solution to \eqref{BP0}. Hence there exists $v\in \R^p$ such that $P_Tv=e\in T$, $\gg_{C}(P_S(v-v_0))\le 1$, and $Dv\in \Im \Phi^*=\Ker N$. It follows that $$0=NDv=N(D_Tv+D_{S}v),$$
which implies 
$ND_{S}v=-NDe.$
By \eqref{cons}, we have \[
ND_{S}(ND_{S})^\dag NDe=NDe\quad\mbox{and}\quad P_{S}v\in -(ND_{S})^\dag NDe +\Ker ND_{S}.
\]
This tells us that 
\[
\rho(e)\le \gg_{C}(P_S(v-v_0))\le 1,
\]
which verifies the necessary part. 


To prove the sufficient part, suppose that both \eqref{yz} and \eqref{xyz} hold. Let $u^*_0\in \Ker ND_{S}$ be  a minimizer to the optimization problem in \eqref{xyz} and define
\[\ou \eqdef  -(ND_{S})^\dag NDe+ u^*\quad 
\mbox{with}\quad \gg_C(\ou-P_Sv_0)=\rho(e)\le1.
\]
Since $0\in C$ and $\gg_C(\ou-P_Sv_0)\le 1$, we have $\ou-P_Sv_0\in C\subset S$.  This implies $\ou\in S$. Note further from \eqref{yz} that
\[
ND(e+\ou)=ND(e+P_S\ou)=NDe-ND_{S}(ND_{S})^\dag NDe=0,
\]
which means $D(e+\ou)\in \Im \Phi^*$. Since $\ou\in S$, we get from \eqref{Decop} that  $e+\ou\in \partial J_0(x_0)$ and thus $D(e+\ou)\in \partial J(x_0)\cap \Im \Phi^*$.  Hence $x_0$ is an optimal solution to problem \eqref{BP0}. The proof is complete. 
\end{proof} 


From Lemma~\ref{Decom}, observe that  the condition \eqref{xyz} cannot be dropped out when checking optimality. The equation \eqref{yz} means that the linear system
\[
ND_{S}v=-NDe
\]
is consistent. This condition is also essential. When \eqref{yz} is valid, condition \eqref{xyz} means that there exists $v$ such that $Dv\in \Im \Phi^*$ and $v\in\partial J_0(x_0)$, which closely relates to the so-called Source Condition in \cite{GHS11}. We call $\rho(e)$ the {\em Source Identity}. Under condition \eqref{yz}, $\rho(e)$ is indeed the optimal value to the following condition
\begin{equation*}\label{ro1}
\min\quad \gg_C(-v-P_Sv_0)\quad \mbox{subject to}\quad  ND_Sv=-NDe,
\end{equation*}
which is equivalent to the following convex optimization problem
\begin{equation}\label{ro2}
\min\quad \gg_C(-v-P_Sv_0)\quad \mbox{subject to}\quad  NDv=-NDe\quad \mbox{and}\quad v\in S. 
\end{equation}

\begin{Remark}[Computing the Source Identity $\rho(e)$ for decomposable norms]\label{Deco}{\rm One important class of regularizers is $J(x)=\|D^*x\|_\AA$, where $J_0(\cdot)=\|\cdot\|_\AA$ is a {\em decomposable} norm in $\R^p$. The class of decomposable norms is introduced in  \cite{NRWY09} including the $\ell_1$ norm, the $\ell_1/\ell_2$ norm, and the nuclear norm.  According to \cite{CR13}, a norm $\|\cdot\|_\mathcal{A}$ is called to be decomposable at $u_0 \eqdef D^*x_0$ if there is a subspace $V\subset \R^p$ and a vector $e_0\in V$ such that
\begin{equation}\label{subA}
    \partial \|u_0\|_{\mathcal{A}}=\left\{z\in \R^p|\; P_{V}z=e_0\quad \mbox{and}\quad \|P_{V^\perp}z\|^*_{\mathcal{A}}\le 1\right\},
\end{equation}
where $\|\cdot\|^*_\AA$ is the dual norm to $\|\cdot\|_\AA$. Define $v_0 \eqdef e_0\in \partial J_0(u_0)=\partial\|u_0\|_\AA$, we get from \eqref{subA} that $C=\partial J_0(u_0)-v_0=\{z\in V^\perp|\; \|z\|^*_\AA\le 1\}$ and that 
$
S={\rm aff}\, (\partial J_0(u_0))-v_0={V^\perp}$. 
This tells us that  $T=V$ and $e_0=e$ in the sense of Definition~\ref{MTan}. In this case, for any $z\in S$ we have 
\[
\gg_C(z)= \inf\left\{r>0|\; \left\|\dfrac{z}{r}\right\|^*_\AA\le 1\right\}=\|z\|^*_\AA.
\]
Hence optimization problem \eqref{ro2} turns to 
\begin{equation}\label{rhoz}
    \Min\quad \|z\|^*_\AA\quad\mbox{subject to}\quad NDz=-NDe\quad \mbox{and}\quad z\in S.
\end{equation}
The matrix $N$ can be chosen from the singular value decomposition of $\Phi=U\Sigma V^*$ as the submatrix  $V_G$ of $V$, where $G$ is the index set of $\{r+1, r+2, \ldots, n\}$ with $r={\rm rank}\, \Phi$. This idea is slightly inspired from \cite{NDEG13,ZYY16} for the case of $\ell_1$ norm. Our Section~6 will discuss further about using Source Identity  to classify sharp solutions and strong/unique solutions to group-sparsity problems. 
}
\end{Remark}


Next, we establish the main result in this section by providing several  characterizations of  sharp minima. 

\begin{Theorem}[Characterizations for sharp solution]\label{mtheo} The following statements  are equivalent:
\begin{enumerate}[label={\rm (\roman*)}]
\item $x_0$ is a sharp  solution to problem \eqref{BP0}.

\item The {\em Restricted Injectivity} holds at $x_0$ in the sense that \begin{equation}\label{GIR}
    \Ker \Phi\cap \Ker D^*_S=\{0\}
\end{equation}  
and  the {\em Source Identity} $\rho(e)$ is less than $1$.  

\item The Restricted Injectivity holds at $x_0$ and the {\em Strong Source Condition} is satisfied at $x_0$ in the sense that  there exists  $v\in \R^p$ such that $Dv\in \Im \Phi^*$ and $v\in \ri \partial J_0(x_0)$.

\end{enumerate}
Moreover, if {\rm (ii)} is satisfied, the sharp constant $c$ at $x_0$ can be chosen as
\begin{equation}\label{ShaCo}
    c=(1-\rho(e))sc_1\quad \mbox{with}\quad  c_1 \eqdef \min_{w\in {\rm Ker}\,\Phi\cap \mathbb{S}^{n-1}}\|D^*_{S}w\|>0
\end{equation}
and $s>0$ satisfying $\B_s(0)\cap S\subset C$. 
\end{Theorem}
\begin{proof} 
Let us start with the implication [(i)$\Rightarrow$(ii)]. Suppose that $x_0$ is a sharp solution to \eqref{BP0}. Hence there exists some $c>0$ such that $d\Psi(x_0)(w)\ge c\|w\|$ for all $w\in \R^n$.  Note from Lemma~\ref{Decom} that 
\begin{eqnarray}\label{dPhi}\begin{array}{ll}
    d\Psi(x_0)(w)&=dJ(x_0)(w)+\iota_{{\rm Ker}\, \Phi}(w)\\
    &=\sup\{\la Dv,w\ra|\; P_Tv=e, P_Sv\in P_Sv_0+ C\}+\iota_{{\rm Ker}\, \Phi}(w)\\
    &=\sup\{\la D_Tv+D_Sv,w\ra|\; P_Tv=e, P_Sv\in P_Sv_0+ C\}+\iota_{{\rm Ker}\, \Phi}(w)\\
    &=\la e,D^*_Tw\ra+\la P_Sv_0,D^*_S w\ra+\sup\{\la z,D^*_Sw\ra|\; z\in C\}+\iota_{{\rm Ker} \Phi}(w)\\
    &=\la e, D^*_Tw\ra+\la P_{S}v_0,D^*_Sw\ra+\sigma_C(D^*_Sw)+\iota_{{\rm Ker} \Phi}(w),
    \end{array}
\end{eqnarray}
where $\sigma_C$ is the support function of $C$ defined in \eqref{Sup}.


For any $w=N^*u\in \Ker\Phi$, we obtain from \eqref{dPhi}, \eqref{yz}, and the inequality $d\Psi(x_0)(w)\ge c\|w\|$ that  
\begin{eqnarray}\label{Tes}\begin{array}{ll}
    \sigma_C(D^*_Sw)-c\|w\|&\ge -\la e, D^*_TN^*u\ra-\la P_Sv_0,D^*_SN^*u\ra\\
    &=-\la NDe,u\ra-\la P_Sv_0,D^*_SN^*u\ra\\
    &=-\la ND_S(ND_S)^\dag NDe,u\ra-\la P_Sv_0,D^*_SN^*u\ra\quad (\mbox{by } \eqref{yz})\\
    &=-\la (ND_S)^\dag NDe,D^*_SN^*u\ra-\la P_Sv_0,D^*_SN^*u\ra
    \end{array}
\end{eqnarray}
If $w\in \Ker\Phi\cap \Ker D^*_S$, the latter tells us that $-c\|w\|\ge 0$, which means $w=0$. Thus the Restricted Injectivity \eqref{GIR} is satisfied. 

Moreover, since $J_0$ is a continuous convex function, $\partial J_0(u_0)$ is bounded, so is $C$. It follows that 
\[
\sigma_C(D_S^*w)\le r\|D^*_Sw\|\le r\|D^*_S\|\|w\|\quad \mbox{with}\quad r \eqdef \max\{\|z\||\; z\in C\}.
\]
Combining the latter with \eqref{Tes} tells us that
\begin{equation}\label{gau}
     \left(1-\frac{c}{r\|D^*_S\|}\right)\sigma_C(D^*_SN^*u)\ge -\la (ND_S)^\dag NDe+ P_Sv_0,D^*_SN^*u\ra.
\end{equation}
Let $C^\circ$ be the polar set of $C$ as in  \eqref{Polar} and define $K \eqdef C^\circ\cap S$. Since $0\in \ri C$, there exists $s>0$ such that and $\B_s(0)\cap S\subset C$. For any $v\in K\setminus\{0\}$, we have $s\frac{v}{\|v\|}\in \B_s(0)\cap S$ and thus $\la v,  s\frac{v}{\|v\|}\ra\le \sigma_C(v)\le 1$. It follows that $\|v\|\le \frac{1}{s}$. Hence, $K$ is a compact set. 

By the classical minimax theorem, e.g., \cite[Corollary~37.3.2]{R70}, we obtain from \eqref{gau} that   
\begin{eqnarray}\label{Mimax}\begin{array}{ll}
1-\dfrac{c}{r\|D^*_S\|}&\disp\ge \sup_{v\in K}\la-(ND_S)^\dag NDe-P_Sv_0,v\ra -\iota_{{\rm Im}\, D^*_SN^*}(v)  \\
&=\disp\sup_{v\in K}\inf_{u\in {\rm Ker}\, N D_S} \la-(ND_S)^\dag NDe-P_Sv_0+u,v\ra\\
&=\disp \min_{u\in {\rm Ker}\, ND_S}\sup_{v\in K} \la-(ND_S)^\dag NDe-P_Sv_0+u,v\ra\\
&=\disp \min_{u\in {\rm Ker}\, N D_S}\sigma_{K} (-(ND_S)^\dag NDe-P_Sv_0+u).
\end{array}
\end{eqnarray}
Let $u^*\in \Ker N D_S$ be a minimizer to the optimization problem above. As $K\subset S$, we have 
\[
\sigma_K (-(ND_S)^\dag NDe-P_Sv_0+u^*)=\sup_{v\in K} \la-P_S((ND_S)^\dag NDe+P_Sv_0-u^*),v\ra.
\]
Note further that $C^\circ=T+ K$, we have
\[
\sup_{v\in K} \la-P_S((ND_S)^\dag NDe+P_Sv_0-u^*),v\ra=\sup_{v\in C^\circ} \la-P_S((ND_S)^\dag NDe+P_Sv_0-u^*),v\ra.
\]
It follows that 
\begin{equation}\label{mnx1}
\sigma_K (-(ND_S)^\dag NDe-P_Sv_0+u^*)=\sigma_{C^\circ}(-P_S((ND_S)^\dag NDe+P_Sv_0-u^*)).
\end{equation}
Since the Restricted Injectivity holds at $x_0$, we have  \[
(ND_S)^\dag=D^*_SN^*(ND_S(ND_S)^*)^{-1}=P_SD^*N^*(ND_S(ND_S)^*)^{-1},
\]
which implies    $P_S(ND_S)^\dag=(ND_S)^\dag$. Moreover, $P_Su^*\in \Ker ND_S$. We obtain that
\[
\sigma_{C^\circ}(-P_S((ND_S)^\dag NDe+P_Sv_0-u^*))\ge \min_{y\in {\rm Ker}\, N D_S}\sigma_{C^\circ} (-(ND_S)^\dag NDe-P_Sv_0+y).
\]
Combining this with \eqref{mnx1} and \eqref{Mimax} gives us that 
\begin{eqnarray*}\begin{array}{ll}
1-\dfrac{c}{r\|D^*_S\|}&\ge\disp \min_{y\in {\rm Ker}\, N D_S}\sigma_{C^\circ} (-(ND_S)^\dag NDe-P_Sv_0+y)\\
&\disp =\min_{y\in {\rm Ker}\, N D_S}\gg_C (-(ND_S)^\dag NDe-P_Sv_0+y),
\end{array}
\end{eqnarray*}
where the equality follows from \eqref{PoGa}. This verifies (ii).


Next, let us justify the implication [(ii)$\Rightarrow$(iii)]. Suppose that (ii) is satisfied and choose $u^*$ as a minimizer of the optimization problem in \eqref{xyz}. We have $\gg_{C}(-(ND_S)^\dag NDe-P_Sv_0+u^*)<1.$ Since the Restricted Injectivity holds, we have $\Ker N D_S=\{0\}$ and thus 
\begin{equation*}
ND_S(ND_S)^\dag NDe= ND_S (ND_S)^*(ND_S(ND_S)^*)^{-1}NDe=NDe,
\end{equation*}
which verifies \eqref{yz}. It is similar to the proof for the sufficient part in Proposition~\ref{Sol} that
\[
D(e-(ND_S)^\dag NDe+u^*)\in \Im \Phi^*\quad \mbox{and}\quad e-N_S^\dag N_Te+u^*\in \ri \partial J(x_0)
\]
by Lemma~\ref{Decom}. This ensures (iii).


Finally, we prove [(iii)$\Rightarrow$(i)]. Suppose that the Restricted Injectivity \eqref{GIR} holds at $x_0$ and there exists  $Dv\in \Im\Phi^*$ and $v\in \ri \partial J(x_0)$. Hence, we have $P_Tv=e$ and $\gg_{C}(P_S(v-v_0))<1$. For any $w\in \Ker \Phi$, note from \eqref{dPhi} that 
\begin{eqnarray}\label{lower}\begin{array}{ll}
d\Psi(x_0)(w)&=\la e, D^*w\ra+\la P_Sv_0,D^*_Sw\ra+\sigma_C(D^*_Sw)\\
&=\la v-P_Sv,D^* w\ra+\la P_Sv_0,D^*_Sw\ra+\sigma_C(D^*_Sw)\\
&=\la-P_Sv, D^*w\ra+\la P_Sv_0,D^*_Sw\ra+\sigma_C(D^*_Sw)\\
&=\la-P_S(v-v_0), D^*_Sw\ra+\sigma_C(P_Sw)\\
&\ge -\sigma_{C}(D^*_Sw)\gg_{C}(P_S(v-v_0))+\sigma_C(D^*_Sw)\\
&=[1-\gg_{C}(P_S(v-v_0))]\sigma_C(D^*_Sw).
\end{array}
\end{eqnarray}
Recall that $0\in \ri C$ and $\B_s(0)\cap S\subset C$. As $D^*_Sw\in S$, we have 
\[
\sigma_C(D^*_Sw)\ge \la D^*_Sw,s\frac{D^*_Sw}{\|D^*_Sw\|}\ra= s\|D^*_Sw\|\ge sc_1\|w\|
\]
with $c_1 \eqdef \min\{\|D^*_Sw\||\; \|w\|=1, w\in \Ker\Phi\}$, which is positive due to the Restricted Injectivity \eqref{GIR}. We derive from \eqref{lower} that
\[
d\Psi(x_0)(w)\ge [1-\gg_{C}(P_S(v-v_0))]sc_1\|w\|\quad \mbox{for all}\quad w\in \Ker \Phi,
\]
which verifies (i). According to \eqref{ro2},  the above inequality  tells us that the sharp constant of $\Psi$ satisfies \eqref{ShaCo}. The proof is complete.  
\end{proof} 
 


\begin{Remark}{\rm 
The Restricted Injectivity \eqref{GIR} appeared in \cite{V14} generalizes the one with the same name for $\ell_1$ problem in \cite{GHS11}. It also has tracks in some special cases, e.g., for the $\ell_1$ norm problems \cite{F05, G17,GHS11,NDEG13,VPDF13,ZYC15, ZYY16}, $\ell_1/\ell_2$ norm problems \cite{G11,JKL15}, and nuclear norm problems \cite{CRPW12, CR09,CR13}. 

The format of Strong Source Condition in Theorem \ref{mtheo} is taken from \cite{V14}. It  generalizes the condition in \cite{GHS11} for $\ell_1$ problem, which actually occurred earlier in  \cite{CT04,F05}. The combination of Restricted Injectivity and Strong Source Condition in the above result are proved in \cite[Theorem~5.3]{V14} as sufficient conditions for  solution uniqueness to problem \eqref{BP0}, but they are not necessary. By revisiting  Example~\ref{Ex12}, we see that $x_0$ is a unique solution to problem \eqref{Ex123} but the Strong Source Condition is not satisfied. Indeed, for any $z\in \R^2$ satisfying $\Phi^*z=(v_1+v_2,v_1,-v_2)^T\in \partial J(x_0)=\{(0,1)\}\times[-1,1]$, we have $z=(1,-1)$ and $\Phi^*z = (0,1,1)\notin \mathrm{ri}\, \partial J(x_0)
$.


Theorem~\ref{mtheo} strengthens \cite[Corollary~1]{VGFP15} by showing that  Restricted Injectivity and Strong Source Condition are necessary and sufficient for sharp minima.  In the case of $\ell_1$ problem, it recovers  part of \cite[Theorem~2.1]{ZYY16} that gives  a characterization for solution uniqueness, which is equivalent to sharp minima in this framework. Some other characterizations are also studied recently in \cite{G17,MS19} by exploiting polyhedral structures. It is worth emphasizing that our result does not need polyhedrality. The proof mainly  relies on the well-known first-order condition in Lemma~\ref{Fa} for sharp minima, the decomposiability \eqref{Decop}, and the classical minimax theorem. Theorem~\ref{mtheo} also covers many results about solution uniqueness in \cite{CRPW12, CR09,CR13, CT04, F05, G11, G17,GHS11, JKL15, NDEG13,RF08, VPDF13, T04, T06, ZYC15, ZYY16}.
}
\end{Remark}


%By Proposition~\ref{Sol}, $x_0$ is an optimal solution to problem \eqref{BP0}.  It suffices to show that $d \Psi(x_0;w)\ge \hat c\|w\|$ for any $w\in \Ker \Phi=\Im N^*$ with some constant $\hat c>0$ due to Fact~\ref{Fa}. Indeed, for any $u\in \R^r$ we get from \eqref{equ} and \eqref{mima} that
%\begin{eqnarray}\label{inq2}
%\begin{array}{ll}
%d\Psi(x_0;N^*u)&=\la ND_{S}(ND_{S})^\dag NDe,D^*_{S}N^*u\ra+\|D^*_{S}N^*u\|_\AA\\
%&\ge -\rho(e)\|D^*_{S}N^*u\|+\|D^*_{S}N^*u\|_\AA. 
%\end{array}
%\end{eqnarray}
%Since $\Ker D^*_{S}N^*=\{0\}$, there exists some constant $\al >0 $ such that $$\|D^*_{S}N^*u\|_\AA\ge \al\|u\|\ge\frac{\al}{\|N^*\|_{2,2}}\|N^*u\| \quad \mbox{for all}\quad u\in \R^r.$$
%This together with \eqref{inq2} tells us that 
%\[
%d\Psi(x_0;N^*u)\ge \frac{\al(1-\rho(e))}{\|N^*\|_{2,2}}\|N^*u\|\quad \mbox{ for all}\quad u\in \R^r,
%\]
%which verifies $d\Psi(x_0;w)\ge \hat c\|w\|$ for any $w\in \Ker \Phi$ with $\hat c \eqdef \frac{\al(1-\rho(e))}{\|N^*\|_{2,2}}>0$. The proof is completed. \end{proof} 


The idea of using first-order analysis to study solution uniqueness to norm regularized optimization problem is not new \cite{CRPW12, CR09,CR13,F05,FPVDS13,GHS11,ZYY16}.  From the calculation in \eqref{dPhi} and Lemma~\ref{Fa}, sharp minima at $x_0$ can be characterized by the {\em Strong Null Space Property} \cite{FPVDS13,V14}:
\begin{equation}\label{SNS}
-\la e, D_T^*w\ra-\la P_Sv_0,D^*_Sw\ra<\gg_C(D^*_{S}w)\quad \mbox{for all}\quad w\in \Ker \Phi\setminus\{0\},
\end{equation}
which is a generalization of the same property for $\ell_1$ regularization \cite{DH01,NDEG13}.
However, our condition in (ii) is more quantitative and could be tested numerically; see Section~6. %Indeed, Proposition~\ref{Sol} suggests the way to compute $\rho(e)$ as the optimal value to
 


\begin{Corollary}[Sufficient condition for sharp solution] If the Restricted Injectivity holds at $x_0$ and the following condition
\begin{equation}\label{xi}
\tau(e) \eqdef \gg_C(-(ND_{S})^\dag NDe-P_Sv_0)<1
\end{equation}
is satisfied, then $x_0$ is a sharp solution to problem \eqref{BP0}.
\end{Corollary}
\begin{proof} 
It is easy to see that $\tau(e)\ge \rho(e)$. The result follows from Theorem~\ref{mtheo}. 
\end{proof} 


%The appearance of Corollary~\eqref{mcor} is also obtained by Zhang, Yan, and Yin  \cite{ZYY16} for a special case of $\ell_1$-norm $\|\cdot\|_\AA=\|\cdot\|_1$. For this case the function $\Psi(x)=\|x\|_1+\iota_{\Phi^{-1}b}(x)$ is a polyhedral convex function. It is well-known that sharp minimizer is equivalent to the uniqueness of optimal solution in the latter situation.  Uniqueness of optimal solution to polyhedral optimization is also studied in \cite{G17,MS19} by exploiting the polyhedral structure and linear programming; see also \cite{ZYY16}.  It is worth noting here that our problem \eqref{BP0} may cover the nonpolyhedral case, e.g., when $\|\cdot\|_\AA$ is the nuclear norm. 

%\begin{Corollary}[Existence characterization for sharp minimizer]\label{mcor} Let $x_0$ satisfy $\Phi x_0=b$. Suppose that $\|\cdot\|_\AA$ is decomposable at $D^*x_0$. Then $x_0$ is a sharp minimizer to problem \eqref{BP0} if and only if 
%\begin{enumerate}[label={\rm (\roman*)}]
%\item $\Ker \Phi\cap \Ker D^*_{S}=\{0\}$,
%\item There exists some $z\in \R^n$ such that $Dz\in \Im \Phi^*$, $P_Tz=e$, and $\|P_{S}z\|^*_\AA<1$.  
%\end{enumerate}
%\end{Corollary}
%{\bf Proof.} Due to Theorem~\ref{mtheo}, it suffices to show that (ii) is equivalent to condition $\rho(e)<1$ provided that $\Ker \Phi\cap \Ker D^*_{S}=\{0\}$. Suppose that there exists $z$ satisfies all the condition in (ii) and define $v \eqdef P_{S}z$. We have $z=e+v$ and $D(e+v)\in \Im \Phi^*$, i.e., $ND_{S}v=-NDe$. It follows that $v\in -(ND_{S})^\dag NDe+\Ker ND_{S}$. Thus $\rho(e)\le \|v\|_\AA<1$.

%Conversely, if $\rho(e)\le \|v\|_\AA<1$, we find some $\ou\in -(ND_{S})^\dag NDe+\Ker ND_{S}$ such that $\|\ou\|_{\AA}<1$. Since $\Ker D^*_{S}N^*=\{0\}$ due to condition (i), we have $ND_{S} \ou=-NDe$. It is similar to the  second part of the proof 
%that $z \eqdef e+P_{S}\ou$ satisfies all the conditions in (ii). The proof is completed. \end{proof} 


%In the case $D^*=\Id$, conditions (i) and (ii) are used as sufficient conditions for the uniqueness of optimal solution to \eqref{BP0} in \cite[Lemma~1]{CR13}. Our result above shows further that they are indeed characterizations for sharp minimizer for the more general problem \eqref{BP0}. This  certainly covers \cite[Lemma~1]{CR13}. Corollary~\ref{mcor} also suggests the way to compute $\rho(e)$ as the optimal value to
%\begin{equation}
  %  \Min\quad \|P_{S} y\|^*_\AA\quad\mbox{subject to}\quad ND_{T}y=-NDe. 
%\end{equation}
%The appearance of Corollary~\eqref{mcor} is also obtained by Zhang, Yan, and Yin  \cite{ZYY16} for a special case of $\ell_1$-norm $\|\cdot\|_\AA=\|\cdot\|_1$. For this case the function $\Psi(x)=\|x\|_1+\iota_{\Phi^{-1}b}(x)$ is a polyhedral convex function. It is well-known that sharp minimizer is equivalent to the uniqueness of optimal solution in the latter situation.  Uniqueness of optimal solution to polyhedral optimization is also studied in \cite{G17,MS19} by exploiting the polyhedral structure and linear programming; see also \cite{ZYY16}.  It is worth noting here that our problem \eqref{BP0} may cover the nonpolyhedral case, e.g., when $\|\cdot\|_\AA$ is the nuclear norm. 




When $\|\cdot\|_\AA=\|\cdot\|_1$, the ``unit'' vector $e$ in \eqref{e} is indeed $(\sign(D_I^*x_0),0_J)^*$, where $I \eqdef {\rm supp}\, (D^*x_0) \eqdef \{i\in\{1,2, \ldots,p\}|\; (D^*x_0)_i\neq 0\}$, $K \eqdef \{1, \ldots, p\}\setminus I$,  and $D_I$ is the submatrix of $D$ with column indices  $I$. Inequality \eqref{xi} is written as
\[
{\tau}(\sign(D^*_Ix_0))=\|(ND_{K})^\dag ND_I\sign(D^*_Ix_0)\|_\infty<1,
\]
which is called the {\em Analysis Exact Recovery Condition} in \cite{NDEG13}. 



Another identity used  in  \cite{VPDF13} to check solution uniqueness for $\ell_1$ problem is the so-called {\em Analysis Identifiability Criteria} at $\sign(D^*_Ix_0)$ denoted by
\begin{equation}\label{IC}
{\bf IC}(\sign(D^*_Ix_0)) \eqdef \min_{v\in {\rm Ker}\, D_{J}} \|D_{K}^\dag(\Phi^*(\Phi^\dag_U)^*U^*-\Id)D_I \sign(D^*_Ix_0)-v\|_\infty<1,
\end{equation} 
where $U$ is basis of $\Ker D_{J}^*$ and $\Phi_U \eqdef \Phi U$. This condition reduces to the synthesis one introduced by Fuchs \cite{F05} in the case of $D^*=\Id$.  As discussed in \cite{NDEG13,VPDF13}, $\tau(\sign(D^*_Ix_0))$ and ${\bf IC}(\sign(D^*_Ix_0))$ are independent even for the case $D=\Id$. 

For our general framework \eqref{BP0} with constants in Definition~\ref{MTan}, the Analysis Identifiability Criteria is said to satisfy at $x_0$ if 
\begin{equation}\label{AIC}
{\bf IC}(e) \eqdef \min_{u\in {\rm Ker}\, D_S} \gg_C(D_S^\dag(\Phi^*(\Phi^\dag_U)^*U^*-\Id)De-P_Sv_0+u)<1,
\end{equation} 
where $U$ is a matrix whose columns form a basis of $\Ker D^*_S$ and $\Phi_U \eqdef \Phi U.$



\begin{Proposition}\label{comp} If the Restricted Injectivity holds at $x_0$ then $\rho(e)\le {\bf IC}(e)$. Consequently, if the Analysis Identifiability Criteria holds at $x_0$, then $x_0$ is a sharp solution to \eqref{BP0}.
\end{Proposition}
\begin{proof} 
 Now suppose that $\Ker \Phi\cap \Ker D^*_S=\{0\}$, which means $\Ker \Phi_U=0$ and $\Phi_U^\dag=(\Phi_U^*\Phi_U)^{-1}\Phi_U^*$. Let $\ou\in\Ker D_S$ be a minimizer to the optimization problem in ${\bf IC}(e)$ and  and define   \[
\ov \eqdef  D_S^\dag(\Phi^*(\Phi^\dag_U)^*U^*-\Id)De+ \ou\quad \mbox{with}\quad \gg_C(\ov-P_Sv_0)={\bf IC}(e).
\] 
Note that 
 \[
 U^*(\Phi^*(\Phi^\dag_U)^*U^*-\Id)De=(\Phi_U^*\Phi_U(\Phi_U^*\Phi_U)^{-1}U^*-U^*)De=0.
 \]
It follows that $(\Phi^*(\Phi^\dag_U)^*U^*-\Id)De\in \Im D_S,$ which tells us that $D_S\ov=(\Phi^*(\Phi^\dag_U)^*U^*-\Id)De$ by \eqref{cons}. Hence we have 
\begin{equation}\label{Nd}
ND_S\ov=(N\Phi^*(\Phi^\dag_U)^*U^*-N)De=-NDe,
\end{equation}
which implies that $\ov\in -(ND_S)^\dag NDe+\Ker ND_S$ and thus $\rho(e)\le \gg_C(\ov-P_Sv_0)={\bf IC}(e)$. When the Analysis Identifiability Criteria is satisfied at $x_0$, we have $\rho(e)\le {\bf IC}(e)< 1$ and thus $x_0$ is a sharp minima to \eqref{BP0} due to Theorem~\ref{mtheo}. The proof is complete. 
\end{proof} 


Proposition~\ref{comp}  tells us that Theorem~\ref{mtheo} is strictly stronger than \cite[Theorem~2]{VPDF13} for the case of $\ell_1$ problem. It also covers the \cite[Proposition~5.7]{V14}. For the case of $\ell_1$ problem,  \cite{ZYY16} provides an example that $\rho(\sign(D^*_Ix_0))$ is  strictly smaller than both $\tau(\sign(D^*_Ix_0))$ and ${\bf IC}(\sign(D^*_Ix_0))$. %Moreover, by defining $\ov \eqdef (s_0, \ov_J)$, we get from \eqref{Nd} that $D\oy\in \Im \Phi^*$. Hence the Analysis Identifiability Criteria at $s_0$ means that $\oy\in {\rm ri}\,\partial \|D^*x_0\|_1 $, which means that 
%\begin{equation*}\label{NonD}
%D\ov\in {\rm ri}\, \partial J(x_0)\quad \mbox{with}\quad J(x)=\|D^*x\|_1,
%\end{equation*}
%which is known as the {\em non-degenerate} condition. It together with the Restricted Injectivity Condition has been used  in \cite{V14,VPF15} to prove robust recovery for more general convex regularizers $J(x)$ in \eqref{BP0}. However, this non-degenerate condition is nontrivial even for the case of $\ell_1$ norms.   




The following result is a direct consequence of Theorem~\ref{Rob} and Theorem~\ref{mtheo} about robust recovery. The bound for $\mathcal{O}(\delta)$ can be derived from \eqref{ShaCo}. It covers parts of  \cite[Theorem~2]{FPVDS13}, \cite[Theorem~4.2]{GHS11}, and \cite[Theorem~2]{ZYY16} for the case of $\ell_1$ minimization problems.

\begin{Corollary}[Robust recovery of decomposable norm minimization]\label{Corode} Suppose that $J_0$ is a nonegative continuous convex function satisfying 
\begin{equation}\label{AC2}
    (D^*)^{-1}(\Ker (J_0)_\infty)\cap\Ker \Phi=\{0\}.
\end{equation}
If the Restricted Condition and Strong Source Condition holds at $x_0$, we have linear rate for robust recovery as in \eqref{Est2} and \eqref{Est}. 
\end{Corollary}
\begin{proof} 
 Note from \cite[Proposition~2.6.3]{AT03} $J_\infty(w)=(J_0)_\infty(D^*w)$ for any $w\in \R^n$. Hence, condition \eqref{AC2} is exactly \eqref{AC}. We obtain the robust recovery with linear  rate as in \eqref{Est2} and \eqref{Est} due to Theorem~\ref{mtheo} and Theorem~\ref{RobCon}. \end{proof} 


%If $J(x)=\|D^*x\|_\AA$, by Theorem~\ref{mtheo}, $x_0$ is the unique solution to \eqref{BP0}. By the discussion in Remark~\ref{Relax}, condition \eqref{AC} is satisfied. The proof is complete. \end{proof} 


In the case $D^*=\Id$, Corollary~\ref{Corode} recovers \cite[Theorem~6.1]{V14}. When $J(x)=\|D^*x\|_\AA$, it covers many results  in \cite{CRPW12,FPVDS13, GHS11, V14, VPF15, ZYY16} about robust recovery. If additionally, $\|\cdot\|_\AA$ is decomposable, the constant $s$ in  \eqref{ShaCo} can be chosen as $1$ and  $v_0=e_0$. This together with Theorem~\ref{Rob} allows us to obtain explicit bounds for robust recovery with linear rate.


%One natural question arising from Corollary~\ref{ell1} is: 
%\begin{enumerate}[{\bf (Q1)}]
%\item Can a unique solution be sharp to a 
%decomposable norm regularized problem?
%\end{enumerate}
%Except for the case of $\ell_1$ norm as discussed in Corollary~\ref{ell1}, we have negative answers for both group sparsity and low-rank problems; see our Example~\ref{Last3}, Example~\ref{Ex12}, and Example~\ref{Last}. However,  the next section shows  that a unique solution to $\ell_1/\ell_2$ problem  is indeed the strong solution. %For nuclear norm problem, the answer for {\bf (Q1)} is negative too. Particularly,  Example~\ref{Last} shows that $x_0$ is a unique solution to \eqref{BP0}, but it is neither  strong nor  sharp. 

When there is noise in observation \eqref{yw}, problem \eqref{Las3} is usually used to recover the original signal $x_0$. Solution uniqueness to \eqref{Las3} is especially important in the area of exact recovery \cite{F05,VPDF13}. We show next that Restricted Injectivity and Strong Source Condition are sufficient  for strong minima to problem \eqref{Las3}; moreover, they become necessary in the case of  $\ell_1$ problems. This result is true for a larger class of norm regularized problems  
\begin{equation}\label{Las0}
    \min_{x\in \R^n}\quad \Theta(x) \eqdef f(\Phi x)+\mu J(x),
\end{equation}
where $\mu$ is a positive constant and the loss function $f:\R^m\to \oR$ is an extended real-valued convex function satisfying the following two conditions:
\begin{enumerate}[label={\rm (\Alph*)}]
    \item $f$ is twice continuously  differentiable in ${\rm int}\,(\dom f)$.
    \item $\nabla f^2(x)$ is positive definite for all $x\in {\rm int}\,(\dom f)$, i.e., $f$ is strictly convex in the interior of its domain. 
\end{enumerate}
In \eqref{Las3}, the function $f$ is $\frac{1}{2}\|\cdot-y\|^2$ that certainly satisfies the above two conditions. Moreover, the standing assumptions (A) and (B) for $f$ cover an important class of  Kullback-Leiber divergence:
\begin{eqnarray}\label{KL}
f_{\rm KL}(z)=\left\{\begin{array}{ll} \disp\sum_{i=1}^my_i\log\dfrac{y_i}{z_i}+z_i-y_i\quad &\mbox{if}\quad z\in \R^m_{++}\\
 +\infty \quad &\mbox{if}\quad z\in \R^m_+\setminus\R^m_{++},\end{array}\right.
\end{eqnarray}
which is broadly used in statistical/machine learning as an estimation of the dissimilarity between two distributions or the loss information when using prior distribution to approximate the posterior.

In the following result, we provide the connection of unique/sharp/strong solutions between two problems \eqref{BP0} and \eqref{Las0}. Part (i) of this result could be obtained from \cite[Proposition~3.2]{MS19}, but we still give  a short proof as our assumptions on $f$ are slightly different, e.g., $f$ may not have full domain.  

\begin{Proposition}[Unique/sharp/strong solutions for problems \eqref{BP0} and \eqref{Las0}] \label{Stheo} Suppose that $\ox$ is an optimal solution to problem \eqref{Las0} and  $\Phi\ox\in {\rm int}\, (\dom f)$. Then $\ox$ is a solution to problem \eqref{BP0} with $x_0=\ox$. Moreover, the following statements hold:
\begin{enumerate}[label={\rm (\roman*)}]
    \item $\ox$ is the unique solution to \eqref{Las0} if and only if it is the unique solution to \eqref{BP0}. 
    \item If $\ox$ is a sharp solution to \eqref{BP0} then it is a strong solution to problem \eqref{Las0}. %Thus conditions $\Ker \Phi\cap \Ker D_{S}^*=\{0\}$ and  $\rho(e)<1$ are sufficient for strong solution at $\ox$ to problem \eqref{Las0}.
    \item If $\ox$ is a strong solution to \eqref{Las0} then it is also a strong solution to \eqref{BP0}.  
\end{enumerate}
\end{Proposition}
\begin{proof} 
 For any $x\in \Phi^{-1}(\Phi\ox)$, we have 
\begin{equation}\label{indy}
f(\Phi \ox)+\mu J(x)=f(\Phi x)+\mu J(x) \ge f(\Phi \ox)+\mu J(\ox).
\end{equation}
It follows that $\ox$ is a solution to problem \eqref{BP0} with $y_0=\Phi \ox$. Moreover, if $\ox$ is the unique solution to problem \eqref{Las0}, we have the strict inequality in \eqref{indy} provided that $x\neq \ox$, which shows that $\ox$ is also the unique solution to problem \eqref{BP0}. 

 To verify (i), it suffices to show that $\ox$ is an isolated point to the convex solution set of problem \eqref{Las0} provided that  $\ox$ is the unique solution to \eqref{BP0}. By contradiction, suppose that there is another solution $\hat x$ to \eqref{Las0} close enough to $\ox$ such that $\Phi \hat x\in {\rm int}\,(\dom f)$. We have $-\Phi^*\nabla f(\Phi\hat x)\in \partial J(\hat x)$ and $-\Phi^*\nabla f(\Phi\ox)\in \partial J(\ox)$. The monotonicity of the subdifferential tells us that 
 \[
 \la -\nabla f(\Phi \hat x)+\nabla f(\Phi \ox), \Phi\hat x-\Phi\ox\ra=\la -\Phi^*\nabla f(\Phi \hat x)+\Phi^*\nabla f(\Phi \ox),\hat x-\ox\ra\ge 0.
 \]
Since $f$ is twice continuously differentiable in ${\rm int}\, (\dom f)$, we obtain from the mean-value theorem that 
\begin{equation}\label{nabla}
-\int_0^1\la t\nabla^2 f(\Phi(t\hat x+(1-t)\ox))\Phi(\hat x-\ox),\Phi(\hat x-\ox)\ra dt\ge 0.
\end{equation}
Since $\nabla^2 f\succ0$ and it is continuous in ${\rm int}\,(\dom f)$, there exists some $\ell>0$ such that $$\la\nabla^2 f(\Phi(t\hat x+(1-t)\ox))\Phi(\hat x-\ox),\Phi(\hat x-\ox)\ra\ge \ell \|\Phi(\hat x-\ox)\|^2$$
for all $t\in [0,1]$.
Combining this with \eqref{nabla} implies that $\Phi\hat x=\Phi\ox$. Since both $\hat x$ and $\ox$ are minimizers to problem \eqref{Las0}, we have $\hat x=\ox$.  This contradiction allows us to verify (i). 

To justify (ii), suppose that $\ox$ is a sharp solution to \eqref{BP0}. By Proposition~\ref{Shar}, \eqref{D0} and \eqref{dPhi}
, we have 
\begin{equation}\label{DD}
\Ker \Phi\cap \CC_J(x_0)=0\quad \mbox{with}\quad \CC_J(x_0)=\{w\in \R^p|\; dJ(x_0)(w)\le0\}.
\end{equation}
Note from the sum rule \eqref{sum} and \eqref{dom2} that 
\begin{equation}\label{Tep}
d^2\Theta(\ox|0)(w)=\la \nabla^2 f(\Phi \ox)\Phi w, \Phi w\ra+\mu d^2J (\ox|-\mu^{-1}\Phi^*\nabla f(\Phi\ox)(w))\ge \la \nabla^2 f(\Phi \ox)\Phi w, \Phi w\ra
\end{equation}
and $\dom d^2\Theta(\ox|0)\subset \{w\in \R^n|\;d\Theta(\ox)(w)= 0\}$. Similarly to the calculation in \eqref{dPhi}, we have \[
d\Theta(\ox)(w)=\la\nabla f(\Phi\ox),\Phi w\ra+\mu dJ(x_0)(w).
\]
It follows that 
\begin{equation}\label{Kx}
\dom d^2\Theta(\ox|0)\subset\{w\in \R^n|\;\la \nabla f(\Phi\ox),\Phi w \ra+\mu dJ(x_0)(w)=0\}.
\end{equation}
To verify that $\ox$ is a strong solution to problem \eqref{Las0} by using Lemma~\ref{Fa}, we claim that  
\begin{equation}\label{Ky}
\la\nabla^2f(\Phi \ox)\Phi w, \Phi w\ra>0\quad \mbox{for all}\quad w\in \dom d^2\Theta(\ox|0)\setminus\{0\}.
\end{equation}
Suppose that  $w\in \dom d^2\Theta(\ox|0)$ satisfying $\la\nabla^2f(\Phi \ox)\Phi w, \Phi w\ra\le 0$. Since   $\nabla^2f(\Phi \ox)\succ 0$, we have $\Phi w=0$.  This together with \eqref{Kx} tells us that $w\in \Ker \Phi\cap \CC_J(x_0)=\{0\}$ by \eqref{DD}. Thus inequality \eqref{Ky} holds and $\ox$ is a strong solution to problem to \eqref{Las0}. 

To verify (iii), suppose that $\ox$ is a strong solution to problem \eqref{Las0}. There exist constants $\kk,\gg>0$ such that
\[
f(\Phi x)+\mu J(x)\ge f(\Phi\ox)+\mu J(\ox)+\frac{\kk
}{2}\|x-\ox\|^2_\AA\quad \mbox{for all}\quad x\in \B_\gg(\ox).
\]
For any $x\in \B_\gg(\ox)\cap \Phi^{-1}(\Phi \ox)$, we obtain that 
\[
 J(x)\ge J(\ox)+\frac{\kk}{2\mu}\|x-\ox\|^2_\AA,
\]
which means that $\ox$ is also a strong solution to \eqref{BP0}. The proof is complete. 
\end{proof} 



    
 For the special case \eqref{Las3} of \eqref{Las0}, \cite[Theorem~1]{FPVDS13} shows that if $\ox$ is an optimal solution to \eqref{Las0} with $x_0=\ox$  and the Strong Null Space Property \eqref{SNS} holds at $\ox$,  $\ox$ is a unique  solution to \eqref{Las0}. As Strong Null Space Property is a characterization for sharp minima to problem \eqref{BP0},  Proposition~\ref{Stheo}(ii) advances \cite[Theorem~1]{FPVDS13} and  \cite[Theorem~3]{VGFP15} with further information that $\ox$ is a strong solution to \eqref{Las3}. 
 
 
 %This result could be explained as follows. Since the Strong Null Space Property is a characterization for sharp minima at $\ox=x_0$ to problem \eqref{BP0} as discussed before \eqref{SNS}, $\ox$ is the unique solution to problem \eqref{BP0}. If $\hat x$ is another solution to \eqref{Las0}, we have $-\Phi^*(\Phi \hat x-y)\in D\partial\|D\hat x\|_\AA$ and $-\Phi^*(\Phi \ox-y)\in D\partial\|D\hat x\|_\AA$, due to the monotonicity of the subdifferential, one has
 %\[
 %\la -\Phi^*(\Phi \hat x-y)+\Phi^*(\Phi \ox-y),\hat x-\ox\ra\ge 0,
% \]
% which implies $\Phi\hat x=\Phi \ox$. Thus $\hat x$ is also a solution to problem \eqref{BP0}, which means $\hat x=\ox$, i.e., $\ox$ is the unique solution to \eqref{Las0}. Another direct explanation could come from \cite[Proposition~3.2]{MS19}. In the following result, we provide another insight, which tells us that Strong Null Space Property or our conditions are sufficient for strong solution to problem \eqref{Las0}. 

There are two questions arising from Proposition~\ref{Stheo}: 
\begin{enumerate}
    \item[{\bf (Q1)}] If  $\ox$ is a strong solution to \eqref{Las0}, can it be a sharp solution to \eqref{BP0} with $x_0=\ox$?
    \item[{\bf (Q2)}]  If $\ox$ is a strong solution to \eqref{BP0}, can it be a strong solution to \eqref{Las0}?
\end{enumerate}
For analysis $\ell_1$ problems, i.e., $J_0(\cdot)=\|\cdot\|_1$,  we have positive answers for both questions.
\begin{Corollary}[Solution uniqueness to $\ell_1$ problems]\label{ell2} Let $\ox$ be a minimizer to \eqref{Las0} with $J_0(\cdot)=\|\cdot\|_1$. Then the following are equivalent:
\begin{enumerate}[label={\rm (\roman*)}]
    \item $\ox$ is the  unique solution to problem \eqref{BP0} with $x_0=\ox$.
    \item $\ox$ is the sharp solution to problem \eqref{BP0} with $x_0=\ox$.
    \item $\ox$ is the unique solution to problem \eqref{Las0}.
    \item $\ox$ is the  strong solution to problem  \eqref{Las0}.
\end{enumerate}
\end{Corollary}
\begin{proof} 
 [(i)$\Leftrightarrow$(iii)] and [(ii)$\Rightarrow$(iv)] are from Proposition~\ref{Stheo}. [(iv)$\Rightarrow$(iii)] is trivial. Moreover, [(i)$\Leftrightarrow$(ii)] is valid as $\|\cdot\|_1$ is a convex piecewise linear function.  The proof is complete. \end{proof} 


According to Theorem~\ref{mtheo}, conditions $\Ker \Phi\cap \Ker D_{S}^*=\{0\}$ 
and  $\rho(e)<1$ form a characterization for solution uniqueness to $\ell_1$ problem.  A similar result was established in \cite[Theorem~1]{ZYY16} for problems \eqref{BP0} and \eqref{Las3} with the extra assumption that $\Phi$ has full row-rank. Corollary~\ref{ell2} is more general and reveals that the unique solution to problem \eqref{Las0} is the strong solution.  


The answer is negative for {\bf(Q1)} in general; see our  Theorem~\ref{Las2} and Example~\ref{Ex12}. For group-sparsity problem, we show that if $\ox$ is a strong solution to \eqref{Las0}, it is also a strong solution to \eqref{BP0}; see Theorem~\ref{Las2}.  Regarding {\bf (Q2)}, we  have the positive answer  for group-sparsity  optimization problem; see Theorem~\ref{BP12} and Theorem~\ref{Las2}.  However, it is not true for the nuclear norm miniminzation problem (NNM).     




\begin{Example}[Difference between strong solutions to problems  \eqref{BP0} and \eqref{Las0}]\label{Last3}
{\rm
Let us consider the following nuclear norm minimization problem
\begin{equation}\label{LN}
    \min_{X\in\R^{2\times 2}} \Theta(X)  \eqdef  \dfrac{1}{2}\|\Phi(X) - Y\|^2+ \|X\|_*,
\end{equation}
where $\|\cdot\|_*$ stands for the nuclear norm of $X$, $\Phi:\R^{2\times2}\to \R^{2}$ is  defined by $\Phi(X)=\left[\begin{array}{c}
     X_{11}  \\
     X_{22} 
\end{array}\right]$ and $Y=\left[\begin{array}{c}
  2\\
  1
\end{array}\right]$. Let $\Bar X=\left[\begin{array}{cc}
  1   &  0\\
   0  &  0
\end{array}\right]$ and $f(\cdot)=\frac{1}{2}\|\cdot-Y\|^2$, we have 
\begin{equation*}
    \Phi^*\nabla f(\Phi(\Bar X)) = \left[\begin{array}{cc}
  -1   &  0\\
   0  &  -1
\end{array}\right] \quad \text{ and } \quad \partial\|\Bar X\|_* = \left\{\left[\begin{array}{cc}
  1   &  0\\
   0  &  \alpha
\end{array}\right]: \alpha\in [-1,1]\right\}.
\end{equation*}
Thus $0\in \partial \Theta(\Bar X)$, i.e., $\Bar X$ is a solution to \eqref{LN}. By Proposition~\ref{Stheo}, it is also a solution to the following problem:
\begin{equation}\label{BPN}
\min_{X\in\R^{2\times 2}} \|X\|_* \quad\text{ subject to }\quad \Phi(X)=\left[\begin{array}{c}
     1  \\
     0 
\end{array}\right].
\end{equation}
For any $2\times 2$ matrix $X$, let $\sigma_1,\sigma_2$ be the singular values of $X$,  we have
\begin{equation}\label{nucl}
   \|X\|_*=\sigma_1+\sigma_2=\sqrt{\sigma_1^2+\sigma^2_2+2\sigma_1\sigma_2}=\sqrt{\|X\|_F^2+2|{\rm det}\,(X)|}. 
\end{equation}
For any feasible solution $X$ to \eqref{BPN} with $X= \left[\begin{array}{cc}
  1   &  a\\
   b  &  0
\end{array}\right]$, we obtain from \eqref{nucl} that 
\[
\|X\|_*= \sqrt{1+a^2+b^2+2|ab|}
.
\]
Thus $\Bar X$ is the unique solution to \eqref{BPN} as well as $\eqref{LN}$ due to Proposition~\ref{Stheo} again. Next we claim that $\Bar X$ is the strong solution to \eqref{BPN}, which means there exist $\kappa, \delta>0$ such that
\begin{equation}\label{nucl_str}
\|X\|_*-\|\Bar X\|_*\geq\dfrac{\kappa}{2}\|X-\Bar X\|^2_F \quad\text{ for all }\quad   X= \left[\begin{array}{cc}
  1   &  a\\
   b  &  0
\end{array}\right] \quad \mbox{with}\quad \|X-\Bar X\|_F=\sqrt{a^2+b^2}\le \delta.
\end{equation} 
Indeed, note that 
\begin{eqnarray*}
\|X\|_*-\|\Bar X\|_* &=& \sqrt{1+a^2+b^2+2|ab|}-1\\
&=&\dfrac{a^2+b^2+2|ab|}{\sqrt{1+a^2+b^2+2|ab|}+1}\\
&\geq& \dfrac{a^2+b^2}{\sqrt{1+2\delta^2}+1}\\
&=& \dfrac{1}{\sqrt{1+2\delta^2}+1}\|X-\bar X\|_F^2.
\end{eqnarray*}
This certainly verifies \eqref{nucl_str}. Next we claim that $\Bar X$ is not a strong solution to \eqref{LN}. Pick $X_\ve \eqdef \left[\begin{array}{cc}
1+\ve^2 & \ve \\
 \ve    & \ve^2
\end{array}\right]$ with $\ve>0$ sufficiently small, observe that $\|X-\Bar X\|^2_F=2(\ve^2+\ve^4)$. It follows from \eqref{nucl} that
\begin{eqnarray*}
\Theta(X_\ve)-\Theta(\Bar X) &=& \dfrac{1}{2}\left\|\left[\begin{array}{c}
    \ve^2-1   \\
    \ve^2-1
\end{array}\right]\right\|^2+\left\|\left[\begin{array}{cc}
    1+\ve^2 & \ve   \\
    \ve & \ve^2
\end{array}\right]\right\|_*-2\\
&=& (\ve^2-1)^2+\sqrt{((1+\ve^2)^2+2\ve^2+\ve^4)+2\ve^4}-2\\
&=& (\ve^2-1)^2+(1+2\ve^2)-2\\
&=&\ve^4.
\end{eqnarray*}
Therefore, $\Bar X$ is not a strong solution to \eqref{LN}, which also implies that $\Bar X$ is neither a sharp solution to \eqref{LN} nor to \eqref{BPN} due to Proposition~\ref{Stheo}.
%\color{red}{My calculation:
%\begin{eqnarray}
%d^2\Theta(\Bar X|0)(W)=\left\{\begin{array}{ll}
%a^2+d^2+(b-c)^2\quad &\mbox{if}\quad d>0,\\
%a^2+(|b|+|c|)^2\color{blue}{\longleftarrow  a^2+(b-c)^2????}\quad &\mbox{if}\quad d=0\\
%\infty \quad &\mbox{if}\quad d<0\end{array}\right.\quad \mbox{with}\quad W=\left[\begin{array}{cc}
%a & b \\
%c    & d
%\end{array}\right].
%\end{eqnarray}
%It follows that $d^2\Theta(\Bar X|0)(W)>0$ for all $W\neq 0$, which tells us that $\Bar X$ is a strong solution!!!
%}

}
\end{Example}

%Theorem~\ref{Rob} highlights the role of sharp minima in robust recovery when $\|\cdot\|_\AA$ is any norm in $\R^p$. In the framework of decomposable norm, we can improve it as follows by discovering the special structure of decomposable norms. This result  generalizes \cite[Theorem~4.7]{GHS11} and \cite[Theorem~2]{ZYY16}, which are established for $\ell_1$ problems only. 

%\begin{Theorem}[Sharp minima for robust recovery] The following are equivalent:
%\begin{enumerate}[label={\rm (\roman*)}]
 %   \item $x_0$ is a sharp solution to problem \eqref{BP0}.
  %  \item For any $\delta>0$ and $c_1>0$ there exists $c_2>0$ such that every minimizer $x_{\delta}$ to \eqref{Las2} satisfies
   % \begin{equation}\label{Est}
     %   \|D^*(x_\mu-x_0)\|\le c_2\delta
    %\end{equation}
%with $\|y-\Phi x_0\|\le \delta$ and $\mu= c_1\delta$. 
%%\end{enumerate}
%\end{Theorem}
%\begin{proof} 
 Let us justify implication $[{\rm (i)}\Rightarrow{\rm (ii)}]$ first. Suppose that $x_0$ is a sharp solution to problem \eqref{BP0}. By Theorem~\ref{mtheo}, the Restricted Injectivity holds at $x_0$ and there exists $\ov\in \R^p$ and $\oz\in \R^m$ such that $D\ov=\Phi \oz $, $P_T\ov=e$, and that $\|P_T\ov\|=\rho(e)<1.$ Note that
%\[
%\frac{1}{2}\|\Phi x_\mu-y\|^2+\mu\|D^*x_\mu\|\le\frac{1}{2}\|\Phi x_0-y\|^2+\mu\|D^*x_0\|
%\]
%Define $\beta_\mu \eqdef \|D^*x_\mu\|-\|D^*x_0\|-\la \ov,D^*x_\mu-D^*x_0\ra$ as the Bregman distance of $D^*x_\mu$ and $D^*x_0$ with respect to $\ov$. It follows from the above inequality  and the equality $D\ov=\Phi\oz$ that
%\begin{eqnarray}\label{Berg}\begin{array}{ll}
%\beta_\mu&\le \disp \frac{1}{2\mu}[\|y-y_0\|^2-\|\Phi x_\mu-y\|^2]-\la \ov, D^*(x_\mu-x_0)\ra\\
%&\disp\le\frac{1}{2\mu}[\|y-y_0\|^2-(\|\Phi (x_\mu-x_0)\|-\|y-y_0\|)^2]-\la \oz, \Phi(x_\mu-x_0)\ra\\
%&\disp\le \frac{1}{2\mu}[-\|\Phi (x_\mu-x_0)\|^2+2\|\Phi (x_\mu-x_0)\|\|y-y_0\|]+\|\oz\| \|\Phi(x_\mu-x_0)\|\\
%&\disp\le -\frac{1}{2\mu}\|\Phi (x_\mu-x_0)\|^2+\left(\|\oz\|+\frac{\delta}{\mu}\right)\|\Phi (x_\mu-x_0)\|\\
%&\le \disp \left(\|\oz\|+\frac{\delta}{\mu}\right)^2\frac{\mu}{2}.
%\end{array}
%\end{eqnarray}
%Moreover, observe that 
%\begin{eqnarray}\label{Ke}\begin{array}{ll}
%\beta_\mu&=J(x_\mu)-\la \ov, D^*x_\mu\ra+J(x_0)-\la \ov, D^*x_0\ra=J(x_\mu)-\la \ov, D^*x_\mu\ra\\
%&=\disp J(x_\mu)-\la P_Te , D^*x_\mu\ra- \la P_{S}\ov , D^*x_\mu\ra\\
%&=\disp J(x_\mu)-\la e , D_T^*x_\mu\ra- \la P_{S}\ov , D_{S}^*x_\mu\ra.
%\end{array}
%\end{eqnarray}
%For any $v\in \partial J(x_0)$, it is similar to  have
%\[
%0\le J(x_\mu)-\la v, D^*x_\mu\ra= J(x_\mu)-\la e , D_T^*x_\mu\ra- \la P_{S}v , D_{S}^*x_\mu\ra. 
%\]
%It follows from \eqref{norA} that
%\[
%0\le J(x_\mu)-\la e , D_T^*x_\mu\ra-\|D^*_{S}x_\mu\|_\AA.
%\]
%This together with \eqref{Ke} tells us that 
%\begin{equation}\label{Lower}
%\beta_\mu\ge \|D^*_{S}x_\mu\|_\AA-\|P_T\ov\|^*_\AA\|\|D^*_{S}x_\mu\|_\AA=(1-\rho(e))\|D^*_{S}x_\mu\|_\AA. 
%\end{equation}
%Combining this with \eqref{Berg}, we have 
%\begin{equation}
 %   \|D^*_{S}x_\mu\|_\AA\le \left(\|\oz\|+\frac{\delta}{\mu}\right)^2\frac{\mu}{2(1-\rho(e))}.
%\end{equation}
%With $u_0=D^*x_0$, note further from definition of Decomposable norm at $u_0$ that for any $v\in \partial \|u_0\|_\AA$:
%\[
%\|u_0\|_\AA=\la v,u_0\ra=\la e, u_0\ra+\la P_{S} v,P_{S} u_0\ra.
%\]
%For $v=e$, we have $\|u_0\|=\la e, u_0\ra$. Moreover, \eqref{norA} tells us that $\|u_0\|=\la e,u_0\ra+\|P_{S}u_0\|$. This implies that $P_{S}u_0=0$, i.e., $u_0\in T.$

%It is time to verify \eqref{Est}. Since $u_0=D^*x_0\in T$, we have
%\begin{eqnarray*}\begin{array}{ll}
%\|D^*(x_\mu-x_0)\|\le \|D^*_T(x_\mu-x_0)\|+\|D^*_{S} x_\mu\|.             
%\end{array}    
%\end{eqnarray*}
%Since $\Ker \Phi\cap \Ker D^*_{S}={0}$


==> tex_220921/sec_strong_group.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Characterizations of unique/strong solutions  to group-sparsity optimization problems}
\label{sec:stronggroup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we study a particular class of \eqref{BP0}, the group-sparsity problem at which $J_0$ is the $\ell_1/\ell_2$ norm; see, e.g.,  \cite{RRN12,RF08,YL06}. Following the notation in \cite{CR13}, we suppose that $\R^p$ is decomposed into $q$ groups by 
\begin{equation}
    \R^p=\bigoplus_{g=1}^q V_g,
\end{equation}
where each $V_g$ is a subspace of $\R^p$ with the same dimension $G$. For any $u\in \R^p$, we write  $u=\disp\sum_{g=1}^qu_g$ with $u_g\in V_g$ being  the vector in group $V_g$. The $\ell_1/\ell_2$ norm in $\R^p$  is defined by
\begin{equation}\label{l12}
\|u\|_{\ell_1/\ell_2}=\sum_{g=1}^q\|u_g\|.  
\end{equation}
Its dual is the  $\ell_\infty/\ell_2$ norm:
\begin{equation}\label{li2}
\|u\|_{\ell_\infty/\ell_2}=\max_{1\le g\le q}\|u_g\|.  
\end{equation}
With  $\ou \eqdef D^*x_0$, define $I \eqdef \left\{g\in \{1,\ldots,q\}|\; \ou_g\neq 0\right\}$, the index set of active groups of $\ou$, and $K \eqdef \{1,\ldots,q\}\setminus I$, the index set of nonactive groups of $\ou$. Note that 
\begin{equation}\label{sub12}
    \partial\|\ou\|_{\ell_1/\ell_2} \eqdef \left\{v\in \R^p|\; v_g= \frac{ \ou_{g}}{\|\ou_{g}\|_2}\mbox{ for } g\in I \mbox{ and } \|v_g\|\le 1 \mbox{ for } g\in K\right\}. 
\end{equation}
Thus $\ell_1/\ell_2$ norm is decomposable at $\ou$ as in Remark~\ref{Deco}, where $T=\disp\bigoplus_{g\in I} V_g$ and 
\begin{equation}\label{e12}
    e=\sum_{g\in I} \frac{\ou_{g}}{\|\ou_{g}\|}.
\end{equation}
This section devotes to  studying the  group-sparsity regularized optimization problem:
\begin{equation}\label{ITV}
\min_{x\in \R^n}\quad \|D^*x\|_{\ell_1/\ell_2}\quad\mbox{subject to}\quad \Phi x=\Phi x_0,
\end{equation}
which is a particular case of \eqref{BP0}. 
Sharp minima at $x_0$ for problem \eqref{ITV} is studied in our previous section. However, unlike the case of $\ell_1$ problem, a unique solution to problem \eqref{ITV} may be not sharp; see  Example~\ref{Ex12}. To characterize the solution uniqueness to group sparsity problem \eqref{ITV}, we compute the  descent cone $\TT_\AA(x_0)$ in \eqref{Des} as follows.  

\begin{Theorem}[Descent cone to $\ell_1/\ell_2$ problem and geometric characterization for solution uniqueness]\label{Uniq} The descent cone  at $x_0$ to problem \eqref{ITV} is computed by 
\begin{equation}\label{Sub}
    \TT_{J} (x_0)=(\mathcal{E}\cap {\rm bd}\,\CC_{J}(x_0
    ))\cup({\rm int}\, \CC_{J}(x_0)),
\end{equation}
where $\mathcal{E}$ is defined by 
\begin{equation}\label{C} \mathcal{E} \eqdef \left\{w\in\R^n|\, D_T^*w\in \span\{(D^*_Tx_0)_g|\; g\in I\}\right\}
\end{equation}
and ${\rm bd}\,\CC_{J}(x_0)$ stands for the boundary of the critical cone $\CC_{J}(x_0)$ defined in \eqref{D0}, i.e., 
\begin{equation}\label{bd}
    {\rm bd}\,\CC_{J}(x_0)=\{w\in \R^p|\; \la De,w\ra+\|D^*_{T^\perp}w\|_{\ell_1/\ell_2}=0\}.
\end{equation}
Consequently, $x_0$ is a unique solution to \eqref{ITV} if and only if 
\begin{equation}\label{Geo}
    \Ker \Phi \cap \Big[(\mathcal{E}\cap {\rm bd}\, \CC_{J}(x_0))\cup({\rm int}\, \CC_{J}(x_0))\Big]=\{0\}.\end{equation}
\end{Theorem}
\begin{proof} 
 Let us start to verify the ``$\supset$'' in \eqref{Sub}.  Recall that  $J(x)=\|D^*x\|_{\ell_1/\ell_2}$.  For any $w\in {\rm int}\, (\CC_{J}(x_0))$, we get from \eqref{D0} that  
\[
dJ(x_0)(w)=\lim_{t\dn 0}\dfrac{J(x_0+tw)-J(x_0)}{t}<0.
\]
Hence there is some $t_0>0$ such that $J(x_0+t_0w)< J(x_0)$. This ensures $w\in \TT_J(x_0)$. For any $w\in \mathcal{E}\cap {\rm bd}\, \CC_{J}(x_0)$, we represent $D_T^*w=\sum_{g\in I}\lm_g (D^*x_0)_g$ with $\lm_g\in \R$, $g\in I$ and 
% \begin{equation}\label{inqe}
%     \la D_Te,w\ra+\|P_{S}w\|_{\ell_1/\ell_2}=\la e,D^*_Tw\ra+\|P_{S}w\|_{\ell_1/\ell_2}=\sum_{g\in I}{\lm_g}+\sum_{g\in J}\|w_g\|= 0.
% \end{equation}
% Define $t_1 \eqdef \min\left\{-\dfrac{\|(D^*x_0)_g\|}{\lm_g}|\; g\in I_-\right\}>0$ with $I_- \eqdef \{g\in I|\; \lm_g<0\}$, we have 
% \[\begin{array}{ll}
% \|D^*x_0+t_1D^*w\|_{\ell_1/\ell_2}-\|D^*x_0\|_{\ell_1/\ell_2}&=\disp\sum_{g\in I}\left|\|(D^*x_0)_g\|+t_1\lm_g\right|+\sum_{g\in J} t_1\|D^*w_g\|-\|(D^*x_0)_g\|\\
% &=\disp\sum_{g\in I}\|(D^*x_0)_g\|+t_1\lm_g+\sum_{g\in J} t_1\|(D^*w)_g\|-\|(D^*x_0)_g\|,
% \end{array}
% \]
\begin{equation}\label{inqep}
   0 = \la D_Te,w\ra+\|D^*_{T^\perp}w\|_{\ell_1/\ell_2}=\la e,D^*_Tw\ra+\|D^*_{T^\perp}w\|_{\ell_1/\ell_2}=\sum_{g\in I}{\lm_g}\|(D^*x_0)_g\|+\|D_{T^\perp}^*w\|_{\ell_1/\ell_2}.
\end{equation}
Define  $I_- \eqdef \{g\in I|\; \lm_g<0\}$. If $I_-=\emptyset$, we get from \eqref{inqep} that $D^*_Sw=0$ and $\lm_g=0$ for all $g\in I$, which implies  that $D^*_Tw=0$ and $D^*w=0$. Thus we have
\[
J(x_0+w)=J_0(D^*(x_0+w))=J_0(D^*x_0)=J(x_0),
\]
which tells us that $w\in \TT_J(x_0)$. If $I_-\neq\emptyset$, define
$t_1 \eqdef \min\left\{-\dfrac{1}{\lm_g}|\; g\in I_-\right\}>0$, we obtain from \eqref{inqep} that  
\[\begin{array}{ll}
J(x_0+t_1w)-J(x_0)&\disp=\|D^*x_0+t_1D^*w\|_{\ell_1/\ell_2}-\|D^*x_0\|_{\ell_1/\ell_2} \\
&=\disp\sum_{g\in I}|1+t_1\lm_g|\|(D^*x_0)_g\|+t_1\|D_{T^\perp}^*w\|_{\ell_1/\ell_2}-\|D^*x_0\|_{\ell_1/\ell_2}\\
&=\disp\sum_{g\in I}(1+t_1\lm_g)\|(D^*x_0)_g\|+t_1\|D_{T^\perp}^*w\|_{\ell_1/\ell_2}-\|D^*x_0\|_{\ell_1/\ell_2}\\
&= 0,
\end{array}
\]
where the second equality is from the choice of $t_1$. In both cases of $I_-$,  $w\in \TT_J(x_0)$. This verifies the inclusion ``$\subset$'' in \eqref{Sub}.


To justify the reverse inclusion ``$\subset$'' in \eqref{Sub}, take any $w\in \TT_J(x_0)$ and find some $t>0$  such that $\|D^*x_0+tD^*w\|_{\ell_1/\ell_2}\le \|D^*x_0\|_{\ell_1/\ell_2}$. For any $\al\in (0,1)$, we have
\[
\|D^*x_0\|_{\ell_1/\ell_2}\ge \al \|D^*x_0+tD^*w\|_{\ell_1/\ell_2}+(1-\al)\|D^*x_0\|_{\ell_1/\ell_2}\ge \|D^*x_0+\al tD^*w\|_{\ell_1/\ell_2}.
\]
Choose $\al>0$ sufficiently small   such that 
\[
\|(D^*x_0)_g+\al t(D^*w)_g\|>0\quad \mbox{for all}\quad  g\in I. 
\]
Since $w\in \CC_{J}(x_0)$ by \eqref{CD2}, it suffices to show that if  $w\in {\rm bd}\, \CC_{J}(x_0)$ then $w\in \mathcal{E}.$ Suppose that  $w\in {\rm bd}\, \CC_{J}(x_0)$, we have 
\[
0=\la D_Te,w\ra+\|D_{T^\perp}^*w\|_{\ell_1/\ell_2}=\la e,D^*_Tw\ra+\|D_{T^\perp}^*w\|_{\ell_1/\ell_2}.
\]
It follows from the latter that 
\begin{eqnarray}\label{Big}\begin{array}{ll}
 0&\ge \disp\|D^*x_0+\al tD^*w\|_{\ell_1/\ell_2}- \|D^*x_0\|_{\ell_1/\ell_2}\\
 &\disp=\sum_{g\in I}\|(D^*x_0)_g+\al t (D^*w)_g\|+\al t\sum_{g\in K}\|(D^*w)_g\|-\|D^*x_0\|_{\ell_1/\ell_2}\\
    &\disp=\sum_{g\in I}\left[\|(D^*x_0)_g+\al t (D^*w)_g\|-\|(D^*x_0)_g\|-\al t\la e_g, (D^*w)_g\ra\right].
    \end{array}
\end{eqnarray}
Since $e_g= \partial \|(D^*x_0)_g\|$, each $\|(D^*x_0)_g+\al t (D^*w)_g\|-\|(D^*x_0)\|_g-\al t\la e_g, (D^*w)_g\ra\ge 0$ for $g\in I$. This together with \eqref{Big} tells us that
\[
0=\|(D^*x_0)_g+\al t (D^*w)_g\|-\|(D^*x_0)_g\|-\al t\la e_g, (D^*w)_g\ra\quad \mbox{for any}\quad g\in I.
\]
Hence, we have
\[
0=\|(D^*x_0)_g\|-\la e_g, (D^*x_0)_g\ra=\|(D^*x_0)g+\al t (D^*w)_g\|-\la e_g,(D^*x_0)g+\al t (D^*w)_g\ra.
\]
As $\|e_g\|=1$ and $(D^*x_0)_g+\al t (D^*w)_g\neq 0$, the latter equality holds when
$$(D^*x_0)_g+\al t (D^*w)_g=\iota_g e_g$$ for some $\iota_g>0$, $g\in I$. It follows that 
\[
(D^*w)_g=\frac{1}{\al t}(\iota_g -\|(D^*x_0)_g\|)e_g
\]
for any $g\in I$, which ensures that $w\in \mathcal{E}$ and verifies the equality \eqref{Sub}. 

The characterization for solution uniqueness at $x_0$ in \eqref{Geo} follows directly from Proposition~\ref{DeUn} and \eqref{Sub}. \end{proof} 




We show next that a unique solution to \eqref{BP0} is indeed a strong solution. The proof is based on the second-order analysis in Lemma~\ref{Fa}. We need the computation of the second subderivative for the function $\Psi$ defined in \eqref{Psi}. 




\begin{Lemma}[Second subderivative to $\ell_1/\ell_2$ norm]\label{SOD}  Suppose that $x_0$ is a minimizer to problem \eqref{ITV}. Then we have 
\begin{equation}\label{dom}
    \dom d^2\Psi(x_0|0)=\Ker \Phi\cap {\rm bd}\, \CC_{J}(x_0)
\end{equation} 
and  
\begin{eqnarray}\label{d2}
d^2\Psi(x_0|0)(w)=\sum_{g\in I} \dfrac{\|(D^*w)_g\|^2\|(D^*x_0)_g\|^2-\la (D^*x_0)_g,(D^*w)_g\ra^2}{\|(D^*x_0)_g\|^3}\;\; \mbox{for}\;\;  w\in \dom d^2\Psi(x_0|0). 
\end{eqnarray}

\end{Lemma}
\begin{proof} 
 Since $x_0$ is an optimal solution to \eqref{ITV}, we have $0\in \partial \Psi(x_0)$. With $C=\Phi^{-1}(\Phi x_0)$, we have
\begin{eqnarray*}
d^2\Psi(x_0|0)(w)&=&\liminf_{t\downarrow 0,\; w'\to w}\dfrac{\|D^*(x_0+tw')\|_{\ell_1/\ell_2}+\iota_C(x_0+tw')-\|D^*x_0\|_{\ell_1/\ell_2}-\iota_C(x_0)-t\la 0,w\ra}{\frac{1}{2}t^2}\\
&=&\liminf_{t\downarrow 0,\; w'\to w}\left(\dfrac{\|D^*(x_0+tw')\|_{\ell_1/\ell_2}-\|D^*x_0\|_{\ell_1/\ell_2} }{\frac{1}{2}t^2}+\iota_{\Ker \Phi}(w')\right).
\end{eqnarray*}
It follows that $\dom d^2\Psi(x_0|0)\subset\Ker \Phi$. Since $D^*_{T^\perp}x_0=0$, we have
\begin{eqnarray}\label{Q1}\begin{array}{ll}
&\disp\liminf_{t\downarrow 0,\; w'\st{{\rm Ker}\, \Phi}\to w}\dfrac{\|D^*(x_0+tw')\|_{\ell_1/\ell_2}-\|D^*x_0\|_{\ell_1/\ell_2} }{\frac{1}{2}t^2}\\ 
&\disp=\liminf_{t\downarrow 0,\; w'\st{{\rm Ker}\, \Phi}\to w}\left(\dfrac{\|D_T^*(x_0+tw')\|_{\ell_1/\ell_2}-\|D_T^*x_0\|_{\ell_1/\ell_2}-t\la De,w'\ra }{\frac{1}{2}t^2}+\dfrac{\la De,w'\ra +\|D_{T^{\perp}}^*w'\|_{\ell_1/\ell_2}}{\frac{1}{2}t}\right).
\end{array}
\end{eqnarray}
Note that the Euclidean norm $\|u\|$ is twice differentiable at $u\neq 0$ with 
\[
\nabla \|u\|=\frac{u}{\|u\|}\quad \mbox{and}\quad \nabla^2\|u\|=\frac{1}{\|u\|}\Id-\frac{1}{\|u\|^3}uu^*
\]
This together with \eqref{smooth} tells us that
 \begin{eqnarray}\label{Q}\begin{array}{ll}
&\disp\liminf_{t\downarrow 0,\; w'\st{{\rm Ker}\, \Phi}\to w}\dfrac{\|D_T^*(x_0+tw')\|_{\ell_1/\ell_2}-\|D_T^*x_0\|_{\ell_1/\ell_2}-t\la De,w'\ra }{\frac{1}{2}t^2}\\
 &\disp=\disp\liminf_{t\downarrow 0,\; w'\st{{\rm Ker}\, \Phi}\to w}\sum_{g\in I}\left[\dfrac{\|(D^*(x_0+tw'))_g\|-\|(D^*x_0)_g\|-t\la e_g,D^*w'\ra }{\frac{1}{2}t^2}\right]\\
 &=\disp\sum_{g\in I}\left\la  (D^*w)_g,    \dfrac{(D^*w)_g}{\|(D^*x_0)_g\|}-\frac{1}{\|(D^*x_0)_g\|^3}(D^*x_0)_g(D^*x_0)_g^*(D^*w)_g\right\ra\\
 &=\disp\sum_{g\in I}\dfrac{\|(D^*w)_g\|^2\|(D^*x_0)_g\|^2-\la (D^*x_0)_g,(D^*w)_g\ra^2}{\|(D^*x_0)_g\|^3}.
\end{array}
 \end{eqnarray}
 
 Since $x_0$ is an optimal solution to \eqref{ITV}, there exists $z\in \R^p$ with $P_Tz=e$, $\|P_{T^\perp}z\|_{\ell_\infty/\ell_2}\le 1$ and $Dz\in\Im \Phi^*$. For $w^\prime \in \Ker \Phi$, we have 
\begin{equation*}
    \la De,w'\ra = \la D_{T}z,w'\ra = -\la D_{T^{\perp}}z,w'\ra=-\la z,D_{T^{\perp}}^*w'\ra.
\end{equation*}
It follows that  $\la De,w'\ra+\|D_{T^{\perp}}^*w'\|_{\ell_1/\ell_2}\ge 0$. Hence we get
\begin{eqnarray*}
\liminf_{t\downarrow 0,\; w'\st{{\rm Ker}\, \Phi}\to w} \dfrac{\la De,w'\ra+\|D_{T^{\perp}}^*w'\|_{\ell_1/\ell_2} }{\frac{1}{2}t} &=&\begin{cases}
0 & \text{ if } \la De,w\ra+ \|D_{T^{\perp}}^*w\|_{\ell_1/\ell_2}= 0, w\in \Ker \Phi,\\
\infty &\text{ otherwise}.
\end{cases}
\end{eqnarray*}
Since  the ``liminf'' in \eqref{Q} indeed becomes ``lim'', the latter together with \eqref{Q} and  \eqref{Q1} verifies \eqref{dom} and \eqref{d2}. \end{proof} 


%and thus combining with \eqref{KerPhi}, \eqref{DT_perp} and by the property of the limit inferior, we have
%\begin{eqnarray}\label{ed2}
 %   d^2\Psi(x_0|0)(w) &\geq& \sum_{r\in I} \left(\dfrac{\|(D^*w)_r\|^2}{\|(D^*x_0)_r\|}-\dfrac{\la (D^*w)_r,(D^*x_0)_r\ra^2}{\|(D^*x_0)_r\|^3}\right)+\iota_{\Ker\Phi}+\iota_{\CC_J(x_0)}.
%\end{eqnarray}
%Thus, $\dom{d^2\Psi(x_0|0)(w)}\subset\CC_J(x_0)\cap \Ker{\Phi}$. Conversely, for any $w\in \CC_J(x_0)\cap \Ker{\Phi}$, by choosing $w'=\lambda w$ with $\lambda=1$, we have $\iota_{\Ker\Phi}(w')=0$ and $\|D_{T^{\perp}}^*w'\|_{\ell_1/\ell_2}+\la De,w'\ra=0$, thus
%%  d^2\Psi(x_0|0)(w)&\leq&\lim_{t\downarrow 0,\; \lambda\to 1}\dfrac{\|D_T^*(x_0+tw')\|_{\ell_1/\ell_2}-\|D_T^*x_0\|_{\ell_1/\ell_2}-t\la De,w'\ra }{\frac{1}{2}t^2}\\
  % &=&\sum_{r\in I} \left(\dfrac{\|(D^*w)_r\|^2}{\|(D^*x_0)_r\|}-\dfrac{\la (D^*w)_r,(D^*x_0)_r\ra^2}{\|(D^*x_0)_r\|^3}\right).
%\end{eqnarray*}
%This together with \eqref{ed2} verifies that   $\dom{d^2\Psi(x_0|0)(w)}=\CC_J(x_0)\cap \Ker{\Phi}$ and \eqref{d2}. The proof is completed. \end{proof} 


This calculation allows us to establish the main result in this section, which gives a quantitative  characterization for unique/strong solutions to $\ell_1/\ell_2$ problem \eqref{ITV}. 

\begin{Theorem}[Characterizations for unique/strong solutions to $\ell_1/\ell_2$ problems]\label{BP12}  The following assertions are equivalent:
\begin{enumerate}[label={\rm (\roman*)}]
    \item $x_0$ is a unique solution to problem \eqref{ITV}.
    \item $x_0$ is a strong solution to problem \eqref{ITV}.
\item $x_0$ is a solution to \eqref{ITV}, $\Ker \Phi\cap \mathcal{E}\cap \Ker D^*_{T^\perp}=\{0\}$,  and 
    \begin{equation}\label{zeta}
    \zeta(e) \eqdef \disp\min_{u\in {\rm Ker}\, MD_{T^\perp}}\|(MD_{T^\perp})^\dag MD_Te-u\|_{\ell_\infty/\ell_2}<1,
    \end{equation}
where $M^*$ is a matrix forming a basis matrix to $\Ker \Phi\cap \mathcal{E}$.

\end{enumerate}
\end{Theorem}
\begin{proof} 
 We first claim that $x_0$ is a solution to \eqref{ITV} if and only if 
\begin{equation}\label{Opt}
    \Ker\Phi \cap {\rm int}\, ( \CC_{J}(x_0))=\emptyset.
\end{equation}
Indeed, $x_0$ is a solution to \eqref{ITV} if and only if $d\Psi(x_0)(w)\ge 0$ for all $w\in \R^n$. Due to the computation of $d\Psi(\ox)(w)$ in \eqref{dPhi}, $d\Psi(\ox)(w)\ge 0$ means  
\begin{equation}\label{Opt2}
\la De,w\ra+\|D^*_{T^\perp}w\|_{\ell_1/\ell_2}\ge 0\quad \mbox{for all}\quad w\in \Ker \Phi,
\end{equation}
which is equivalent to \eqref{Opt}. 

Next let us  verify the equivalence between (i) and (ii). By Theorem~\ref{Uniq}, it suffices to show that condition \eqref{Geo} implies (ii).  Note from \eqref{dom} and \eqref{d2} that if  $d^2\Psi(x_0|0)(w)\le 0$ then  $w\in \Ker \Phi \cap {\rm bd}\,  \CC_{J}(x_0)$ and $w\in \mathcal{E}.$  Since $\Ker \Phi\cap (\mathcal{E}\cap {\rm bd}\,  \CC_{J}(x_0))=\{0\}$ by \eqref{Geo}, we have  $d^2\Psi(x_0|0)(w)>0 $ for all $w\neq 0$. It follows from Lemma~\ref{Fa} that $x_0$ is a strong solution. This verifies the equivalence between (i) and (ii). 



To justify the equivalence between (i) and (iii), by  \eqref{Opt}, we only need to show that condition 
\begin{equation}\label{CD3}
    \Ker \Phi  \cap \mathcal{E}\cap {\rm bd}\,  \CC_{J}(x_0)=\{0\}
\end{equation}
 in \eqref{Geo} is equivalent to the combination  of $\Ker\Phi\cap \mathcal{E}\cap\Ker D^*_{T^\perp}=\{0\}$ and \eqref{zeta} provided that  $x_0$ is a solution to \eqref{ITV}. According to \eqref{Opt2},  \eqref{CD3} is equivalent to  the condition that there exists some $c>0$ such that 
\begin{equation}\label{h}
k(w) \eqdef \la De,w\ra+\|D^*_{T^\perp}w\|_{\ell_1/\ell_2}\ge c\|w\|\quad \mbox{for all}\quad w\in \Ker\Phi \cap \mathcal{E}.
\end{equation}
Since $x_0$ is a solution to \eqref{ITV}, there exists $v\in \R^p$ such that $v\in \partial \|D^*x_0\|_{\ell_1/\ell_2}$ and $Dv\in \Im \Phi^*$. It follows that  $D(e+P_{T^\perp}v)\in \Ker M=\Im \Phi^*+\mathcal{E}^\perp$, we have $MD_{T^\perp}v=-MDe$. It follows from \eqref{cons} that 
\[
MD_{T^\perp}(MD_{T^\perp})^\dag MD_Te=MD_Te.
\]
For any $w=M^*u\in 
\Ker \Phi\cap C$ it follows that 
\begin{eqnarray}\label{hM}\begin{array}{ll}
k(w)&=k(M^*u)=\la De,M^*u\ra+\|D^*_{T^\perp}M^*u\|_{\ell_1/\ell_2}\\
&=\la MD_Te, u\ra+\|D^*_{T^\perp}w\|_{\ell_1/\ell_2}\\
&=\la (MD_{T^\perp})^\dag MD_Te,D^*_{T^\perp}M^*u\ra+\|D^*_{T^\perp}M^*u\|_{\ell_1/\ell_2}.
\end{array}
\end{eqnarray}
Mimicking  the proof of Theorem~\ref{mtheo} by replacing $N$ there by $M$ and $\Ker \Phi$ by its subspace $\Ker \Phi\cap \mathcal{E}$, the inequality $k(w)\ge c\|w\|$ in \eqref{h} is equivalent to (iii). The proof is complete. \end{proof} 
 




It is worth noting that condition 
\begin{equation}\label{HJC}
    \Ker \Phi\cap \mathcal{E}\cap \Ker D^*_{T^\perp}=\{0\}
\end{equation}
in part (iii) is strictly weaker than  the Restricted Injectivity in Theorem~\ref{mtheo}; see  Example~\ref{Ex12}. It means that $\Phi$ is injective on the subspace $\mathcal{E}\cap \Ker D^*_{T^\perp}$. We refer \eqref{HJC} as {\em Strong Restricted Injectivity} condition. Moreover, we call the constant $\zeta(e)$ {\em Strong Source Identity}, while the condition $\zeta(e)<1$ is refered as {\em Analysis Strong Source Condition} for solution uniqueness to $\ell_1/\ell_2$ problem \eqref{BP0}.

 \begin{Remark}[Checking the Strong Restricted Injectivity and the Analysis Strong Source Condition]{\rm  Set the matrix $S \eqdef ((D^*_Tx_0)_g)_{ g\in I}$ to be an $p\times |I|$ matrix, where $|I|$ is the cardinality of $I$.  Observe from  \eqref{d2} that $w\in \mathcal{E}$ if and only if the following system 
 \[
 D^*_Tw=S\lm \mbox{ is consistent  with }\lm\in \R^{|I|}.
 \]
 Since $S$ is injective, we have $\lm=S^\dag  D^*_Tw =(S^*S)^{-1}S^*D^*_Tw$ due to \eqref{cons}. It follows that $w\in \mathcal{E}$ if and only if \begin{equation}\label{Si}
 S(S^*S)^{-1}S^*D^*_Tw-D^*_Tw=0
 \end{equation}
Note that  $S^*S={\rm diag}\, (\|(D^*_Tx_0)_g\|^2)_{b\in I}$ is an $|I|\times |I|$ diagonal matrix. Representing $S$ in terms of groups, we have 
 \[
 S(S^*S)^{-1}S^*={\rm diag\,}\left(\sum_{b\in I}\|(D_T^*x_0)_g\|^{-2}\iota_g\right)SS^*,
 \]
 where $\iota_g=(0,\ldots,0, \underbrace{1,1,\ldots,1}_\text{in $V_g$},0,\ldots,0)$ is the unit vector in $V_g$. This together with \eqref{Si} tells us that
 $\mathcal{E}$ is the kernel to the following matrix
 \begin{equation}\label{Q3}
     Q={\rm diag\,}\left(\sum_{g\in I}\|(D_T^*x_0)_g\|^2\iota_g\right)D_T^*-SS^*D_T^*\quad\mbox{with}\quad S=((D^*_Tx_0)_g)_{ g\in I}.
 \end{equation}
The Strong Restricted Injectivity \eqref{HJC} is equivalent to $\Ker\left[\begin{matrix}\Phi\\Q\end{matrix}\right]\cap \Ker D^*_{T^\perp}=\{0\}. $
 
 
 
Furthermore, $M^*$ forms a basis matrix to $\Ker\left[\begin{matrix}\Phi\\Q\end{matrix}\right]$, which is found from the SVD of $\left[\begin{matrix}\Phi\\Q\end{matrix}\right]$. It is similar to \eqref{rhoz}, $\zeta(e)$ is the optimal solution to 
\begin{equation}\label{Comz}
    \Min\quad \|z\|_{\ell_2/\ell_\infty}\quad \mbox{subject to}\quad MDz=-MDe\quad \mbox{and}\quad z\in \bigoplus_{g\in I}V_g. 
\end{equation}
So $\zeta^2(e)$ is the optimal value to the following smooth convex optimization problem 
\begin{equation}\label{zeta2}
\Min\quad  t\quad \mbox{subject to}\quad  MDz=-MDe, \quad \|z_g\|^2-t\le 0,\quad g\in I\quad  \mbox{and}\quad z\in\bigoplus_{g\in I}V_g 
\end{equation}
with $|I|G+1$ variables,  which can be solved by available packages such as \texttt{cvxopt}; see Section 6 for further discussion.
} 
\end{Remark} 



Next we show that $\zeta(e)\le \rho(e)$ when $x_0$ is an optimal solution to \eqref{ITV}. 

\begin{Proposition}[Comparison between $\rho(e)$ and $\zeta(e)$]\label{Com} Suppose that $x_0$ is an optimal solution to \eqref{ITV}. Then we have $\zeta(e)\le \rho(e)\le 1$.
\end{Proposition}
\begin{proof} 

It follows from \eqref{yz} that 
\[
ND_{T^\perp}(ND_{T^\perp})^\dag ND_Te=ND_Te\quad \mbox{and}\quad \rho(e)\le 1. 
\]
For any $w\in \Ker\Phi \cap\mathcal{E}=\Im M^*\subset \Ker\Phi=\Im N^*$, it is similar to \eqref{hM} that
\[
\la De,w\ra=\la (MD_{T^\perp})^\dag MD_Te,D^*_{T^\perp}w\ra=\la (ND_{T^\perp})^\dag ND_Te,D^*_{T^\perp}w\ra
\]
Note from the definition in \eqref{zeta} that 
\begin{eqnarray}\label{zen}\begin{array}{ll}
\zeta(e)&=\disp\sup_{\|v\|\le 1}\la -(MD_{T^\perp})^\dag MD_Te,v\ra-\iota_{\Im D^*_{T^\perp}M^*}(v)\\
&= \disp\sup_{\|v\|\le 1}\la -(ND_{T^\perp})^\dag ND_Te,v\ra-\iota_{\Im D^*_{T^\perp}M^*}(v)\\
&=\disp\min_{u\in {\rm Ker}\, MD_{T^\perp}}\|(ND_{T^\perp})^\dag ND_Te-u\|_{\ell_\infty/\ell_2}.
\end{array}
\end{eqnarray}
Since $\Ker ND_{T^\perp}\subset {\rm Ker}\, MD_{T^\perp}$, we have $\zeta(e)\le \rho(e)$. \end{proof} 




Although $\zeta(e)$ could be computed by involving $N$ via \eqref{zen}, the format in \eqref{zeta} is more preferable. This is due to the fact that the Moore-Penrose inverse $MD_{T^\perp}^\dag$ has a closed form as $(MD_{T^\perp})^* (MD_{S}(MD_{T^\perp})^*)^{-1}$  when the Strong Restricted Injectivity  \eqref{HJC} is in charged. In general, $\rho(e)$ is strictly smaller $\zeta(e)$. This fact is obtained through numerical experiments in our Section~6.


 
 







 By replacing $\zeta(e)$ by $\rho(e)$ in Theorem~\ref{BP12}, we do not need to assume $x_0$ to be an optimal solution, but we only have a sufficient condition for solution of uniqueness. %Note that this condition is not necessary as discussed in our Example~\ref{Ex12}.  
\begin{Corollary}[Sufficient condition for  solution uniqueness to $\ell_1/\ell_2$ problem]\label{CoBP} $x_0$ is the unique solution to problem \eqref{ITV} provided that $\rho(e)<1$ and both conditions $\eqref{yz}$ and \eqref{HJC} are satisfied. 
\end{Corollary}
\begin{proof} 
 It follows directly from Proposition~\ref{Sol}, Theorem~\ref{BP12}, and Proposition~\ref{Com}. \end{proof} 



 An simple upper bound for $\zeta(e)$ is
\begin{equation}\label{gamma}
\zeta(e)\le \gg(e) \eqdef \|(MD_{T^\perp})^\dag MD_Te\|_{\ell_\infty/\ell_2},
\end{equation}
which is also used in Section 6 to check solution uniqueness. The inequality is indeed strict. The following result  is straightforward from Theorem~\ref{BP12}. 


\begin{Corollary}[Sufficient condition for solution uniqueness to $\ell_1/\ell_2$ problem]\label{Corogg} Suppose that $x_0$  is an optimal solution to \eqref{ITV}. Then the Strong Restricted Injectivity \eqref{HJC} h at $x_0$ and $\gg(e)<1$ 
are sufficient for solution uniqueness at $x_0$. They become necessary conditions provided that $MD_{T^\perp}$ is injective.  
\end{Corollary}
%\begin{proof} 
 The result follows from Theorem~\ref{BP12} by noting that 
%\[
%\zeta(e)\le \|(MD_{S})^\dag MD_Te\|_{\ell_\infty/\ell_2}.
%\]
%The equality occurs when if $MD_{S}$ is injective. \end{proof} 


In the spirit of Proposition~\ref{Com}, it is possible that $x_0$ is a unique solution to \eqref{ITV} but $\rho(e)=1$. It means that the Strong Source Condition may not happen. However, the following result provides characterizations for solution uniqueness whose statement closely relates to the Strong Source Condition. 


\begin{Corollary}[Characterization for solution uniqueness to problem \eqref{ITV}]\label{LoBP} The following are equivalent:
\begin{enumerate}[label={\rm (\roman*)}]
    \item $x_0$ is the unique solution to problem \eqref{ITV}.

\item With an arbitrary $v\in \R^p$ satisfying $Dv\in \Im \Phi^*$, $P_Tv=e$, and $\|P_{T^\perp}v\|_{\ell_\infty/\ell_2}\le 1$,  the following system has only trivial solution
\[
\Phi w=0, \quad w\in \mathcal{E}, \quad \mbox{and}\quad D_{T^\perp}^*w\in \cone \{v_g|g\in L\}\times\{0_H\},
\]
where $L \eqdef \{g\in K|\; \|v_g\|=1\}$ and $H \eqdef K\setminus L.$

\end{enumerate}
\end{Corollary}
\begin{proof} 
 Pick an arbitrary $v\in \R^p$ satisfying $Dv\in \Im \Phi^*$, $P_Tv=e$, and $\|P_{T^\perp}v\|_{\ell_\infty/\ell_2}\le 1$. Such an $v$ always exists as when $x_0$ is a solution to \eqref{ITV}, i.e., $\Ker \Phi \cap {\rm int}\, \CC_{J}(x_0)=\emptyset$. We claim that 
\begin{equation}\label{D2}
    \Ker \Phi\cap {\rm bd}\, \CC_{J}(x_0)=\{w\in \Ker\Phi |\; D_{T^\perp}^*w\in \cone \{v_g|g\in L\}\times\{0_H\}\} 
    \end{equation}
with   $L=\{g\in K|\; \|v_g\|=1\}$ and $H=K\setminus L.$ For any $w\in \Ker\Phi$, note that 
\[
\begin{array}{ll}
\disp\la De,w\ra+\|D^*_{T^\perp}w\|&=\la Dv,w\ra-\la DP_{T^\perp}v,w\ra+\|D^*_{T^\perp}w\|\\
&=\disp -\la P_{T^\perp}v,D^*_{T^\perp}w\ra+\| D^*_{T^\perp}w\|_{\ell_1/\ell_2}\\
&\disp=\sum_{g\in L}\left(-\la v_g, (D^*_Tw)_g\ra+\|(D^*_Tw)_g\|\right)+\sum_{g\in H}\left(\la v_g, (D^*_Tw)_g\ra+\|(D^*_Tw)_g\|\right)\\
&\disp=\sum_{g\in L}\left(-\la v_g, (D^*_Tw)_g\ra+\|(D^*_Tw)_g\|\right)+\sum_{g\in H}\|(D^*_Tw)_g\|\ge 0.
\end{array}
\]
It follows that $w\in{\rm bd}\, \CC_{J}(x_0)$ if and only if there exist $\lm_g\ge 0 $, $g\in L$ such that $(D^*_Tw)_g=\lm_gv_g$ for any $g\in L$ and $(D^*_Tw)_g=0$ for any $g\in H$, which verifies \eqref{D2}. The equivalence between (i) and (ii) follows from   Theorem~\ref{Uniq}. \end{proof} 


%Although Corollary~\ref{LoBP} provides another characterization for solution uniqueness, using it in practice is not simple. After solving \eqref{ITV} we have 


As $\Ker\Phi\cap\mathcal{E}\cap {\rm bd}\, \CC_{J}(x_0)\subset\Ker\Phi\cap\Ker D^*_{V_H}$ with  $\disp V_H \eqdef \bigoplus_{g\in H}V_g$, the following result is straightforward from Corollary~\ref{CoBP}.
\begin{Corollary}[Sufficient condition to the solution uniqueness to problem \eqref{ITV}]\label{SufCoBP} $x_0$ is the unique solution to problem \eqref{ITV} provided that there exists some $v$ such that $Dv\in \Im \Phi^*$, $P_Tv=e$,  $\|P_{T^\perp}v\|_{\ell_\infty/\ell_2}\le1$, and that  
\begin{equation}\label{H}
\Ker\Phi\cap\Ker D^*_{V_H} =\{0\} 
\end{equation}
with $K=\{g\in J|\; \|v_g\|=1\}$,  $H=J\setminus K$, and $\disp V_H \eqdef \bigoplus_{g\in H}V_g$.
\end{Corollary}


 The sufficient condition in \cite[Proposition~7.1]{G11} is a special case of Corollary~\ref{SufCoBP} where $D^*$ is the discrete gradient operator. Moreover, \cite[Theorem~3.4]{JKL15} and \cite[Theorem~3]{RF08} even assume a stronger condition as they require $K=\emptyset$. Let us revisit Example~\ref{Ex12}. Pick any $v\in \partial \|x_0\|_{\ell_1,\ell_2}\cap \Im\Phi^*$, i.e., $v\in (0,1)\times [-1,1]\cap \span\{(1,1,0),(1,0,-1)\}$. It follows that $v=(0,1,1)$ and thus $K=\{3\}$, $H=\emptyset$, which clearly implies \eqref{H}.







%In all the results about characterizations for solution uniqueness to group-sparsity problem \eqref{ITV} up till now, we need to assume in advance that $x_0$ is an optimal solution in Theorem~\ref{BP12}. These results are particularly helpful when after solving \eqref{ITV} we have a solution and then using them to check the uniqueness. However, it is possible to characterize solution uniqueness to group-sparsity problem \eqref{BP0} without assuming initially about optimality as follows.





According to Theorem~\ref{BP12}, Theorem~\ref{SRob}, and Proposition~\ref{NRC}, solution uniqueness to group-sparsity problem \eqref{ITV} is equivalent to the robust recovery with rate $\mathcal{O}(\sqrt{\delta})$.

\begin{Corollary}[Robust recovery and solution uniqueness  for group-sparsity problems] The following statements are equivalent: 
\begin{enumerate}[label={\rm (\roman*)}]
\item $x_0$ is a unique solution to \eqref{ITV}.

\item For sufficiently small $\delta>0$, any solution $x_\delta$ to problem \eqref{BP1} with $J_0(\cdot)=\|\cdot\|_{\ell_1/\ell_2}$ satisfies $\|x_\delta-x_0\|\le \mathcal{O}(\sqrt{\delta})$ whenever $\|y-y_0\|\le \delta.$

 \item For any $c_1>0$ and sufficiently small $\delta>0$, any solution $x_\mu$ to \eqref{Las3} with $J_0(\cdot)=\|\cdot\|_{\ell_1/\ell_2}$ satisfies $\|x_\mu-x_0\|\le \mathcal{O}(\sqrt{\delta})$ whenever $\|y-y_0\|\le \delta$ and $\mu=c_1\delta$.
\end{enumerate}
\end{Corollary}
%\textcolor{red}{
%\begin{Remark}{\rm 
%\cite{V14} showed that Non-degenerate Source Condition (NDSC) and Restrictive Injectivity Condition (INJ) together imply the solution uniqueness of $x_0$ and the linear convergence rate of $x_{\mu}$ to $x_0$. It is worth to emphasize that our result in Corollary~\ref{LoBP} does not contradict \cite{V14}. In fact, the conditions (NDSC) and (INJ) are too strong for the solution uniqueness, which is showed in Example~\ref{Ex12} and Example~\ref{Ex52}.   }
% \end{Remark}
%}


From Theorem~\ref{BP12}, it is natural to raise the following question for other decomposable norm minimization problem. 
\begin{enumerate}
    \item[{\bf (Q3)}] If $x_0$ is a unique solution to \eqref{BP0}, can it be a strong solution to \eqref{BP0}? 
\end{enumerate}
The answer is Yes for $\ell_1/\ell_2$ problem as in Theorem~\ref{BP12}. For the $\ell_1$ problem when $\|\cdot\|_\AA=\|\cdot\|_1$, we also have the positive answer due to Corollary~\ref{ell2}. However, it is not the case for the  nuclear norm minimization problem. The following example modifies \cite[Example~3.1]{BLN19} to prove that claim. 


\begin{Example}[Difference between unique solution and strong solution to NNM]\label{Last}  
{\rm Consider the following optimization problem 
\begin{equation}\label{Impo}
\min_{X\in\R^{2\times 2}} \|X\|_* \quad\text{ subject to }\quad \Phi(X) \eqdef \left[\begin{array}{c}
     X_{11}+X_{22}  \\
     X_{12}-X_{21}+X_{22} 
\end{array}\right]=\left[\begin{array}{c}
     1  \\
     0
\end{array}\right].
\end{equation}
For any $X=\left[\begin{array}{cc}
     a &b  \\
     c &d
\end{array}\right]$ with $a+d=1$ and $b-c+d=0$, we obtain from \eqref{nucl} that 
\[
\|X\|_*=\sqrt{a^2+b^2+c^2+d^2+2|ad-bc|}\ge \sqrt{|a+d|^2+|b-c|^2}\ge 1,
\]
where the equality occurs when $\|X\|_*=1$, $b-c=0$, $a+d=1$, and $b-c+d=0$,  which means $b=c$, $a=1$, $d=0$, and  $\|X\|_*=\sqrt{1+b^2+c^2+2|bc|}=1$. So $\Bar X=\left[\begin{array}{cc}
     1 &0  \\
     0 &0
\end{array}\right]$ is the unique solution to problem \eqref{Impo}. Choose $X_\ve=\left[\begin{array}{cc}
     1-\ve^{1.5}&\ve-\ve^{1.5}   \\
     \ve &\ve^{1.5}
\end{array}\right]$ with $\ve>0$ sufficiently small and note that $X_\ve$ satisfies the equation in \eqref{Impo}. It follows that 
\[\begin{array}{ll}
\|X_\ve\|_*-\|\Bar X\|_*&=\disp\sqrt{(1-\ve^{1.5})^2+(\ve-\ve^{1.5})^2+\ve^2+\ve^3+2|(1-\ve^{1.5})\ve^{1.5}-(\ve-\ve^{1.5})\ve|}-1\\
&=\disp\sqrt{(1-\ve^{1.5})^2+(\ve-\ve^{1.5})^2+\ve^2+\ve^3+2(1-\ve^{1.5})\ve^{1.5}-2(\ve-\ve^{1.5})\ve}-1\\
&=\disp\sqrt{1+\ve^3}-1=O(\ve^3)
\end{array}
\]
Moreover, $\|X_\ve-\Bar X\|_F^2=\ve^3+(\ve-\ve^{1.5})^2+\ve^2+\ve^3=O(\ve^2)$. This tells us that $\Bar X$ is not a strong solution to \eqref{Impo}. 
}
\end{Example}



Finally, let us consider a particular case of problem \eqref{Las0}
\begin{equation}\label{Las12}
    \Min\quad \Theta(x) \eqdef f(\Phi x)+\mu\|D^*x\|_{\ell_1/\ell_2}
\end{equation}
with constant $\mu>0$. In the following result, we show that  a unique solution to \eqref{Las12} is also a strong solution.  Consequently, all the characterizations for solution uniqueness to \eqref{ITV} in this section can be used to characterize unique/strong solutions to problem \eqref{Las12} due to Proposition~\ref{Stheo}. Moreover, this result gives an affirmative answer for {\bf (Q2)} in the previous section.

\begin{Theorem}[Characterization to solution uniqueness to $\ell_1/\ell_2$ regularized problem]\label{Las2} Suppose that $\ox$ is an optimal solution to problem \eqref{Las12}. The following are equivalent:
\begin{enumerate}[label={\rm (\roman*)}]
\item $\ox$ is the unique solution to \eqref{Las12}.

\item $\ox$ {is} the strong solution to \eqref{Las12}.

\item $\ox$ is the strong solution to \eqref{ITV} with $x_0=\ox$.
\end{enumerate}

\end{Theorem}
\begin{proof} 
 (i) and (iii) are equivalent due to Proposition~\ref{Stheo} and Theorem~\ref{BP12}. [(ii)$\Rightarrow$(i)] is trivial. It suffices to verify [(iii)$\Rightarrow$(ii)]. Suppose that $\ox$ is a strong solution to \eqref{ITV}. By Theorem~\ref{BP12} and Theorem~\ref{Uniq}, $\Ker \Phi\cap \mathcal{E}\cap {\rm bd}\,\CC_{J}(x_0)=\{0\}$.  Since $\ox$ is an optimal solution to \eqref{Las2}, we have $$0\in \partial \Theta(\ox)=\Phi^*\nabla f(\Phi \ox)+D\partial\|D^*\ox\|_{\ell_1/\ell_2}\subset D\partial\|D^*\ox\|_{\ell_1/\ell_2}+\Im\Phi^*.$$ Thus there exists $\oz\in \partial\|D^*\ox\|_{\ell_1/\ell_2}$ such that $D\oz=-\Phi^*\nabla f(\Phi \ox)$, $P_T\oz=e$, and $\|P_{T^\perp}\oz\|_{\ell_\infty/\ell_2}\le 1$, where $e,T$, and $I$ are defined at the beginning at the section with $x_0=\ox$.


For any $w\in \R^n$, note further that 
\begin{equation}\label{Stro}
d^2\Theta(\ox|0)(w)=\la \Phi w,\nabla^2f(\Phi\ox)\Phi w\ra+d^2 J(\ox|\; D\oz)(w)
\end{equation}
with $J(x)=\|D^*x\|_{\ell_1/\ell_2}$. Since $D^*_{T^\perp}\ox=0$, we have
\[\begin{array}{ll}
&d^2 J(\ox|\; D\oz)(w)\disp=
\liminf_{t\downarrow 0,\; w'\to w}\dfrac{\|D^*(\ox+tw')\|_{\ell_1/\ell_2}-\|D^*\ox\|_{\ell_1/\ell_2}(\ox)-t\la D\oz,w'\ra}{\frac{1}{2}t^2}\\
&\disp=\liminf_{t\downarrow 0,\; w'\to w}\left(\dfrac{\|D_T^*(x_0+tw')\|_{\ell_1/\ell_2}-\|D_T^*x_0\|_{\ell_1/\ell_2}- t\la De,w'\ra }{{\frac{1}{2}t^2}}+\dfrac{{-}\la D_{T^\perp}\oz,w'\ra {+} \|D_{T^\perp}^*w'\|_{\ell_1/\ell_2}}{\frac{1}{2}t}\right).
\end{array}
\]
Note further that 
\[
-\la D_{T^\perp}\oz,w'\ra +\|D_{T^\perp}^*w'\|_{\ell_1/\ell_2}= -\la P_{T^\perp}\oz,D_{T^\perp}^*w'\ra+\|D_{T^\perp}^*w'\|_{\ell_1/\ell_2}\ge 0
\]
as $\|P_{T^\perp}\oz\|_{\ell_\infty/\ell_2}\le 1$. 
It is similar to \eqref{Q1} and \eqref{Q} that 
\begin{eqnarray}
\dom d^2 J(\ox|\; D\oz)&=&\{w\in \R^n|\; - \la DP_{T^\perp}\oz,w\ra +\|D_{T^\perp}^*w\|_{\ell_1/\ell_2}=0\} \eqdef \mathcal{F},\label{d21}\\
d^2 J(\ox|\; D\oz)(w)&=&\sum_{g\in I}\dfrac{\|(D_T^*w)_g\|^2}{\|(D_T^*x_0)_g\|}-\dfrac{\la (D_T^*w)_g,(D_T^*x_0)_g\ra^2}{\|(D_T^*x_0)_g\|^3}.\label{d22}
\end{eqnarray}
Since $\nabla^2f(\Phi \ox)\succ 0$, we derive from \eqref{Stro}, \eqref{d21}, and \eqref{d22} that  
\begin{equation*}
\Ker d^2\Theta(\ox|0)=\Ker \Phi\cap \mathcal{E}\cap \mathcal{F}. 
\end{equation*}
Furthermore, with  $w\in \Ker \Phi$ we have $\Phi w=0$ and 
\[
\la DP_{T^\perp}\oz,w\ra=\la D\oz,w\ra-\la De,w\ra=\la -\Phi^*\nabla f(\Phi \ox),w\ra-\la De,w\ra=-\la De,w\ra.
\]
This together with \eqref{d21} implies that  $$\Ker d^2\Theta(\ox|0)=\Ker \Phi\cap \mathcal{E}\cap \mathcal{F}=\Ker \Phi\cap \mathcal{E}\cap {\rm bd}\,\CC_{J}(x_0)=\{0\}.$$ By Lemma~\ref{Fa}, $\ox$ is a strong solution to problem \eqref{Las12}. The proof is complete.  \end{proof} 





==> tex_220921/sec_unique.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Unique, sharp, and strong solutions for robust recovery}
\label{sec:unique}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uniqueness and robust recovery}
Let us consider the optimization problem in \eqref{BP0}
% \begin{equation*}\label{ABP}
%     \min\quad J(x)\quad \mbox{subject to}\quad \Phi x=\Phi x_0,
% \end{equation*}
where we suppose that $J:\R^n \to \oR$ is a non-negative lsc function but not necessarily convex. We denote by $J_\infty: \R^n \to \oR$ the {\em asymptotic (or horizon) function} \cite{AT03} associated with $J$, which is defined by
\begin{equation}\label{AF}
J_\infty(w) \eqdef \liminf_{w^\prime \to w, t\to \infty}\dfrac{J(tw^\prime)}{t} .
\end{equation}
Throughout this section, we assume that $J$ satisfies 
\begin{equation}\label{AC}
\Ker J_\infty\cap \Ker \Phi=\{0\},
\end{equation}
where $\Ker J_\infty \eqdef \enscond{w\in \R^n}{J_\infty(w)=0}$, and the range of $J_\infty$ is on $\R_+$ since $J$ is non-negative. It then follows from \cite[Corollary~3.1.2]{AT03} that \eqref{AC} ensures that problem \eqref{BP0} has a non-empty compact set of minimizers. 

Define $\Psi:\R^n\to \oR$ as
\begin{equation}\label{Psi}
\Psi(x) \eqdef  J(x)+\iota_{\Phi^{-1}(\Phi x_0)}(x)\quad \mbox{for all}\quad x\in \R^n.
\end{equation}
We say that $x_0$ is a unique, sharp, or strong solution to \eqref{BP0} if it is a unique, sharp, or strong solution to the function $\Psi$, respectively. 


Our first result shows that solution uniqueness is a sufficient for robust recovery. If $J$ is also convex, then uniqueness is also necessary. The sufficiency part of our result generalizes the corresponding part of \cite[Theorem~3.5]{HKPS07} to nonconvex problems. 
%When the observation $\Phi x_0=y_0$ is disrupted by small noise, the problems \eqref{BP1} and \eqref{Las3} are usually used to recover $x_0$. 
%We have the stage of {\em robust recovery} if any solutions to these two problems are close to the original signal $x_0$ when $\|y-y_0\|, \mu,\delta$ are near to $0$. Robust recovery has been studied extensively in the literature, especially the area of Inverse Problem and Compressive Sensing; see, e.g., \cite{FR13, FPVDS13,GHS11,ZYY16}. In the case $\ell_1$ problem, i.e., $\|\cdot\|_\AA=\|\cdot\|_1$, \cite[Theorem~4.7]{GHS11} shows that solution uniqueness to problem \eqref{BP0} plays a crucial role in robust recovery. The original proof for this fact is nontrivial and lengthy by involving Bregman distance and several deep characterizations for solution uniqueness to $\ell_1$ problems. In the  $\ell_1$ framework, $x_0$ is a unique solution to \eqref{BP0} if and only if it is a sharp solution due to the polyhedral structure there.  For more general settings, this equivalence is invalid (see, e.g.,  Example~\ref{Ex12}), but sharp solutions and strong solutions always imply solution uniqueness. In this section we mainly show that sharp solutions and strong solutions guarantees robust recovery, of course, with different rate. This is one of the main motivations for us to have more studies  about sharp and strong minima in the later sections.        



%This section devotes to the study for sharp minima to problem \eqref{BP0}. Besides known importance of sharp minima in optimization and algorithm, the first result in this section highlights its essential in the area of robust recovery. 


\begin{Proposition}[Solution uniqueness for robust recovery]\label{NRC} Suppose that $J$ is a non-negative lsc function which satisfies \eqref{AC}. 
\begin{enumerate}[label={\rm (\roman*)}]
\item If $x_0$ is the unique solution to problem \eqref{BP0} then: \label{NRC:item1}
\begin{enumerate}[label={\rm (\alph*)}]
\item any solution $x_\delta$ to problem \eqref{BP1} with $\|y-y_0\| \le \delta$ converges to $x_0$ as $\delta \to 0$, \label{NRC:item1a}
    
\item for any constant $c_1>0$, any solution $x_{\mu}$ to problem \eqref{Las3} with $\mu=c_1\delta$ and $\|y-y_0\|\le \delta$ converges to $x_0$ as $\delta \to 0$. \label{NRC:item1b}
\end{enumerate}
\item Conversely, if $J$ is convex and $\dom J = \R^n$, then: \label{NRC:item2}
\begin{enumerate}[label={\rm (\alph*)}] 
\item if for any $\delta > 0$, $\exists u \in \Im(\Phi)$ such that $\norm{y-u} < \delta$ (which is for instance the case if $y \in \Im(\Phi)$), then \ref{NRC:item1}-\ref{NRC:item1a} implies $x_0$ is the unique solution to \eqref{BP0}. 
\item \ref{NRC:item1}-\ref{NRC:item1b} implies $x_0$ is the unique solution to \eqref{BP0}. 
\end{enumerate}
\end{enumerate}
\end{Proposition}
\begin{proof} 
\begin{enumerate}[label={\rm (\roman*)}]
\item Suppose that $x_0$ is the unique solution to problem \eqref{BP0}. To justify \ref{NRC:item1}-\ref{NRC:item1a}, define the function $g \eqdef \iota_{\B_\delta(y)} \circ \Phi$. We have, using \cite[Propositions~2.6.1, 2.6.3 and 2.1.2]{AT03}, that
\begin{eqnarray*}
(J+g)_\infty(w) \geq J_\infty(w)+g_\infty(w) = J_\infty(w)+(\iota_{\B_\delta(y)})_\infty(\Phi w) 
&=& J_\infty(w)+\iota_{\{0\}}(\Phi w) \\
&=& J_\infty(w)+\iota_{\Ker \Phi}(w) \geq 0 .
\end{eqnarray*}
Thus, under \eqref{AC}, the set of solutions to \eqref{BP1} is nonempty and compact thanks to \cite[Corollary~3.1.2]{AT03}. If $\{x_\delta\}_{\delta>0}$ is unbounded, without passing to subsequences suppose that $\|x_\delta\|\to \infty$ and  $\dfrac{x_\delta}{\|x_\delta\|} \to w$ as $\delta \dn 0$ with $\|w\|=1$. We have
\[ 
0 \le \anorm{\Phi \pa{\frac{x_\mu}{\|x_\mu\|}}-\frac{y}{\|x_\mu\|}} \le \frac{\delta}{\|x_\mu\|},
\] 
and after passing to the limit, we get that $w\in \Ker \Phi$. Moreover, since $x_0$ is a feasible point of \eqref{BP1}, we have $J(x_\delta) \le J(x_0)$, and thus
\[
0=\liminf_{\delta\dn 0}\dfrac{J(x_0)}{\|x_\delta\|}\ge \liminf_{\delta\dn 0}\dfrac{J(x_\delta)}{\|x_\delta\|}\ge J_\infty(w)\ge 0, 
\]
which means that $w \in \Ker J_\infty$. This entails that  $0 \neq w \in \Ker J_\infty\cap \Ker \Phi$, which  contradicts \eqref{AC}. Thus $\{x_\delta\}_{\delta>0}$ is bounded. Pick any subsequence $\{x_{\delta_k}\}_{k \in \N}$ of $\{x_\delta\}_{\delta>0}$ converging to some $\bar{x}$ as $\delta_k \dn 0$. From lower semicontinuity of $J$ and of the norm, we get
\[
J(\bar{x}) \leq \liminf_{k} J(x_{\delta_k}) \leq J(x_0) \qandq 0 \leq \norm{y_0 - \Phi\bar{x}} \leq \liminf_{k} \norm{y_0 - \Phi x_{\delta_k}} \leq 2 \lim_{k} \delta_k = 0 .
\]
This means that $\bar{x}$ is a solution of \eqref{BP0}, and by uniqueness of the minimizer, $\bar{x}=x_0$. Since the subsequence $\{x_{\delta_k}\}_{k \in \N}$ was arbitrary, we have $x_\delta \to x_0$ as $\delta\dn 0$, whence claim \ref{NRC:item1}-\ref{NRC:item1a} follows.\\

The proof of \ref{NRC:item1}-\ref{NRC:item1b} uses a similar reasoning. Let $g = \frac{1}{2}\norm{y-\cdot}^2 \circ \Phi$. One has, using \cite[Propositions~2.6.1, 2.6.3 and 2.6.7]{AT03}, that
\begin{eqnarray*}
(\mu J+g)_\infty(w) \geq \mu J_\infty(w)+g_\infty(w) = \mu J_\infty(w)+\frac{1}{2}\pa{\norm{\cdot}^2}_\infty(\Phi w) 
&=& \mu J_\infty(w)+\iota_{\{0\}}(\Phi w) \\
&=& \mu J_\infty(w)+\iota_{\Ker \Phi}(w) \geq 0 .
\end{eqnarray*}
Hence the set of optimal solutions to problem \eqref{Las3} is nonempty and compact according to \cite[Corollary~3.1.2]{AT03}. Similarly to part \ref{NRC:item1}-\ref{NRC:item1a}, we claim that  $\{x_\mu\}_{\mu > 0}$ is bounded. By contradiction, suppose again that $\|x_\mu\|\to \infty$  and $ \dfrac{x_\mu}{\|x_\mu\|} \to z$ with $\|z\|=1$. Note that by optimality of $x_\mu$
\begin{equation}\label{Sim}
\mu J(x_\mu) \leq \frac{1}{2}\|\Phi x_\mu-y\|^2+\mu J(x_\mu) \leq \frac{1}{2}\|\Phi x_0-y\|^2+\mu J(x_0) \leq \frac{\delta^2}{2}+\mu J(x_0) .
\end{equation}
As $\mu=c_1\delta$, we obtain from \eqref{Sim} that 
\[
0=\liminf_{\delta\dn 0}\dfrac{J(x_0)+\frac{\delta}{2c_1}}{\|x_\mu\|}\ge \liminf_{\delta\dn 0}\dfrac{J(x_\mu)}{\|x_\mu\|}\ge J_\infty(z)\ge 0, 
\]
which means $z\in \Ker J_\infty$. Furthermore, \eqref{Sim} also entails 
\[
0\le \frac{1}{2}\anorm{\Phi\pa{\frac{x_\mu}{\|x_\mu\|}}-\frac{y}{\|x_\mu\|}}^2 \le \frac{1}{\|x_\mu\|^2 } \pa{\frac{\delta^2}{2}+\mu J(x_0)},
\]
which tells us, after passing to the limit, that $0 \neq z \in \Ker J_\infty \cap \Ker \Phi $, hence contradicting \eqref{AC}. Thus $\{x_\mu\}_{\mu > 0}$ is bounded. Arguing as in \ref{NRC:item1}-\ref{NRC:item1a}, we use lower semicontinuity of $J$ and of the norm to show that any cluster point of $\{x_\mu\}_{\mu > 0}$ is a solution of \eqref{BP0}, and deduce claim \ref{NRC:item1}-\ref{NRC:item1b} thanks to uniqueness of the minimizer $x_0$.
%Let $\{x_{\mu_q}\}$ be an arbitrary subsequence of $\{x_\mu\}$ converging to some $v_0$. Taking $\delta\to 0$, we derive from \eqref{Sim} that $J(x_0)\ge J(v_0)$ and $\Phi v_0=y_0$. Since $x_0$ is the unique solution to problem \eqref{BP0}, $x_0=v_0$. As the  subsequence $\{x_{\mu_q}\}$ is arbitrary,  $\{x_\mu\}$ converges to $x_0$ as $\delta\dn 0$. This verifies \ref{NRC:item2}. 

\item Suppose now that $J$ is also convex and $\dom J = \R^n$ (hence continuous). If \ref{NRC:item1}-\ref{NRC:item1a} holds, we have 
\begin{equation}\label{BP4}
J(x_\delta) \leq J(x) \qforanyq x \qstq \|y - \Phi x\| \le \delta \qandq \|y-y_0\|\le \delta.
\end{equation}
It follows that 
\[
J(x_\delta) \leq J(x) \qforanyq x \qstq \Phi x=y_0.
\]
By letting $\delta\dn 0$, and using continuity of $J$, we obtain that $x_0$ is a minimizer to \eqref{BP0}. Let $\ox$ be an arbitrary minimizer to problem \eqref{BP0}. As $\dom J=\R^n$, Fermat's rule for \eqref{BP0} and subdifferential calculus gives
\[
0\in \partial \Psi(\ox)=\partial J(\ox)+N_{\Phi^{-1}y_0}(\ox)=\partial J(\ox)+\Im \Phi^*.
\]
Or, equivalently, there exists a dual multiplier $\eta\in \R^m$ such that $\Phi^*\eta\in \partial J(\ox)$\footnote{This is known as the source condition.}. If $\eta=0$, we have $0\in  \partial J(\ox)$, which means that $\ox$ is a minimizer to 
$J$. Thus, $\ox$ is also a minimizer to problem \eqref{BP1} for any $\delta>0$. By \ref{NRC:item1}-\ref{NRC:item1a}, $\ox-x_0\to 0$ as $\delta\dn 0$, i.e., $\ox=x_0$. 

If $\eta\neq 0$, take any $\delta>0$ and define $\mu \eqdef \dfrac{\delta}{\|\eta\|}$ and $y \eqdef y_0+\mu \eta=\Phi \ox+\mu \eta$. It follows that $\|y - \Phi\ox\| = \|y - y_0\| = \delta$ and that
\begin{equation}\label{eq:fermatox}
\frac{1}{\mu}\Phi^*(y - \Phi\ox)= \Phi^*\eta\in \partial J(\ox).
\end{equation}
On the other hand, under our assumption, we have that $x^\star$ is a solution to \eqref{BP1} if and only if
\[
0 \in \partial J(x^\star)  + \Phi^* N_{\B_\delta(y)}(\Phi x^\star) ,
\]
where $N_{\B_\delta(y)}(\Phi x^\star) = \R_+(y-\Phi x^\star)$ whenever $\norm{y-\Phi x^\star}=\delta$. This is precisely the optimality condition verified by $\ox$ in \eqref{eq:fermatox}, which shows that $\ox$ is also a solution to \eqref{BP1}. By \ref{NRC:item1}-\ref{NRC:item1a} again, we have $\ox=x_0$. Since the choice of  $\ox$ is arbitrary, $x_0$ is the unique solution to \eqref{BP0}.

Finally, suppose that \ref{NRC:item1}-\ref{NRC:item1b} is satisfied. We have for any $x \in \Phi^{-1}y_0$ that
\[
\mu J(x_\mu) \leq \frac{1}{2}\|\Phi x-y\|^2+\mu J(x) \leq \frac{\delta^2}{2}+\mu J(x) .
\]
Dividing both sides by $\mu=c_1\delta$ and letting $\delta\to 0$ entails $J(x_0) \leq J(x)$ for any  $x\in \Phi^{-1}y_0$, which is equivalent to saying that $x_0$ is a solution to problem \eqref{BP0}. The proof of uniqueness follows similar lines as for problem \eqref{BP1} with the choice $y = \Phi \ox + \mu \eta$ and $\mu=c_1\delta$. Note that under our assumption, Fermat's rule for problem \eqref{Las3} is \eqref{eq:fermatox} without further qualification condition unlike what is required for \eqref{BP1}.
\end{enumerate}
\end{proof} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sharp minima and robust recovery}

A sufficient and necessary condition for uniqueness to problem \eqref{BP0}, together with its implication for robust recovery, is studied in \cite{CRPW12} via the key geometric notion of {\em descent cone} that we recall now.
%
\begin{Definition}[Descent cone] The descent cone of the function $J$ at $x_0$ is defined by 
\begin{equation}\label{Des}
\TT_J(x_0) \eqdef \cone\enscond{x-x_0}{J(x) \le J(x_0)} .
\end{equation}
\end{Definition}
 
The following proposition provides a characterization for solution uniqueness whose proof can be found in \cite[Proposition~2.1]{CRPW12}.

\begin{Proposition}[Descent cone for solution uniqueness \cite{ALMT14,CRPW12}]\label{DeUn} 
$x_0$ is a unique solution to \eqref{BP0} if and only if $\Ker \Phi \cap \TT_J(x_0)=\{0\}$. 
\end{Proposition}

In \cite[Proposition~2.2]{CRPW12} (see also \cite[Proposition~2.6]{Tropp15}), the authors also prove a robust recovery result for solutions of \eqref{BP1} via the descent cone. %Since our problem \eqref{BP0} is slightly different  from the model in \cite{CRPW12}, we provide a short proof.

\begin{Proposition}[Robust recovery via descent cone \cite{CRPW12}] \label{Pop} 
Suppose that there exists some $\al>0$ such that $\|\Phi w\|\ge \al\|w\|$ for all $w\in \TT_J(x_0)$. Then any solution $x_\delta$ to problem \eqref{BP1} satisfies
\begin{equation}\label{Est7}
\|x_\delta-x_0\|\le  \frac{2\delta}{\al}.
\end{equation}
\end{Proposition}

The parameter $\alpha$ is known as the minimum conic singular value of $\Phi$ with respect to the cone $\TT_J(x_0)$. One may observe that the condition in Proposition~\ref{Pop} is not the same with the one for solution uniqueness in Proposition~\ref{DeUn}. The reason is that the descent cone $\TT_J(x_0)$ is not necessarily closed in general. To see this, we first unveil the relation between the descent and {\em critical} cones. Denote 
\begin{equation*}
L_{x_0}(J) \eqdef \enscond{x\in \R^n}{J(x)\le J(x_0)}
\end{equation*}
the {\em sublevel set} of $J$ at $x_0$. The {\em critical cone} of $J$ at $x_0$ is 
\begin{equation}\label{D0}
\CC_J(x_0) \eqdef \enscond{w\in \R^n}{dJ(x_0)(w)\le 0} .
\end{equation} 

\begin{Lemma}
Suppose that $J$ is a continuous convex function and $0\notin \partial J(x_0)$. Then
\[
\cl (\TT_J(x_0)) = \CC_J(x_0).
\]
\end{Lemma}

\begin{proof}
We have from \eqref{Dual} that  
\begin{equation}\label{ClD}
\cl (\TT_J(x_0))=(\TT_J(x_0))^{\circ\circ}=\pa{(\cl \TT_J(x_0))^{\circ}}^\circ=(N_{L_{x_0}(J)}(x_0))^\circ=(\cone \partial J(x_0))^\circ=\CC_J(x_0),
\end{equation}
where we used \eqref{Dual} in the first two equalities, polarity in the third, and \cite[Corollary~23.7.1]{R70} and \cite[Proposition~10.3]{RW98} in the last two equalities.
\end{proof}

% \begin{proof} 
% Suppose that $x_0$ is the unique solution to \eqref{BP0} but $0 \neq w \in \Ker \Phi \cap \TT_\AA(x_0)$. Hence there exists some $t>0$ such that $J(x_0+tw) \le J(x_0)$ and $\Phi(x_0+tw)=\Phi x_0$, or equivalently that $x_0+tw$ is a solution \eqref{BP0}, contradicting uniquness of $x_0$. Conversely, suppose that $x_0$ is not a unique solution but $\Ker \Phi \cap \TT_\AA(x_0) = \{0\}$. We know then that there exists $\ox \neq x_0$ such that $J(\ox) \leq J(x_0)$ and $\ox - x_0 \in \Ker \Phi$. This implies that $\ox-x_0\in \Ker \Phi \cap \TT_\AA(x_0) \neq \{0\}$, leading again to a contradiction. The proof is complete. 
% \end{proof} 

In the case $J(x)=\|D^*x\|_\AA$, where $\|\cdot\|_\AA$ is a norm in $\R^p$ and $D$ is an $n\times p$ matrix, we show next that \eqref{CD2} holds without the condition $0\notin \partial J(x_0)$.

\begin{Proposition}[Relationship between descent cone and critical cone] Suppose that  $J(x)=\|D^*x\|_\AA$, where $\|\cdot\|_\AA$ is any norm in $\R^p$, we have
\begin{equation}\label{CD4}
   \cl (\TT_J(x_0))=\CC_J(x_0). 
\end{equation}
\end{Proposition}
\begin{proof} 
 Note that $0$ is the minimum value of  $J$. If $J(x_0)>0$, we have $0\notin \partial J(x_0)$. Thus \eqref{CD4} holds by \eqref{CD2}.  If $J(x_0)=0$, we have $x_0\in \Ker D^*$, $L=\Ker D^*$, $\TT_J(x_0)=\Ker D^*$, and that 
\[
\partial J(x_0)=\{Dv|\; \|v\|^*_{\AA}\le 1, v\in \R^p\},\]
where $\|\cdot\|^*_{\AA}$ is the dual norm of $\|\cdot\|_\AA$.  This  gives us \[
N_L(x_0)=(\Ker D^*)^\perp=\Im D=\cone \partial J(x_0).
\]
Hence \eqref{ClD} is also satisfied. This verifies \eqref{CD4} and completes the proof. \end{proof} 
 




If the descent cone $\TT_J(x_0)$ is closed, it is $\CC_J(x_0)$. But in general, $\TT_J(x_0)$ is not closed. 

We show next that the condition in Proposition~\ref{Pop} actually means that $x_0$ is a sharp solution to \eqref{BP0}. 

\begin{Proposition}[Characterizations for sharp minima via descent cone and critical cone]\label{Shar} Let $J$ be a continuous convex function. The following are equivalent:
\begin{enumerate}[label={\rm (\roman*)}]
    \item $x_0$ is a sharp solution to \eqref{BP0}.
    \item $\Ker \Phi\cap \CC_J(x_0)=\{0\}.$
\end{enumerate}
If additionally, $J(x)=\|D^*x\|_\AA$ then {\rm (i)} holds if and only if  there exists $\al>0$ such that $\|\Phi w\|\ge \al\|w\|$ for all $w\in \TT_\AA(x_0)$.
\end{Proposition}
\begin{proof} 
 By Lemma~\ref{Fa}, $x_0$ is a sharp solution to \eqref{BP0} if and only if $d\Psi (x_0)(w)>0$ for all $w\in \R^n\setminus\{0\}$. Observe that 
\begin{equation}\label{dP}
    d\Psi (x_0)(w)=\lim_{t\dn 0}\dfrac{J(x_0+tw)-J(x_0)}{t}+\iota_{{\rm Ker}\, \Phi}(w)=dJ(x_0)(w)+\iota_{{\rm Ker}\, \Phi}(w).
\end{equation}
This together with Lemma~\ref{Fa} verifies the equivalence between (i) and (ii). 

Finally, let us consider the special case when $J(x)=\|D^*x\|_{\AA}$. If  (ii) holds,  there exists $\al>0$ such that $\|\Phi w\|\ge \al\|w\|$ for all $w\in \CC_J(x_0)$, since $\CC_J(x_0)$ is closed. As $\TT_J(x_0)\subset \CC_J(x_0)$ by \eqref{CD4}, we get $\|\Phi w\|\ge \al\|w\|$ for all $w\in \TT_J(x_0)$. Conversely, if there is $\al>0$ such that $\|\Phi w\|\geq \al\|w\|$ for all $w\in \TT_J(x_0)$, we have 
$\|\Phi w\|\ge \al\|w\|$ for all $w\in \CC_J(x_0)$ due to \eqref{CD4}. It follows that $\Ker \Phi\cap \CC_J(x_0)=\{0\}$. By  the equivalence between (i) and (ii), $x_0$ is a sharp solution to \eqref{BP0}. \end{proof} 


From Proposition~\ref{DeUn} and Proposition~\ref{Shar}, we observe that the difference between solution uniqueness and sharp minima for problem \eqref{BP0} relies on the closedness of the descent cone. The following  example shows that the descent cone for group-sparsity problem is not closed. This can be seen from our precise calculation for the descent cone in Theorem~\ref{Uniq}, at which the interior of the critical cone $\CC_J(x_0)$ plays a significant role. This example reconfirms  that the condition in Proposition~\ref{Pop} is different from the one in Proposition~\ref{DeUn}. 


\begin{Example}[Difference between unique solution and sharp solution for group-sparsity problems]\label{Ex12}{\rm  Consider the following $\ell_1/\ell_2$ optimization problem:
\begin{equation}\label{Ex123}
\Min\quad J(x)=\sqrt{x_1^2+x_2^2}+|x_3|\quad \mbox{subject to}\quad \Phi x=\Phi x_0
 \end{equation}
with $\Phi=\left[\begin{array}{ccc}1& 1 &0\\ 1& 0 &-1\end{array}\right]$, $x_0=(0,1,0)^T$, and $y_0=\Phi x_0=(1,0)^T$. For any $x=(x_1,1-x_1,x_1)^T\in \Phi^{-1}y_0$, we have 
\begin{eqnarray*}
J(x)-J(x_0)=\sqrt{x_1^2+(1-x_1)^2}+|x_1|-1=\dfrac{x_1^2+2(|x_1|-x_1)}{\sqrt{x_1^2+(1-x_1)^2}+1-|x_1|},
\end{eqnarray*}
which tells us that $x_0$ is a unique/strong solution to \eqref{Ex12} but is not a sharp solution.  The following figure illustrates the difference between the descent cone computed in Theorem~\ref{Uniq} and the critical cone \eqref{CD2}. It is obvious that $\Ker \Phi\cap \CC_J(x_0)\neq \{0\}$,  but $\Ker \Phi\cap \TT_J(x_0)= \{0\}$. 
\begin{figure}[!ht]
 \centering
\includegraphics[width=0.5\linewidth]{example36.png}
 \caption{The descent cone $\TT_J (x_0)=(\mathcal{E}\cap{\rm bd}\, \CC_J(x_0))\cup\mathrm{int}\,(\CC_J(x_0))$ with $\mathcal{E}=\{(0,x_2,x_3)|\; x_2, x_3 \in\R\}$ and $\CC_J(x_0)=\{(x_1,x_2,x_3)|\; x_2+|x_3|\leq 0\}$.}
\label{fig:signal}
 \end{figure}
}
\end{Example}


%\[
%\lim_{x_1\downarrow 0}\dfrac{J(x)-J(x_0)}{\|x-x_0\|}=\lim_{x_1\downarrow 0}\dfrac{x_1}{\sqrt{3}(\sqrt{x_1^2+(1-x_1)^2}+1-x_1)}=0.
%\]




Inspired by Proposition~\ref{Pop}, we show next that sharp minima guarantees robust recovery for both problems \eqref{BP1} and \eqref{Las3} with linear rate. Unlike \cite[Proposition~2.2]{CRPW12} and many other results \cite{FPVDS13, GHS11, V14, VPF15, ZYY16} in this direction, convexity is not assumed on $J$. We only need $x_0$ to be a unique and sharp solution to problem \eqref{BP0}. 



\begin{Theorem}[Sharp minima for robust recovery]\label{Rob} Suppose that $J$ satisfies \eqref{AC} and is Lipschitz continuous around $x_0$ with modulus $L$. If  $x_0$ is a unique and sharp solution to \eqref{BP0} with constant $c>0$, for sufficiently small $\delta>0$ the following statements hold:
\begin{enumerate}[label={\rm (\roman*)}]
\item Any solution $x_\delta$ to problem \eqref{BP1} satisfies
\begin{equation}\label{Est2}
        \|x_\delta-x_0\|\le \frac{2(L+c)\|\Phi^\dag\|}{c}\delta.
    \end{equation}
    
\item For any $c_1>0$ and $\mu=c_1\delta$,  every minimizer $x_{\mu}$ to \eqref{Las3} satisfies
\begin{equation}\label{Est}
\|x_\mu-x_0\|\le \frac{c_1}{2c} \left(\frac{1}{c_1}+(c+L)\|\Phi^\dag\|\right)^2\delta.
\end{equation}
\end{enumerate}
\end{Theorem}
\begin{proof} 
 As $J$ is Lipschitz conitnuous around $x_0$, we find  $\ve, L>0$ such that 
\begin{equation}\label{Lip}
    \|J(x)-J(u)\|\le L\|x-u\|\quad \mbox{for all}\quad x,u\in \B_\ve(x_0). 
\end{equation}
To justify (i),  suppose that $x_\delta$ is a solution to \eqref{BP1}. We have $J(x_0)\ge J(x_\delta)$. Let $\ox_\delta$ be the projection from  $x_\delta$ to $A=\Phi^{-1}y_0$. Since $x_0$ is a sharp solution to \eqref{BP0} with constant $c$, there exists $\eta>0$ such that 
\begin{equation}\label{InSharp}
    J(x)-J(x_0)\ge c\|x-x_0\|\quad \mbox{for all}\quad x\in \Phi^{-1}y_0\cap\B_\eta(x_0). 
\end{equation} 
 Since $x_0$ is a unique solution to problem \eqref{BP0},  Proposition~\ref{NRC} tells us that $x_\delta\to x_0$ as $\delta\dn 0$. Let $\ox_\delta$ be the projection of $x_\delta$ to $\Phi^{-1}y_0$. As $\|x_\delta-x_0\|\ge \|x_\delta-\ox_\delta\|$, we may assume that $\ox_\delta, x_\delta\in \B_{\min\{\ve,\eta\}}(x_0)$ with $\ve, \eta$ in \eqref{Lip} and \eqref{InSharp}. By the Lipschitz property of $J$ in \eqref{Lip}, we have 
\begin{eqnarray*}\begin{array}{ll}
L\|\ox_\delta-x_\delta\|&\ge J(\ox_\delta)-J(x_\delta)\ge\disp J(\ox_\delta)-J(x_0)\\
&\displaystyle\ge c\|\ox_\delta-x_0\|\ge c\|x_\delta-x_0\|-c\|x_\delta-\ox_\delta\|.
\end{array}
\end{eqnarray*}
This together with the projection formula \eqref{Pro} tells us that 
\[\begin{array}{ll}
c\|x_\delta-x_0\|&\disp\le (L+c)\|x_\delta-\ox_\delta\|=(L+c)\|\Phi^\dag \Phi (x_\delta -x_0)\|\\
&\disp\le(L+c)\|\Phi^\dag\|\cdot\|\Phi (x_\delta -x_0)\|\\
&\le(L+c)\|\Phi^\dag\|(\|\Phi x_\delta -y\|+\|y-\Phi x_0\|)\\
\disp&\le(L+c)\|\Phi^\dag\|2\delta,
\end{array}
\]
which verifies \eqref{Est2}.

It remains to justify (ii).  Note that 
\begin{equation}\label{Sim1}
    \frac{1}{2}\|\Phi x_0-y\|^2+\mu J(x_0)\ge \frac{1}{2}\|\Phi x_\mu-y\|^2+\mu J(x_\mu).
\end{equation}
%which tells us that $\|D^*x_\mu\|\le  J(x)+\frac{\|y-y_0\|^2}{\mu}\le  J(x)+\frac{\delta}{c_1}$ for any $x\in \Phi^{-1}\oy$. Take any subsequence  $\{x_{\mu_n}\}$ such that  $D^*x_{\mu_q}$ is converging to some $D^*u_0$. The latter inequality also implies that $\|D^*u_0\|\le  J(x)$ for any $x\in \Phi^{-1}y_0$. Hence $u_0$ is a solution to problem \eqref{BP0}. Since $x_0$ is a sharp solution to \eqref{BP0}, we have $u_0=x_0$. Note that the choice of converging subsequence $\{x_{\mu_q}\}$ is arbitrary, $D^* x_\mu \to D^*x_0$ for sufficiently small $\delta$. Since $D$ is surjective, $x_\mu \to x_0$ as $\delta\dn 0$. Without loss of generality, we suppose $\|x_\mu-x_0\|\le \ve$.
It follows that 
\begin{eqnarray*}\begin{array}{ll}
\disp\frac{\|y-y_0\|^2}{2\mu}&\disp\ge J(x_\mu)-J(x_0)+\frac{1}{2\mu}(\|\Phi(x_\mu-x_0)\|-\|y-y_0\|)^2.
%&\disp\ge J(x_\mu)-J(x_0)+\frac{1}{2\mu}\left[2r\|\Phi(x_\mu-x_0)\|\|y-y_0\|-(r^2+2r)\|y-y_0\|^2 \right],
\end{array}
\end{eqnarray*}
Hence, we have
\begin{eqnarray}\label{Low}\begin{array}{ll}
\disp\frac{2\|y-y_0\|\cdot\|\Phi(x_\mu-x_0)\|-\|\Phi(x_\mu-x_0)\|^2}{2\mu}&\disp\ge J(x_\mu)-J(x_0).
%&\disp\ge J(x_\mu)-J(x_0)+\frac{1}{2\mu}\left[2r\|\Phi(x_\mu-x_0)\|\|y-y_0\|-(r^2+2r)\|y-y_0\|^2 \right],
\end{array}
\end{eqnarray}
Since $x_0$ is the unique solution to problem \eqref{BP0}, we have $x_\mu\to x_0$ due to Proposition~\ref{NRC}(ii). Let $\ox_\mu$ be the projection of $x_\mu$ to $\Phi^{-1}y_0$. It follows that  $x_\mu,\ox_\mu\in \B_{\min\{\ve,\eta\}}(\ox)$ with $\ve,\eta$ in \eqref{Lip} and \eqref{InSharp} when $\delta$ is sufficiently small. 

Combining \eqref{InSharp} with \eqref{Pro} and \eqref{Lip} gives us that 
\begin{eqnarray*}\begin{array}{ll}
J(x_\mu)-J(x_0)&=\disp J(\ox_\mu)-J(x_0)+J(x_\mu)-J(\ox_\mu)\\
&\disp\ge c\|\ox_\mu-x_0\|-L\|x_\mu-\ox_\mu\|\\
&\disp\ge c\|x_\mu-x_0\|-(c+L)\|x_\mu-\ox_\mu\|\\
&\disp= c\|x_\mu-x_0\|-(c+L)\|\Phi^\dag \Phi(x_\mu-x_0)\|\\
&\disp\ge c\|x_\mu-x_0\|-(c+L)\|\Phi^\dag\|\cdot  \|\Phi(x_\mu-x_0)\|.
\end{array}
\end{eqnarray*}
Define $\al \eqdef \|\Phi(x_\mu-x_0)\|$, the latter together with \eqref{Low} gives us that
\begin{eqnarray}\label{beta}\begin{array}{ll}
c\|x_\mu-x_0\|&\disp\le \frac{2\delta\al-\al^2}{2\mu}+(c+L)\|\Phi^\dag\| \al\\
&=\disp \left(\frac{\delta}{\mu}+(c+L)\|\Phi^\dag\|\right)\al-\frac{\al^2}{2\mu}\\
&\disp\le\frac{\mu}{2} \left(\frac{\delta}{\mu}+(c+L)\|\Phi^\dag\|\right)^2,
\end{array}
\end{eqnarray}
which clearly verifies \eqref{Est}. The proof is complete. 
\end{proof} 



In Theorem~\ref{Rob}, the estimate \eqref{Est2} and \eqref{Est} hold when $\delta$ is sufficiently small. However, when the function $J$ is a continuous convex function, they are satisfied for any $\delta>0$.
 
 \begin{Corollary}[Sharp minima for robust recovery under convexity]\label{RobCon} Suppose that $J$ is a continuous convex function satisfying condition \eqref{AF} and $x_0$ is a sharp solution to \eqref{BP0}. Then both {\rm (i)} and {\rm (ii)} of {\rm Theorem~\ref{Rob}} hold for any $\delta>0$ with some constant $L>0$.
 \end{Corollary}
\begin{proof} 
 Let us revisit the proof of Theorem~\ref{Rob}. When $J$ is a continuous convex function and $x_0$ is a sharp solution to \eqref{BP0}, it is also a unique solution to \eqref{BP0}. Since $J$ satisfies \eqref{AC},  $\{x_\delta\},\{x_\mu\}$ are bounded as proved in Proposition~\ref{NRC}. There exists some $R>0$ such that $x_\delta,\ox_\delta, x_\mu,\ox_\mu\in \B_R(0)$. Since $J$ is a continuous convex function, it is Lipschitz continuous on $\B_R(0)$ with some Lipschitz constant $L>0$. Moreover, sharp minima is a global property under convexity. We can choose $\ve, \eta$ in \eqref{Lip} and \eqref{InSharp} by $R$. Other parts of the proof of Theorem~\ref{Rob} stay the same. \end{proof} 



\begin{Remark}\label{Relax}{\rm It is worth noting that  Corollary~\ref{RobCon} covers many results in  \cite{FPVDS13, GHS11, V14, VPF15, ZYY16}. When $J=\|\cdot\|_\AA$ is a norm in $\R^n$, part (i) of Theorem~\ref{Rob} is exactly \cite[Proposition~2.2]{CRPW12} due to Proposition~\ref{Shar}. In this case the condition \eqref{AC} holds trivially and the Lipschitz continuity $L$ of $J$ is $\|\Id\|_{\AA,2}$.   
For the case  $J=\|\cdot\|_{\ell_1}$,  Corollary~\ref{RobCon} returns \cite[Theorem~4.7]{GHS11} whose proof is more involved and based on Bregman distance together with the characterizations of solution uniqueness to $\ell_1$ optimization problem. 

When $J(x)=\|D^*x\|_\AA$ with $D$ being an $n\times p$ matrix and $\|\cdot\|_\AA$ being a norm in $\R^p$, 
Corollary~\ref{RobCon} covers \cite[Theorem~2]{FPVDS13}. Another result in this direction is \cite[Theorem~2]{ZYY16}, which only obtains linear rate for $\|D^*(x_\mu-x_0)\|$ with extra nontrivial assumptions on $D$.  In this case condition \eqref{AC} means that 
\[
\Ker D^*\cap \Ker\Phi=\{0\},
\]
which is satisfied automatically when $x_0$ is a unique solution to \eqref{BP0}. Thus, condition \eqref{AC} could be omitted in the statement of Corollary~\ref{RobCon}. Moreover,  the Lipschitz modulus $L$ of $J$ is $\|\Id\|_{\AA,2}\|D^*\|$. It seems to us that the bounds obtained in \eqref{Est2} and \eqref{Est} are more explicit than several results in \cite{FPVDS13, GHS11, ZYY16}. The only constant that is not trivial is $c$. In  Theorem~\ref{mtheo} we provide an estimation for this number via the so-called {\em Source Identity} that can be computed numerically. %The bounds in the aforementioned results  \cite{FPVDS13, GHS11, V14, VPF15, ZYY16} have  hidden constants  that are hard to estimate. 

In the case of general continuous convex regularizers as in Corollary~\ref{RobCon}, \cite{V14,VPF15} use the so-called  Restricted Injectivity and non-degenerate source condition to obtain robust recovery. Our later Theorem~\ref{mtheo} shows that  these two conditions are equivalent to sharp minima at $x_0$. It means that Corollary~\ref{RobCon} is equivalent to \cite[Theorem~6.1]{V14} or \cite[Theorem~2]{VPF15}. However, our approache is different. \cite[Theorem~6.1]{V14} uses Bregman distance and some nontrivial results in \cite{V14} that typically work with  convexity. Corollary~\ref{RobCon} provides a simple and direct proof.  Most importantly,  Theorem~\ref{Rob} suggests that robust recovery with linear rate occurs  without convexity and reveals the lying property (sharp minima) for robust recovery with linear rate. %The approach is employed later in Theorem~\ref{SRob} when sharp minima is replaced by strong minima.   

%Although the Lipschitz modulus $L$ could be estimated for any continuous convex functions \cite[Proposition~8.28]{BC11}, it is rather complicated. However, the similar bound to \eqref{Est} in \cite[Theorem~6.1]{V14}

%Although descent cones can be used to prove (i) as in Proposition~\ref{Shar}, it is not clear how to use it to prove (ii). Our technique in Theorem~\ref{Rob} is uniform for both (i) and (ii) by using the projection to the affine constraint. The same idea will be  employed in Theorem~\ref{SRob}.

%Another important thing about Theorem~\ref{Rob} is that both bounds obtained in \eqref{Est2} and \eqref{Est} are explicit. The only constant that is not trivial is $c$. In  Theorem~\ref{mtheo} we provide an estimation for this number via the so-called {\em Source Identity} that can be computed numerically. The bounds in the aforementioned results  \cite{FPVDS13, GHS11, V14, VPF15, ZYY16} have  hidden constants  that are hard to estimate. \end{proof} 

}
\end{Remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Strong minima and robust recovery}
We now turn to showing that a strong solution to problem \eqref{BP0} also guarantees robust recovery, but the rate of convergence is slower. Unlike sharp minima, the property of strong solution in \eqref{Str} is only  local. 

\begin{Theorem}[Strong minima for robust recovery]\label{SRob} Suppose that $J$ satisfies \eqref{AC} at $x_0$ and is Lipschitz continuous around $x_0$ with modulus $L>0$. If  $x_0$ is a unique and strong solution to problem \eqref{BP0} with constant $\kk>0$, the following statements hold when $\delta>0$ is sufficiently small.
\begin{enumerate}[label={\rm (\roman*)}]
\item Any solution $x_\delta$ to problem \eqref{BP1} with $\|y-y_0\|\le \delta$ satisfies:
\begin{eqnarray}\label{Est4}
        \|x_\delta-x_0\|\le \left[\frac{4}{\kk}L\|\Phi^\dag\| \delta+4\|\Phi^\dag\|^2\delta^2\right]^{\frac{1}{2}}.
    \end{eqnarray}
    
\item For any constant $c_1>0$, every minimizer $x_{\delta}$ to problem \eqref{Las3} with $\|y-\Phi x_0\|\le \delta$ and $\mu= c_1\delta$ satisfies
    \begin{equation}\label{Est3}
        \|x_\mu-x_0\|\le\sqrt{\dfrac{c_1}{(1-c_1\kk\|\Phi^\dag\|^2\delta)\kk}}\left(\dfrac{1}{c_1}+L\|\Phi^\dag\|\right)\delta^\frac{1}{2}.
        \end{equation}
    \end{enumerate}
\end{Theorem}
\begin{proof} 
 Suppose that $x_0$ is the strong solution to \eqref{BP0} with constant $\kk>0$. We find $\ve>0$ such that 
\begin{equation}\label{Stron}
   J(x) \ge J(x_0)+\frac{\kk}{2}\|x-x_0\|^2\quad \mbox{for all}\quad x\in \Phi^{-1}y_0\cap\B_\nu(x_0). 
\end{equation}
%Since $x_0$ is the unique solution to problem \eqref{BP0}, we have $\Ker D^*\cap \Ker \Phi=\{0\}$. Hence there exists $\ell>0$ such that 
%\begin{equation}\label{DPhi}
  %   J(x)\ge \ell\|x\|\quad \mbox{for all}\quad x\in \Ker \Phi.
%\end{equation}
%To justify (i), let $\ox_\delta$ be the projection of $x_\delta$ to $\Phi^{-1}y_0$. 
%Note that $J(x_0)\ge J(x_\delta)$. Since $J$ is coercive, the sequence $\{x_\delta\}$ is bounded. Pick any subsequence $\{x_{\delta_q}\}$ of $\{x_\delta\}$ converging to some $u_0$ as $q\to \infty$. We get that $J(x_0)\ge J(u_0)$ and $\Phi u_0=y_0$. Since $x_0$ is the unique solution to \eqref{BP0}, we have $u_0=x_0$. 
%\begin{eqnarray}\label{Phid2}\begin{array}{ll}
%J(x_0)&\disp\ge J(x_\delta)\ge J(\ox_\delta)-L\|x_\delta-\ox_\delta\|\\
%&\ge \disp J(\ox_\delta)- L\|\Phi^\dag\Phi(x_\delta-x_0)\|\quad \mbox{(by \eqref{Prox})}\\
%&\ge \disp J(\ox_\delta)- L\|\Phi^\dag\|\cdot\|\Phi(x_\delta-x_0)\|\\
%&\ge\disp J(\ox_\delta)- L\|\Phi^\dag\|2\delta.
%\end{array}
%\end{eqnarray}
%Moreover, we obtain from \eqref{DPhi} that
%\begin{equation}\label{Bo}
%J(\ox_\delta)\ge \|D^*(\ox_\delta-x_0)\|_\AA-J(x_0)\ge \ell\|\ox_\delta-x_0\|-J(x_0).
%\end{equation}
Since $x_0$ is the unique solution to \eqref{BP0}, Proposition~\ref{NRC} tells us that $x_\delta\to x_0$. Let $\ox_\delta$ be the projection of $x_\delta$ to $\Phi^{-1}y_0$. We have $x_\delta,\ox_\delta\in \B_{\min\{\ve,\nu\}}(x_0)$ with $\nu$ in \eqref{Stron} and $\ve$ in \eqref{Lip}, when $\delta$ is sufficiently small. Observe from \eqref{Lip} and \eqref{Stron} that  
\begin{eqnarray}\begin{array}{ll}
L\|x_\delta-\ox_\delta\|&\ge J(\ox_\delta)-J(x_\delta)\ge  J(\ox_\delta)-J(x_0)\\
&\disp\ge \disp\frac{\kk}{2}\|\ox_\delta-x_0\|^2=\frac{\kk}{2}\left[\|x_\delta-x_0\|^2-\|x_\delta-\ox_\delta\|^2\right].
\end{array}
\end{eqnarray}
This together with \eqref{Pro} tells us that 
\begin{eqnarray*}\begin{array}{ll}
\dfrac{\kk}{2}\|x_\delta-x_0\|^2&\disp\le  L \|x_\delta-\ox_\delta\|+\frac{\kk}{2}\|x_\delta-\ox_\delta\|^2\\
&\disp=L\|\Phi^\dag \Phi (x_\delta -x_0)\|+\frac{\kk}{2}\|\Phi^\dag \Phi (x_\delta -x_0)\|^2\\
&\disp\le L\|\Phi^\dag\| \cdot\|\Phi x_\delta-y+y-y_0\|+\frac{\kk}{2}\|\Phi^\dag\|^2\cdot\| \Phi x_\delta -y+y-y_0\|^2\\
&\disp\le L\|\Phi^\dag\| 2\delta+\frac{\kk}{2}\|\Phi^\dag\|^24\delta^2,\\
\end{array} 
\end{eqnarray*}
which verifies \eqref{Est4} and completes the proof of (i).


To justify (ii), let $\ox_\mu$ be the projection of $x_\mu$ to $\Phi^{-1}y_0$. By Proposition~\ref{NRC}, we have $x_\mu,\ox_\mu\in \B_{\min\{\ve,\nu\}}(x_0)$  when $\delta$ is sufficiently small. Observe from \eqref{Stron}  that 
\begin{eqnarray*}\begin{array}{ll} J(x_\mu)-J(x_0) 
&\disp = J(\ox_\mu)-J(x_0)+J(x_\mu)-J(\ox_\mu)\\
&\disp\ge \frac{\kk}{2}\|\ox_\mu-x_0\|^2-L\|x_\mu-\ox_\mu\|\\
&\disp= \frac{\kk}{2}\big[\|x_\mu-x_0\|^2-\|x_\mu-\ox_\mu\|^2\big]-L\|x_\mu-\ox_\mu\|.
\end{array}
\end{eqnarray*}
Set $\al \eqdef \|\Phi(x_\mu-x_0)\|$. Since $\|x_\mu-\ox_\mu\|=\|\Phi^\dag\Phi(x_\mu-x_0)\|$ by \eqref{Pro}, we obtain from \eqref{Low} and the latter  that  
\begin{eqnarray*}\begin{array}{ll}
\dfrac{2\al\delta-\al^2}{2\mu}\ge \disp\frac{\kk}{2}\left[\|x_\mu-x_0\|^2-\|\Phi^\dag\|^2\al^2\right]-L\|\Phi^\dag\|\al.
\end{array}   
\end{eqnarray*}
It follows that 
\[\begin{array}{ll}
\frac{\kk}{2}\|x_\mu-x_0\|^2&\le\disp \left[\frac{\delta}{\mu}+L\|\Phi^\dag\|\right]\al-\left(\dfrac{1}{2\mu}-\dfrac{\kk}{2}\|\Phi^\dag\|^2\right)\al^2\\
&\disp\le \frac{1}{2}\left(\dfrac{1}{\mu}-\kk\|\Phi^\dag\|^2\right)^{-1}\left[\frac{\delta}{\mu}+L\|\Phi^\dag\|\right]^2,
\end{array}
\]
which ensures \eqref{Est4} by involving  some simple algebra. The proof is complete.  
\end{proof} 


 If the regularizer $J$ is convex, the Lipschitz property of $J$ around $x_0$ is equivalent to the continuity of $J$ at $x_0$; see, e.g., \cite[Theorem~8.29]{BC11}. Moreover, the assumption that $x_0$ is a unique solution in Theorem~\ref{SRob} holds trivially when $x_0$ is a strong minimizer. 
 
 \begin{Corollary} Suppose that $J$ is a convex function satisfying condition \eqref{AC} and that $J$ is continuous at $x_0$. If $x_0$ is a strong solution to problem \eqref{BP0} then the convergence rate $\mathcal{O}(\delta^\frac{1}{2})$ in both {\rm (i)} and {\rm (ii)} of Theorem~\ref{SRob} hold. 
 
 \end{Corollary}



One question from Theorem~\ref{SRob} is whether the rate $\mathcal{O}(\delta^\frac{1}{2})$ in \eqref{Est2} and \eqref{Est} is optimal under strong solution. We do not have the answer yet, it may depend on different norms. For the case of Euclidean norm $J(x)=\|x\|$, we could prove that the rate could be improved to $\mathcal{O}(\delta)$. This fact is minor, we omit the details.%  In this case, $x_0$ is the projection from $0$ to the affine $\Phi x=y_0$, i.e., $x_0=\Phi^\dag y_0$ is the unique solution to \eqref{BP0}. According to Theorem~\ref{BP12}, it is a strong solution, as the Euclidean norm is a particular case of the $\ell_1/\ell_2$ norm.


%\begin{Theorem}[Robust recovery for $\ell_2$ optimization problems]\label{ell5} Let $J(\cdot)$ be  the Euclidean norm $\|\cdot\|$. Suppose that $x_0$ is a solution to problem \eqref{BP0}. Then for sufficiently small $\delta>0$, the following are satisfied.
%\begin{enumerate}[label={\rm (\roman*)}]
%\item Any solution $x_\delta$ to problem \eqref{BP1} satisfies
%\begin{equation}\label{Est5}
 %       \|x_\delta-x_0\|\le\mathcal{O}(\delta).
  %  \end{equation}
    
%\item Every minimizer $x_{\delta}$ to \eqref{Las3} with $\|y-\Phi x_0\|\le \delta$ and $\mu= c_1\delta$  satisfies
 %   \begin{equation}\label{Est6}
  %      \|x_\mu-x_0\|\le\mathcal{O}(\delta).
   % \end{equation}
    %\end{enumerate}
%\end{Theorem}
%\begin{proof} 
 Let us start with (i). If $x_0=0$, we have 
%$J(x)-J(x_0)= \|x-x_0\|$, which means $x_0$ is a sharp solution to \eqref{BP0}. By Theorem~\ref{Rob}, $\|x_\delta-x_0\|\le \mathcal{O}(\delta).$

%Now suppose that $x_0\neq 0$. Note that $x_0=\Phi^\dag y_0$. By Theorem~\ref{SRob}, $x_\delta\to x_0$. Observe that $x_\delta$ is the minimizer to the following nonlinear problem
%\[
%\min\quad   \frac{1}{2}\|x\|^2\quad \mbox{subject to}\quad \|\Phi x-y\|^2\le \delta^2.
%\]
%Hence, there exists a Lagrange multiplier $\lm\ge 0$ such that 
%%\begin{equation}\label{La}
%x_\delta+\lm \Phi^*(\Phi x_\delta-y)=0\quad \mbox{and}\quad \lm (\|\Phi x_\delta-y\|^2-\delta^2)=0.
%\end{equation}
%Since $x_\delta\to x_0\neq 0$, $\lm\neq0$ when $\delta$ is sufficiently small. Suppose without loss of generality that $\lm>0.$ It follows from \eqref{La} that $x_\delta=\lm(\Id+\lm \Phi^*\Phi)^{-1}( \Phi^*y)$. We obtain from \eqref{La} that \[\delta=\|(\lm \Phi(\Id+\lm \Phi^*\Phi)^{-1} \Phi^*-\Id)y\|.\]
%Let $\Phi=U\Sigma V^*$ be the SVD of $\Phi$ with $U\in \R^{m\times r}$, $V\in \R^{n\times r}$, $\Sigma\in \R^{r\times r}$, and $r={\rm rank}\, \Phi$. It follows that $x_0=V\Sigma^{-1}U^*y_0$, $x_\delta=\lm V(\Id+\lm \Sigma^2)^{-1}\Sigma U^*y$,  and 
%\begin{equation}\label{La2}
%\delta=\|U(\lm \Sigma (\Id+\lm \Sigma^2)^{-1} \Sigma-\Id ) U^*y\|=\|U(\Id+\lm \Sigma^2)^{-1}U^*y\|. 
%\end{equation}
%Since $x_0\neq 0$ and $y_0\neq 0$, we have $\|U^*y\|=\|y\| \ge \|y_0\|-\delta>0$.  \eqref{La2} tells us that $\lm\to \infty$ as $\delta\dn 0$. 
%Define $\eta \eqdef \lm^{-1}\to 0$ as $\eta\dn 0$, we derive from \eqref{La2} that  
%\[
% \delta=\eta \|U (\eta\Id+ \Sigma^2)^{-1}  U^*y\|^2.
 %\]
%It follows that $\eta=\mathcal{O}(\delta)$. Hence we have
%\[\begin{array}{ll}
%\|x_\delta-x_0\|&\disp=\|\lm V(\Id+\lm \Sigma^2)^{-1}\Sigma U^*y-V\Sigma^{-1}U^*y_0\|\\
%&=\disp\|
%V(\eta\Id+ \Sigma^2)^{-1}\Sigma U^*y-V\Sigma^{-1}U^*y_0\|\\
%&=\disp \|
%V(\eta\Id+ \Sigma^2)^{-1}\Sigma U^*y-V\Sigma^{-1}U^*y\|+\|V\Sigma^{-1}U^*(y-y_0)\|\\
%&\le \disp\|
%\eta V(\eta\Id+ \Sigma^2)^{-1}\Sigma^{-1} U^*y\|+\|\Sigma^{-1}\|\cdot\|y-y_0\|\\
%&\le \disp
%\eta \|(\eta\Id+ \Sigma^2)^{-1}\Sigma^{-1}\|\cdot\|y\|+\|\Sigma^{-1}\|\cdot\|y-y_0\|.
%\end{array}
%\]
%Since $\eta =\mathcal{O}(\delta)$, $y\to y_0\neq 0$, and $\|y-y_0\|\le \delta$, we have $\|x_\delta-x_0\|\le \mathcal{O}(\delta)$. This verifies \eqref{Est5} and (i). 

%To justify (ii), observe from Theorem~\ref{SRob} again that $x_\mu\to x_0=\Phi^\dag y_0$ as $\delta\dn 0$. It is similar to the beginning of the proof of part (i) that we only need to check \eqref{Est6} when $x_0\neq 0$. Thus $x_\mu\neq 0$ when $\delta$ is sufficiently small. Since $x_\mu$ is a solution to problem \eqref{Las3}, we have 
%\begin{equation}\label{xmu}
%\mu \frac{x_\mu}{\|x_\mu\|}+\Phi^*(\Phi x_\mu-y)=0.
%\end{equation}
%Define $s \eqdef \|x_\mu\|>0$, \eqref{xmu} gives us that  $x_\mu=s(\mu\Id+s\Phi^*\Phi)^{-1}\Phi^* y.$ 
%We have
%\[\begin{array}{ll}
%\|x_\mu-x_0\|&=\disp\|sV(\mu\Id+s\Sigma^2)^{-1} \Sigma U^*y-V\Sigma^{-1}U^*y_0\|\\
%&\le \disp\|sV(\mu\Id+s\Sigma^2)^{-1} \Sigma U^*y-V\Sigma^{-1}U^*y\|+\|V\Sigma^{-1}U^*(y-y_0)\|\\
%&\le \disp\mu\|V(\mu\Id+s\Sigma^2)^{-1} \Sigma^{-1} U^*y\|+\|V\Sigma^{-1}U^*\|\cdot\|y-y_0\| .\\
%\end{array}
%\]
%Since $s\to \|x_0\|>0$ as $\delta\dn 0$ and $\|y-y_0\|\le \delta$, the latter gives us that 
%\[
%\|x_\mu-x_0\|\le \mathcal{O}(\delta), 
%\]
%which verifies \eqref{Est6} and completes the proof of the theorem. \end{proof} 


%Since Euclidean norm is a particular case of $\ell_1/\ell_2$ norm, our Theorem~\ref{BP12} tells that the strong solution assumed in Theorem~\ref{ell5} is just a unique solution. This together Proposition~\ref{NRC} implies that solution uniqueness to \eqref{BP0} with Euclidean norm is equivalent to robust recovery with linear rate.



%The reason we refer  $\mathcal{O}(\delta^\frac{2}{3})$ as optimal rate for robust recovery when $x_0$ is a strong solution is the order $\frac{2}{3}$ cannot be improved. The following shows that $\mathcal{O}(\delta^\frac{2}{3})$ is achieved. 


%\begin{Example}[Strong solution  for robust recovery achieves optimal rate $\mathcal{O}(\delta^\frac{2}{3})$] {\rm 
%}
%\end{Example}





